RV-CURE: A RISC-V Capability Architecture for Full Memory Safety

Despite decades of efforts to resolve, memory safety violations are still persistent and problematic in modern systems. Various defense mechanisms have been proposed, but their deployment in real systems remains challenging because of performance, security, or compatibility concerns. In this paper, we propose RV-CURE, a RISC-V capability architecture that implements full-system support for full memory safety. For capability enforcement, we first propose a compiler technique, data-pointer tagging (DPT), applicable to protecting all memory types. It inserts a pointer tag in a pointer address and associates that tag with the pointer's capability metadata. DPT enforces a capability check for every memory access by a tagged pointer and thereby prevents illegitimate memory accesses. Furthermore, we investigate and present lightweight hardware extensions for DPT based on the open-source RISC-V BOOM processor. We observe that a capability-execution pipeline can be implemented in parallel with the existing memory-execution pipeline without intrusive modifications. With our seamless hardware integration, we achieve low-cost capability checks transparently performed in hardware. Altogether, we prototype RV-CURE as a synthesized RTL processor and conduct full-system evaluations on FPGAs running Linux OS. Our evaluations show that RV-CURE achieves strong memory safety at a 10.8% slowdown across the SPEC 2017 C/C++ workloads.

==> Submitted/A.Abstract.tex <==
%-------------------------------------------------------------------------------
\begin{abstract}
%-------------------------------------------------------------------------------
Despite decades of efforts to resolve, memory safety violations are still persistent and problematic in modern systems. Various defense mechanisms have been proposed, but their deployment in real systems remains challenging because of performance, security, or compatibility concerns.

In this paper, we propose \mech{}, a RISC-V capability architecture that implements full-system support for practical memory safety. For capability enforcement, we first propose a compiler technique, data-pointer tagging (DPT), applicable to protecting all memory types. It inserts a pointer tag in a pointer address and associates that tag with the pointer's capability metadata. DPT enforces a capability check for every memory access by a tagged pointer and thereby prevents illegitimate memory accesses. Furthermore, we investigate and present lightweight hardware extensions for DPT based on the open-source RISC-V BOOM processor. We observe that a capability-execution pipeline can be implemented in parallel with the existing memory execution pipeline without incurring much hardware complexity. With our seamless hardware integration, we achieve low-cost capability checks transparently performed in hardware. Altogether, we prototype \mech{} as a synthesized RTL processor and conduct full-system evaluations on FPGAs running Linux. Our evaluations show that \mech{} achieves strong memory safety at a 10.9\% slowdown across SPEC 2017 C/C++ workloads at the cost of 8.6\% area and 11.6\% power overheads. Lastly, DPT is highly synergistic with static taint analysis that helps identify security-critical objects and prune unnecessary security checks. With static taint analysis, we show that the average performance overhead can be reduced to 7.5\%.

% Finally, we evaluate \mech{}'s security capabilities by testing the NIST Juliet test suite.
\end{abstract}

==> Submitted/B.Introduction.tex <==
%-------------------------------------------------------------------------------
\section{Introduction}
%-------------------------------------------------------------------------------

For decades, memory safety issues have exposed substantial security threats to computer systems. Memory safety violations occur when instructions perform illegitimate memory accesses to a program's address space. There are broadly two types of memory safety violations. If a memory access occurs outside of its allowed range, e.g., buffer overflow and out-of-bounds (OOB) access, it violates spatial memory safety. When a memory region is accessed after the region is no longer valid, temporal memory safety is violated, e.g., use-after-free (UAF). Despite long-term efforts to resolve, memory safety issues are still the most prevalent and problematic in the wild. Recent studies~\cite{GoogleReport,BluehatReport} show that $\sim$70\% of security vulnerabilities addressed in industry stemmed from memory violations.
%TODO:... \AK{Here a list with the 2 types of memory safety issues may be useful instead of just text.} 

Arguably, the primary hindrance to ensuring memory safety in practice is the performance overhead resulting from defense mechanisms~\cite{SoK_paper}. While various proficient software tools for detection of memory safety violations ~\cite{asan,Softbound,BaggyBounds,BaggyBoundsChecking,TaintCheck,EffectiveSan} have been developed, the significant runtime overhead of such tools, e.g., a 73\% slowdown in AddressSanitizer (ASan)~\cite{asan}, has hampered their adoption as a viable solution for runtime bug detection, limiting their usage to debug and testing.

Hardware-based mechanisms address the performance concern by adopting architectural support for accelerating security checks. However, most prior work either requires intrusive hardware changes or lacks security guarantees, impeding their deployment in commodity. For instance, despite its strong security guarantees, the fat pointer design in the CHERI architectures~\cite{CHERI,Cheri-concentrate,CHERIvoke,Cornucopia} may impose non-trivial hardware complexity, whereas Intel MPX~\cite{IntelMPX} lacks temporal safety guarantee.

In addition, the history of security solutions deployed in commodity systems reveals that compatibility\footnote{In this paper, we consider source and binary compatibility (\cref{s:overview}).} is one of the major factors hindering their successful deployment~\cite{SoK_paper}. However, maintaining compatibility while ensuring full memory safety remains challenging, particularly in hardware-based mechanisms. For instance, modifying almost the entire system stacks lets the CHERI capability model give up compatibility with legacy code.\footnote{With such changes, Arm has developed the Morello prototype board rather than adding it to their mainstream architectures~\cite{morello}.} %Califorms~\cite{Califorms} and No-FAT~\cite{No-FAT} modify data-type structures for fine-grained safety, thereby losing source and binary compatibility.

To avoid the non-trivial problems caused by the design choice of having a fat pointer, recent proposals~\cite{AOS,in-fat-pointer,No-FAT,C3} have started adopting a pointer-tagging method, which stores a pointer tag in the unused upper bits of a pointer without expanding the pointer size and uses the tag to look up object metadata or perform an object-based tag match. Nevertheless, simultaneously achieving three essential properties, i.e., performance, security, and compatibility, has seemed far-off until now. For example, AOS~\cite{AOS} and C\textsuperscript{3}~\cite{C3} only protect heap memory regions, and In-Fat Pointer~\cite{in-fat-pointer} does not support temporal safety. No-FAT~\cite{No-FAT} requires data structure modifications, causing compatibility loss.
%and In-Fat Pointer~\cite{in-fat-pointer}, lacks security assurance, e.g., heap or spatial safety only, while No-FAT~\cite{No-FAT} loses source and binary compatibility for sub-object safety.

As an attempt to end this eternal war on memory safety bugs, we propose \mech{}, a RISC-V capability architecture that orchestrates compiler, architecture, and system designs for practical memory safety. To this end, we first propose a pointer-tagging method, \textit{data-pointer tagging} (DPT), applicable to all memory types, including stack, heap, and global memory. Using DPT, \mech{} enforces per-object capability\footnote{E.g., bounds information, privileges, and access permissions.} that defines the legitimacy of memory accesses. Whenever an object is allocated, DPT places a pointer tag in a pointer address and associates that tag with the pointer's capability metadata maintained in a capability metadata table (CMT). During the object's lifetime, DPT enforces every memory access by the tagged pointer to be validated via a capability check, ensuring spatial safety. Upon a deallocation, DPT clears its metadata from the CMT while its pointer aliases remain tagged. Hence, any subsequent accesses by the tagged dangling pointers would trigger capability checks and end up with failures, i.e., temporal safety is ensured.

%Furthermore, we extend the proposed DPT to support fine-grained (intra-object) safety, i.e., overflow detection between different fields in a struct. Providing sub-object safety at low cost is difficult, as evidenced by prior studies~\cite{Califorms,No-FAT,EffectiveSan} that end up relinquishing either compatibility or performance. Aiming to retain both performance and compatibility, we propose \textit{dynamic pointer mutation} that re-tags (mutate) sub-object pointers and assigns narrowed capability metadata. [TODO] write more...

While DPT manifests as a generalized approach to all memory types, na\"ively broadening security coverage may result in non-trivial runtime overheads due to the increased number of security metadata and checks. To accomplish robust yet practical protection, we further investigate efficient, lightweight hardware extensions for DPT based on the RISC-V BOOM core~\cite{BOOM}, which is one of the most sophisticated open-source out-of-order processors. In our design exploration, we observe that a capability-execution pipeline can be seamlessly integrated in parallel with the existing memory execution pipeline. Furthermore, we analyze that potential performance degradation due to DPT is mostly caused by hardware resource contentions through the shared data cache access path, including a load-store unit (LSU) scheduler, a translation look-aside buffer (TLB), and a data cache. To mitigate those contentions, we come up with micro-architectural optimizations.

% static taint analysis
Last but not least, we focus on the known security concept that attackers typically exploit security vulnerabilities via external inputs, e.g., file I/O, user inputs, and network, and only the memory locations influenced by external sources are exploitable~\cite{TaintCheck,perl,scrash}. Hence, DPT can be synergistic with static taint analysis by identifying vulnerable (tainted) memory objects and enabling selective protection only to those. %By employing the static taint analysis, we explore the trade-off between performance and security.

Putting it all together, we prototype \mech{} on top of FireSim~\cite{firesim}, an FPGA-accelerated full-system hardware simulation platform. In our full-system framework, we evaluate the SPEC 2017 C/C++ workloads~\cite{SPEC2017} and show that \mname{} incurs a 10.9\% slowdown on average. Moreover, when static taint analysis is applied, we observe the average slowdown reduced down to 7.5\%. Our RTL synthesis task measures 8.6\% area and 11.6\% power overheads due to our hardware modifications. To contribute to the research communities, we plan to open-source \mech{} upon publication.\footnote{https://github.com/xxxxxx/xxxxxx}

\begin{figure}[t]
\begin{lstlisting}[language=c++, style=mystyle3]
int main(void) {
  char constArr[] = "Hello World";
  char vulArr[10];
  scanf("%s", vulArr);
  printf("constArr: %s\n", constArr);
  printf("vulArr: %s\n", vulArr);
... }
\end{lstlisting}
\caption{A simple buffer overflow example.}
\label{lst:example_code}
\end{figure}

In summary, we make the following contributions:

\begin{compactitem}[$\bullet$]
  \item We present \mname{}, a full-system framework that orchestrates compiler, architecture, and system designs.
  \item We propose DPT, a generalized data-pointer tagging method for all memory types protection, including stack, heap, and global memory.
  \item We explore realistic design space on top of the RISC-V BOOM core and realize a synthesizable RTL processor.
  \item We employ static taint analysis and explore the trade-off between performance and security.
  \item \mech{} reports a 7.5\% average slowdown across the SPEC 2017 C/C++ workloads at the best case.
  %\item To the best of our knowledge, \mname{} is the first hardware-based mechanism that ensures complete memory safety with legacy code compatibility.
\end{compactitem}


==> Submitted/C.Background.tex <==
%-------------------------------------------------------------------------------
\section{Background}
%-------------------------------------------------------------------------------

\subsection{Memory Safety Vulnerability}
Memory safety errors occur when an instruction performs spatially or temporally illegal access to a program's memory address space. Accessing outside its designated memory address range violates spatial memory safety, whereas temporal safety is violated when accessing no-longer-valid memory regions. Despite its notoriety for a long time, recent studies by Microsoft~\cite{BluehatReport} and Google~\cite{GoogleReport} show that memory safety issues are still the most prevailing ($\sim$70\%) and problematic. The resulting side-effects include a system crash, privilege escalation, and information leakage. Given the criticality of such vulnerabilities, ensuring memory safety becomes the task at hand in modern systems.
%Given their prevalence and critical side-effects, including a system crash, privilege escalation, and information leakage, ensuring memory safety becomes the task at hand in modern systems.

\fref{lst:example_code} shows a simple yet vulnerable code example where a user provides an input string via \cc{scanf()}. In this example, an attacker can simply inject a long input sequence, whose size exceeds the size of the target array (\cc{vulArr}), to invoke a buffer overflow. Since the unsafe \cc{scanf()} has no knowledge of the array size, it will just store the given input to the target memory address and end up overwriting the adjacent memory space. Note that unlike \cc{vulArr}, \cc{constArr} is initialized with a constant string, so it could be safe from buffer overflows caused by user inputs. In \fref{ss:taint}, we discuss such security implications and our protection strategy with an instrumented code example (\fref{fig:selective_sign}b).

\ignore{
\subsection{Challenges in Memory Safety}
\label{ss:challenge}
From previously proposed mechanisms against memory safety vulnerabilities, we identify the following essential but challenging properties to achieve altogether to be an ideal memory protection mechanism. %, as shown in most prior work. %We defer detailed discussion on related work to \fref{s:related_work}.

\noindent
\textbf{Performance.} Reducing a performance overhead is crucial for a runtime detection solution. For this reason, most software tools tend~\cite{asan,PhASAR,BaggyBounds,Softbound} to be used only for testing and debugging and fail to be deployed at runtime. On the other hand, hardware mechanisms reduce the performance overhead but often compromise security assurance or compatibility.

\noindent
\textbf{Security.} Ensuring strong security guarantees is non-trivial even with a possible trade-off between performance and security. The primary challenge is how to properly maintain security metadata, e.g., memory objects' size and lifetime, and enable spatial and temporal security checks. In particular, many prior studies~\cite{AOS,C3,REST} do not guarantee sub-object safety, i.e., detecting intra-object overflow, while some studies~\cite{Califorms,No-FAT} support that at the cost of painful compatibility loss.

\noindent
\textbf{Compatibility.} Preserving compatibility is important to be deployable in commodity systems. 
Source compatibility is lost if it requires any manual source modification, while binary compatibility is lost if instrumented binaries cannot run with legacy code. The lack of source compatibility may make a solution unscalable for a large software project, and a solution with binary incompatibility cannot run with unmodified user or system libraries.

\noindent
\textbf{Hardware Complexity.} Implementing architectural support for security can bring in a significant performance gain, as evidenced by many prior studies~\cite{Cheri-concentrate,CHERI,CHERIvoke,Watchdog,Hardbound}. However, such hardware schemes often require intrusive hardware changes and discourage CPU vendors from adopting the proposed features. For instance, despite their strong security guarantees, CHERI architectures are known to require non-trivial hardware complexity due to their fat-pointer and co-processor implementations, e.g., 32\% logic overhead~\cite{CHERI}.
}

\begin{table}[t]
    \centering
    \caption{Comparison of pointer-tagging approaches.}
    \label{tab:comparison}
    \begin{threeparttable}
    \begin{scriptsize}
    \begin{tabular}{@{}lccc@{}}
    
    \toprule
    Mechanism & Spatial Safety & Temporal  Safety & Compatibility Loss~\tnote{1} \\
    \midrule
    AOS~\cite{AOS}                  & $\triangle$~\tnote{2}     & $\triangle$~\tnote{2}     & $-$                   \\
    %CHEx86~\cite{CHEx86}            & $\triangle$~\tnote{2}     & $\triangle$~\tnote{2}     & $-$                   \\
    C\textsuperscript{3}~\cite{C3}  & $\triangle$~\tnote{2}     & $\triangle$~\tnote{2}     & $-$                   \\
    In-Fat~\cite{in-fat-pointer}    & $\bigcirc$                & X                         & $-$     \\
    NoFat~\cite{No-FAT}             & $\bigcirc$                & $\bigcirc$                & Src,Bin    \\
    \midrule
    \mech{}                         & $\bigcirc$                & $\bigcirc$                & $-$           \\
    \bottomrule
    \end{tabular}
    \end{scriptsize}

    \begin{tablenotes}
    \begin{footnotesize}
    \item[1] Source modifications or recompiling the libraries are required, losing source compatibility (Src) or binary compatibility (Bin).
    \item[2] Protection only applies to heap memory regions.

    \end{footnotesize}
    \end{tablenotes}   
\end{threeparttable}
\label{tab:ptr_comp}
\end{table}

\subsection{Pointer-Tagging Approaches}
\label{ss:point-tag}

A recent trend shows that pointer-tagging approaches~\cite{No-FAT,C3,AOS,in-fat-pointer,zero21,Califorms} draw great attention from research communities thanks to their potential advantages in performance, compatibility, and hardware complexity. These methods place a pointer tag in a pointer and use the tag to look up object metadata in memory or perform an object-based tag match. Hence, it not only complies with conventional execution models but also enables efficient metadata management; no explicit metadata propagation is required since pointer tags are propagated along with pointer addresses. Note that fat pointer designs with an increased pointer size have suffered from non-trivial hardware complexity and compatibility issues, which are avoidable in pointer-tagging methods.

Nevertheless, none of the prior work appears to be a full memory safety solution with legacy code compatibility. As shown in \fref{tab:ptr_comp}, AOS~\cite{AOS} and C\textsuperscript{3}~\cite{C3} provide heap memory protection only, while In-Fat Pointer~\cite{in-fat-pointer} does not support temporal safety. No-Fat~\cite{No-FAT} requires Abstract Syntax Tree (AST)-level translation that modifies data structure types, losing source and binary compatibility. These limitations by prior work indicate that the war against memory safety bugs is not over yet, and devising a comprehensive but practical solution is still urgently called for. More discussions on prior work are provided in \fref{s:related_work}.



\subsection{Prior Work: AOS}\label{ss:aos}
Among the prior work, AOS is prominent for its pointer-signing scheme using the Arm pointer authentication (PA) primitives and its approach to handling hash collisions. As shown in \fref{fig:aos_overview}, AOS generates 16-bit pointer authentication code (PAC) and 2-bit address hashing code (AHC) and then associates the PAC with a pointer's bounds. Since the PAC size is limited, there can exist PAC collisions across different pointers. To deal with the PAC collisions, AOS maintains a multi-way bounds table structure, called a hashed-bounds table (HBT). The HBT is indexed by PACs, and each row can accommodate multiple bounds. To support such a structure, AOS implements an iterative bounds search performed over multiple ways of the HBT.

While AOS presents a promising 8.4\% slowdown, we note that AOS only runs 3-billion instructions using the gem5 simulator~\cite{gem5} for the sake of simulation time. We speculate that running a small portion of programs in AOS might not produce realistic results since memory allocation and access behaviors can vary over the period of program execution. In our evaluations where we entirely execute SPEC CPU 2017 C/C++ workloads, our speculation turns out to be true providing an additional observation.

First, AOS measures the average number of iterative accesses to the HBT to be close to one. However, as shown in Column 3 in \fref{tab:hit_iter}, we observe that the average number of iterations is not trivial even with its proposed bounds way buffer (BWB), 17.03 at a maximum and 3.75 on average. It is obvious that the performance guarantee by AOS would not hold true anymore with such non-trivial iterations. In addition, we observe more frequent bounds-table resizing happen, whereas AOS observes only once for \cc{sphinx3} and twice for \cc{omnetpp}, respectively.% kmalloc() can fail at runtime. 

Besides the characteristic of the HBT, AOS only supports heap memory safety. Even though AOS foresees the diminishing number of stack corruption errors, non-trivial error cases on stack memory still exist~\cite{GoogleReport,BluehatReport}. Given that only one memory bug could lead to a chain of other memory violations, complete protection on all memory types is desirable.

%We take an analogous approach, however, we unveil the performance characteristics of the hashed metadata table that may require iterative accesses until valid metadata are found.
%Furthermore, ****.
\ignore{
%Moreover, AOS implements a memory check unit (MCU) that generates bounds-checking requests for memory accesses by signed pointers. To allow for the HBT's multi-way structure, the MCU operates on a finite-state machine (FSM) that supports an iterative bounds search. Within the FSM, a bounds check can iterate over multiple ways of a row in the HBT until valid bounds metadata are found, which can lead to \cc{n}-repeated memory accesses in a \cc{n}-way HBT at the worst case. [Mention that AOS reports close-one iteration numbers]
While AOS presents promising results, an 8.4\% slowdown, we find two limitations as follows.

[average iteration numbers]
[physicslly-addressed HBT] <<<
However, once we have a virtually-addressed table, new hardware resource contentions.

once we execute entire program, the number of allocation stacks up.

First, AOS only supports heap memory safety. Even though AOS foresees the diminishing number of stack corruption errors, non-trivial error cases on stack memory still exist~\cite{GoogleReport,BluehatReport}. Given that only one memory bug could lead to a chain of other memory violations, complete protection on all memory types is desirable. In addition, AOS does not provide intra-object protection. Second, AOS evaluates its performance using the gem5 simulator~\cite{gem5} by running 3 billion instructions for the sake of simulation time. However, it turns out that running a small portion of a program does not properly capture the overhead of its iterative bounds-search operation. Although AOS reported the average number of iterations close to one, in our evaluation where we run the whole programs, we observe that the average number can significantly increase (up to $\sim$ in SPEC CPU 2017 benchmarks), which would notoriously impact the overall performance.
}

\begin{figure}[t]
\centering
\includegraphics[width=0.8\columnwidth]{Fig/aos.pdf}
\caption{Pointer-tagging format and HBT access in AOS.}
\label{fig:aos_overview}
\end{figure}

\begin{figure*}[t]
\centering
\includegraphics[width=2\columnwidth]{Fig/overview.pdf}
\caption{Overview of the \mech{} workflow.}
\label{fig:overview}
\end{figure*}

As discussed, despite the attractive advantages of pointer-tagging methods, prior work still does not manifest as a complete solution. In addition, a precise performance evaluation using architecture simulators for security solutions requiring metadata management appears to be challenging. From these observations, we bring up two questions; 1) can we generalize a pointer-tagging method to support \textit{full memory safety}? and 2) can we build a \textit{full-stack system} where we can explore practical design space and conduct realistic performance evaluations? In the rest of this paper, we answer these by exploring a full-system framework with a multidisciplinary approach.

%disclose

%When running the whole program, we observe that the average number of iterations can significantly increase (up to $\sim$) in SPEC 2017 workloads, which would obviously lead to poor performance.

%As mentioned in Section 2.2, pointer-tagging methods provide. Nevertheless, we note that with the above-mentioned limitations, realistic performance analysis is not thoroughly investigated and disclosed yet. For this reason, in this work, we decide to build a full-system framework on top of the open-source RISC-V processor and deep-dive into the architecture, compiler, and system design space towards practical memory safety.

%Regarding the security aspect, we bring up one question. \textit{Can we generalize the pointer-tagging method for complete memory safety?} As an answer to the question, we present more sophisticated compiler support explained in \fref{ss:ensuring}.

%Regarding the second limitation, we note that the restriction on reasonable simulation time in most architecture simulators makes it difficult to measure the realistic overhead of the iterative bounds-search operation. This limitation brings up another question. \textit{What if we can build a real system and evaluate the whole program execution?} It should be possible to measure realistic overheads and devise more practical optimization techniques. For this reason, we decide to build a full-system framework on top of the open-source RISC-V processor and deep-dive into the architecture design space towards practical memory safety.

%the fact that most architecture simulations do not run entire program execution for the sake of simulation time makes it difficult to measure the realistic overhead of the iterative bounds-search operation. This brings up one question for us: what if we can build a full-system framework and entirely run programs? Based on the framework, it should be possible to investigate realistic optimization techniques and develop a practical solution. As we implement our design on top of an open-source CPU processor, we deep-dive into potential performance bottlenecks and mitigate those from the architecture and compiler design viewpoints.
%[TODO] adopt an analogous approach 
%We bring up a question: what if we can and enable (ideally equal to one).
%it could be possible to eliminate potential performance loss due to iteration overhead.

%\noindent
%\textbf{Performance overhead.} We note that its overhead is still not close to zero. Given that the performance overhead can keep increasing as we pursue broader security coverage, deep-diving into  potential performance bottlenecks and mitigating those from the architecture or compiler design viewpoints should be worthwhile.

%In this paper, we aim to address common challenges of typical memory safety solutions, including the above-mentioned limitations of AOS, and realize a full-system capability architecture for practical memory safety. In \fref{s:overview}, we overview our multidisciplinary approach encompassing architecture, compiler, and system designs

%we observe that its evaluation fails in capturing the behavior of the entire program execution, particularly regarding the overhead of iterative accesses to the HBT. I
%\noindent
%\textbf{Hardware integration}


%we present more details on the AOS's mechanism since we base our design on its hardware extensions because of its efficient, lightweight implementation. On top of the underlying platform, we introduce slight hardware changes to adapt our proposed protection capabilities (see \fref{ss:hardware_extension}) and employ compiler techniques for optimal performance and security assurance (see \fref{ss:ensuring} and \fref{ss:taint}).
\ignore{
AOS tags each protected pointer with a 16-bit Pointer Authentication Code (PAC) and uses the pointer tag to index a bounds table in memory to look up the corresponding bounds. To enable bounds checking, AOS implements a memory check unit (MCU), as shown in \fref{fig:hardware}, that takes memory access instructions, i.e., load and store, as well as bounds instructions, i.e., \cc{bndstr} and \cc{bndclr}. Depending on the bounds-instruction type, the MCU generates memory requests to store or clear bounds in a hashed bounds table (HBT). Since the HBT is indexed by PACs (embedded in memory addresses), the locations of bounds are calculated using the base address of the HBT and PACs, i.e., \cc{HBT[PAC]}. The MCU examines addresses of memory instructions to determine the necessity of bounds checking. If an address embedding a nonzero PAC is detected, the MCU loads its corresponding bounds and validates the access via hardware-based bounds checking. AOS extends the instruction set architecture (ISA) for the required operations.
}



\ignore{
\begin{compactitem}[$\bullet$]
    \item \textbf{\cc{pacma ptr, mod}}. The \cc{pacma} is used to \textit{sign} a pointer. Using the QARMA block cipher~\cite{QARMA}, it calculates a PAC using a pointer address (\cc{ptr}), a modifier~\footnote{A modifier is a 64-bit tweak to differentiate contexts of a program.} (\cc{mod}), and a PA key.\footnote{New PA keys invisible to user are assigned to each new process.} The PAC is stored in the upper bits of the \cc{ptr}.
    
    \item \textbf{\cc{xpacm ptr}}. The \cc{xpacm} \textit{strips} a pointer to remove the PAC located in the upper bits of the pointer (\cc{ptr}).
    
    \item \textbf{\cc{bndstr ptr, size}}. The \cc{bndstr} calculates bounds using a pointer (\cc{ptr}) and a size and stores the bounds in the location indexed by the PAC of the \cc{ptr} in an HBT.
    
    \item \textbf{\cc{bndclr ptr}}. The \cc{bndclr} clears bounds from the location indexed by the PAC of a pointer (\cc{ptr}) in an HBT.
\end{compactitem}

Since the PAC has a limited size, some pointers can share the same PAC, resulting in PAC collisions. Consequently, the HBT is implemented as a multi-way structure to handle the collisions by accommodating multiple bounds for the same PAC. While such a design makes the HBT scalable, bounds instructions will perform an iterative bounds search over multiple ways. To lower the overhead, a bounds way buffer (BWB) keeps track of recent bounds-table accesses and tries to give correct locations for subsequent accesses upon their first attempts.
}






\ignore{
\subsection{Challenges in Memory Safety}
\label{ss:challenge}

Numerous prior proposals have been presented to prevent memory safety vulnerabilities. While we defer the discussion on related work to \fref{s:related_work}, we identify three major challenges of hardware-based mechanisms in achieving robust (security coverage), efficient (performance), and deployable (compatibility) memory safety.

\noindent
\textbf{How to support full security coverage.}
%\subsubsection{How to support full security coverage?}
The primary challenges in building a hardware-based framework are: 1) how to properly expose software semantics to hardware and 2) how to enable efficient hardware operations using such information. Specifically, we should expose each memory object's size and lifetime to hardware and implement an efficient detection mechanism for illegal accesses. To protect the entire memory space, the distinct allocation method and lifetime of each memory type should be carefully addressed. We also need to devise how to maintain metadata and enforce fine-grained safety at the sub-object granularity. %Most importantly, all software interfaces should be succinct in program code. Otherwise, the benefit of hardware supports would be overwhelmed by the instruction overhead.

\noindent
\textbf{How to minimize slowdown by security checks.}
%\subsubsection{How to minimize slowdown by security checks?}
To enhance the security level of systems, security-check statements are typically defined and inserted in programs based on the targeted threat model and security coverage. However, given that security checks are always needless, in terms of the correctness of program execution, excessive check operations can cause a significant slowdown, which is unacceptable in most cases. To minimize the slowdown, it is important to define a threat model built upon sophisticated attack models and apply a minimally required set of security checks to sustain performance but not hamper security.

\noindent
\textbf{How to retain compatibility with legacy code.}
%\subsubsection{How to retain compatibility with legacy code?}
Preserving compatibility is important to be practical and deployable in commodity systems. For example, a solution loses source compatibility if it requires any manual source modification. Even minimal human intervention, such as code annotation and source-to-source translation,  may make a solution unscalable and impractical for a large software project. Binary compatibility is lost if instrumented binaries cannot run with legacy code, e.g., unmodified libraries. Given that system libraries are typically protected and unchangeable without high privileges, the binary incompatibility not only prevents incremental development but also limits the operating platforms.
}



==> Submitted/D.ThreatModel.tex <==
%-------------------------------------------------------------------------------
\section{Threat Model}
\label{s:threat}
%-------------------------------------------------------------------------------
In our threat model, attackers can exploit one or more memory bugs that may exist in the address space of a user process and thereby obtain arbitrary read and write capabilities to leak sensitive information or gain root permissions via privilege escalation. We do not limit the scope of memory regions; therefore, memory bugs can exist anywhere in a program, including stack, heap, and global memory regions. However, we assume that the payload, i.e., the attack vector for exploitation, is given through external inputs, such as user input and network. Hence, the inherently existing benign memory bugs in programs not controlled by users are considered unexploitable by attackers. Since we deem hardware components to be trustworthy, we leave out of scope hardware-oriented attacks, such as side-channel~\cite{primeprobe,flushreload,eddie,power_channel}, speculative execution~\cite{spectre,meltdown,foreshadow,zombieload}, and row-hammer attacks~\cite{row_hammer,RAMBleed,ECCploit,PThammer} and focus only on memory safety bugs.



==> Submitted/E.Overview.tex <==
%-------------------------------------------------------------------------------
\section{Overview}
\label{s:overview}
%-------------------------------------------------------------------------------

In this section, we overview the proposed full-system architecture for memory safety, namely \mech{}. To achieve robust yet practical memory safety, we identify four properties, which are essential but challenging to achieve altogether, and set those as target design goals. We introduce our approaches to each property below and then describe the workflow.

\noindent
\textbf{Security.} Although various novel mechanisms have been proposed, prior work tends to specialize in specific memory type protection, e.g., heap protection~\cite{AOS,C3,CHEx86}. To overcome this limitation, we propose a generalized method, called \textit{data-pointer tagging} (DPT), applicable to all memory types (\cref{ss:ensuring}).
%DPT uses a 16-bit cyclic redundancy check hash (CRC-16) as a pointer tag and 
%In this work, we investigate a generalized approach, called \textit{data-pointer tagging} (DPT). DPT generates a 16-bit cyclic redundancy check hash (CRC-16), used as a pointer tag, and stores the hash in the high-order bits of a pointer. DPT is applicable to protecting all memory types and ensuring fine-grained sub-object safety. Details are described in \fref{ss:ensuring}.

%We propose \textit{data-pointer tagging} (DPT) that generates a 16-bit cyclic redundancy check hash (CRC-16), used as a pointer tag, and stores the hash in the high-order bits of a pointer. As mentioned in \fref{ss:point-tag}, the pointer-tagging idea itself is not new. However, prior work tends to specialize in specific memory type protection, e.g., heap protection~\cite{AOS,C3}. In this work, we investigate a generalized approach applicable to protecting all memory types and ensuring fine-grained sub-object safety.

%Ensuring strong security guarantees is non-trivial even with a possible trade-off between performance and security. The primary challenge is how to properly maintain security metadata, e.g., memory objects' size and lifetime, and enable spatial and temporal security checks. In particular, many prior studies~\cite{AOS,C3,REST} do not guarantee sub-object safety, i.e., detecting intra-object overflow, while some studies~\cite{Califorms,No-FAT} support that at the cost of painful compatibility loss.

\noindent
\textbf{Compatibility.} Preserving compatibility is important to be deployable in commodity systems. Unlike fat pointer designs relying on an extended pointer size~\cite{CHERI,CHERIvoke,Cheri-concentrate,Cornucopia}, our proposed method, DPT, conforms to conventional programming models. Hence, instrumented programs can run with unmodified legacy code, i.e., binary compatibility is retained. Furthermore, in contrast to prior work, such as Califorms~\cite{Califorms} and No-Fat~\cite{No-FAT}, our compiler support requires neither source code modifications nor data structure changes. Thus, source compatibility is assured.

%We note that since we utilize the unused bits of a pointer, unlike fat pointer designs with a modified pointer size~\cite{CHERI,CHERIvoke,Cheri-concentrate,Cornucopia}, we conform to conventional language models. Hence, the instrumented programs can run with unmodified legacy code. Furthermore, unlike Califorms~\cite{Califorms} and No-Fat~\cite{No-FAT}, our compiler passes neither require source code modifications nor modify structure data types. Hence, we retain both source and binary compatibility.
%Source compatibility is lost if it requires any manual source modification, while binary compatibility is lost if instrumented binaries cannot run with legacy code. The lack of source compatibility may make a solution unscalable for a large software project, and a solution with binary incompatibility cannot run with unmodified user or system libraries.

\noindent
\textbf{Hardware.} Despite a number of novel architecture proposals for security~\cite{Cheri-concentrate,CHERI,CHERIvoke,Watchdog,Hardbound}, intrusive hardware changes required have often discouraged CPU vendors from adopting new proposals. For this reason, we decide to explore realistic and practical design space on top of the RISC-V BOOM processor~\cite{BOOM}. Based on the BOOM core, we investigate lightweight hardware extensions for DPT and propose a capability-execution pipeline seamlessly integrated with the existing memory pipeline (\cref{s:hardware}).
%Despite the performance gains achieved by architectural support for security, many prior studies~\cite{Cheri-concentrate,CHERI,CHERIvoke,Watchdog,Hardbound} end up with intrusive hardware changes, which may discourage CPU vendors from adopting the proposed features. On top of the open-source out-of-order RISC-V BOOM core~\cite{BOOM}, we prototype our design, \mech{}, and demonstrate full-system evaluations on FPGAs. Although \mech{} is prototyped based on the RISC-V architecture, we believe that the proposed hardware extensions are generally applicable to other commodity architectures, such as x86, AArch64, and IBM Power. 
%+ hardware overhead estimates
%Implementing architectural support for security can bring in a significant performance gain, as evidenced by many prior studies~\cite{Cheri-concentrate,CHERI,CHERIvoke,Watchdog,Hardbound}. However, such hardware schemes often require intrusive hardware changes and discourage CPU vendors from adopting the proposed features. For instance, despite their strong security guarantees, CHERI architectures are known to require non-trivial hardware complexity due to their fat-pointer and co-processor implementations, e.g., 32\% logic overhead~\cite{CHERI}.

\noindent
\textbf{Performance.} Sustaining high performance is crucial for a runtime solution. To do so, we dive into hardware design space and root-cause the sources of potential performance overheads. Based on our design analysis, we devise lightweight micro-architecture units (\cref{ss:cache} and \cref{ss:buffer}). Furthermore, we focus on a known security concept that memory safety vulnerabilities are typically exploited through untrusted external inputs~\cite{TaintCheck,scrash,perl}. Leveraging this, we show a use case of static taint analysis that helps identify vulnerable objects in a program and avoid redundant capability checks (\cref{ss:taint}).

\fref{fig:overview} shows the overview of the proposed workflow. To protect unsafe code against memory safety, we instrument the program by applying DPT which assigns capability metadata to memory objects existing in the program. The instrumented code is run on a custom hardware platform, i.e., \mech{}, where capability checks are accelerated with hardware support. Before applying DPT, static taint analysis can be optionally conducted to prune possibly redundant checks. %We discuss the trade-off between performance and security through the static analysis in \fref{ss:taint}.

%Extending security coverage typically results in performance loss due to the increased security metadata and checks. 
%\noindent
%\textbf{Performance.} Reducing a performance overhead is crucial for a runtime detection solution. For this reason, most software tools tend~\cite{asan,PhASAR,BaggyBounds,Softbound} to be used only for testing and debugging and fail to be deployed at runtime. On the other hand, hardware mechanisms reduce the performance overhead but often compromise security assurance or compatibility.

%In this paper, we investigate a multidisciplinary approach encompassing architecture, compiler, and system designs and build a capability architecture that supports full memory safety, including, spatial, temporal, and sub-object safety. On top of the open-source out-of-order RISC-V BOOM core~\cite{BOOM}, we prototype our design, \mech{}, and demonstrate full-system evaluations on FPGAs. Although \mech{} is prototyped based on the RISC-V architecture, we believe that the proposed hardware extensions are generally applicable to other commodity architectures, such as x86, AArch64, and IBM Power. Below, we brief our approaches and overview the workflow of \mech{}.

%discuss how we address the existing challenges in memory safety and briefly overview the workflow of \mech{}.

%In this paper, we propose \mname{}, a full-system level RISC-V architecture ensuring full memory safety, including spatial, temporal, and sub-object safety. Although \mech{} is prototyped on top of the open-source out-of-order BOOM core~\cite{BOOM} for real demonstration, we believe that the hardware extensions are generally applicable to other commodity architectures, such as x86, AArch64, and IBM Power.
%By addressing all the challenges discussed in \fref{ss:challenge}, \mname{} aims to be a robust yet practical security solution deployable on commodity systems.
\ignore{
\noindent
\textbf{Achieving full memory safety.} We propose \textit{data-pointer tagging (DPT)} that generates a 16-bit cyclic redundancy check hash (CRC-16), used as a pointer tag, and stores the hash in the high-order bits of a pointer. As mentioned in \fref{ss:point-tag}, the pointer-tagging idea itself is not new. However, prior work tends to specialize in specific memory type protection, e.g., heap protection~\cite{AOS,C3}. In this work, we investigate a generalized approach that is applicable to protecting all memory types and ensuring fine-grained sub-object safety in synergy with our custom hardware support.

%the way of generalized compiler support applicable to all memory types in the LLVM compiler framework. For stack and global variables that might not have explicit pointers to themselves, we utilize the concept of a \textit{shadow pointer}. For fine-grained safety, we present \textit{dynamic pointer mutation}. Details are presented in \fref{ss:ensuring}.
%cooperation with
%Like AOS, we generate a PAC using the Arm pointer authentication (PA) primitives~\cite{armpa} and use it as a pointer tag. On top of the AOS's hardware platform, we introduce slight hardware changes to adapt \mech{}'s stronger security policies. To protect all memory types, including stack, heap, and global memory, we introduce the concept of a \textit{shadow pointer}. Moreover, we enforce fine-grained safety via \textit{dynamic pointer mutation}. Details are presented in \fref{ss:ensuring}.

\noindent
\textbf{Maintaining compatibility with legacy code.} Since we utilize the unused bits of a pointer, unlike fat pointer designs with a modified pointer size~\cite{CHERI,CHERIvoke,Cheri-concentrate,Cornucopia}, we conform to conventional language models. Hence, the instrumented programs can run with unmodified legacy code. Also, our compiler passes are designed at the LLVM intermediate representation (IR) level without source modifications. Therefore, we retain both source and binary compatibility.

\noindent
\textbf{Pruning unnecessary security checks.} Extending security coverage results in performance loss due to the increased security metadata and checks. To optimize performance, we rely on the known security concept that memory safety vulnerabilities are typically exploited through untrusted external inputs~\cite{TaintCheck,scrash,perl}. To leverage this concept, we design static taint analysis, which helps identify vulnerable objects in a program and avoid unnecessary operations for untainted (safe) objects. We present more details in \fref{ss:taint}.
}


%we optionally perform static taint analysis to identify security-critical objects. Then, we assign capability metadata memory objects that exist in a program by applying DPT. The instrumented code is run on a custom hardware platform where security operations are accelerated with architectural support.
%identify security-critical objects and apply selective DPT to the identified vulnerable objects. The instrumented code is run on a custom hardware platform where security operations are accelerated with architectural support. %In the following section, we overview the hardware platform and present the proposed compiler techniques.

%\subsection{Capability Checks via Data-Pointer Tagging}



\ignore{
\subsection{Design Changes in \mech{}}
\label{ss:hardware_extension}

Compared to AOS, we make the following design changes in \mech{}. First, we create an 18-bit PAC as a pointer tag, whereas AOS generates 16-bit PAC and 2-bit AHC. In AOS, AHC (Address Hashing Code) is used to calculate an address hash used to look-up the BWB and to determine if a pointer has been signed. Note that while AOS's protection is limited to heap regions, \mech{} protects all memory types. Hence, \mech{} needs to sign and manage more data pointers, leading to more PAC collisions. Our empirical studies find that the benefit of using longer PACs is greater than that of using AHCs when non-trivial PAC collisions occur. Without using AHCs, \mname{} ensures that the \cc{pacma} always generates a nonzero PAC and determines a pointer's \textit{signess} by checking if its PAC is zero or not. Second, we introduce a new instruction, \cc{bndsrch}, to enable practical sub-object safety. In \fref{sss:protection}, we present the details on when and how the \cc{bndsrch} is used.

\vspace{1pt}
\begin{compactitem}[$\bullet$]
    \item \textbf{\cc{bndsrch ptr, size}}. The \cc{bndsrch} calculates bounds using a pointer address (\cc{ptr}) and a size and then finds the same bounds in the location indexed by the PAC of the \cc{ptr} in an HBT. If found, it returns 1 (\cc{true}), and otherwise 0 (\cc{false}).
\end{compactitem}
\vspace{1pt}
}


==> Submitted/F.Compiler.tex <==
%-------------------------------------------------------------------------------
\section{Compiler Support}
\label{ss:ensuring}
%-------------------------------------------------------------------------------

In this section, we first study the distinct allocation method and lifetime of each memory type and understand how and during which period we protect each type. Based on this, we develop a generalized pointer-tagging method, DPT. We conduct our study and design new passes at the intermediate representation (IR) level in the LLVM compiler framework~\cite{LLVM} since its language-agnostic characteristic makes many optimization and transformation techniques independent of source languages and target architectures. 

%in the LLVM compiler framework~\cite{LLVM}. As a language-agnostic intermediate representation (IR), LLVM IR 

\subsection{Object Allocation Methods and Lifetime}

\label{sss:allocation}
\fref{lst:alloc} shows memory allocation methods in LLVM IR.

\begin{figure}
\begin{lstlisting}[language=c++, style=mystyle3, escapechar=!]
@glbObj = common hidden !\color{codered}{global}! [100 x i8] ...
define hidden i32 @main() #0 {
entry:
  %stackObj = !\color{codered}{alloca}! [100 x 8], align 1
  %heapPtr = !\color{codered}{alloca}! i8*, align 8
  %call = !\color{codered}{call}! noalias i8* @!\color{codered}{malloc}!(i64 100) #2
  store i8* %call, i8** %heapPtr, align 8
  %0 = load i8*, i8** %heapPtr, align 8
  !\color{codered}{call}! !\color{black}{void}! @!\color{codered}{free}!(i8* %0) #2 ...
\end{lstlisting}
%\vspace{0.2cm}
%\centering \small (b) LLVM IR code example.
\caption{Memory allocation methods in LLVM IR.}
\label{lst:alloc}
\end{figure}

\noindent
\textbf{Stack object.} With type information, a stack object is declared using an \cc{alloca} instruction (see line 4). Its memory region is allocated on the stack frame upon the function call and is released when the function returns to its caller.

\noindent
\textbf{Heap object.} With a size argument, heap objects are declared using dynamic allocation functions, such as \cc{malloc()} (see line 6). In LLVM IR, the integer pointer type (\cc{i8*}) is always returned from an allocation function and is cast to the object type to use. The allocated objects are valid until being freed using library functions, such as \cc{free()} (see line 9).

\noindent
\textbf{Global object.} With a \cc{global} or \cc{constant} qualifier, global objects are declared with an explicit type in the global scope (see line 1). Once a program starts, those are initialized and alive until the program ends.

Despite the various allocation methods, the size of each object to allocate is explicitly provided; for stack and global objects, the size can be calculated using the type information based on a given data layout. This indicates that LLVM IR preserves enough information to maintain the exact bounds of memory objects of any type.

\subsection{ISA Extensions} \label{ss:isa_extensions}
To allow for DPT, we introduce new instruction types that share the basic mechanism with the prior work~\cite{AOS}. However, as we base our design on the RISC-V architecture, we extend the RV64I base integer instruction set~\cite{RISC-V-ISA} and adapt their operations to our new architecture explained in \fref{s:hardware}.

%for pointer-tagging and capability management purposes. Since we base our design on the RISC-V architecture as mentioned in \fref{s:overview}, we extend the RV64I base integer instruction set~\cite{RISC-V-ISA} with the following instructions.

\begin{compactitem}[$\bullet$]
    \item \textbf{\cc{tagd rd, rs1}}: takes as input a pointer address (\cc{rs1}) and and calculates a CRC-16 hash using the given input. It places the generated hash, used as a pointer tag, in the upper bits of the pointer and returns a tagged pointer address (\cc{rd}).
    
    %XORs a pointer address (\cc{rs1}) and a stack pointer (\cc{rs2}) and calculates a CRC-16 hash of the XORed value. It stores the hash, used as a pointer tag, in the upper bits of the pointer and returns a tagged pointer address (\cc{rd}).
    %is used to \textit{tag} a data pointer. Using the CRC16, it calculates a PAC using a pointer address (\cc{ptr}), a modifier~\footnote{A modifier is a 64-bit tweak to differentiate contexts of a program.} (\cc{mod}), and a PA key.\footnote{New PA keys invisible to user are assigned to each new process.} The PAC is stored in the upper bits of the \cc{ptr}.
    
    \item \textbf{\cc{xtag rd, rs1}}: takes as input a tagged pointer address (\cc{rs1}) and zeros its tag. It returns a stripped pointer address (\cc{rd}).
    
    %. The \cc{xpacm} \textit{strips} a pointer to remove the PAC located in the upper bits of the pointer (\cc{ptr}).
    
    \item \textbf{\cc{cstr rs1, rs2}}: takes as input a tagged pointer address (\cc{rs1}) and a size (\cc{rs}). It calculates capability metadata for the pointer and stores it in a capability metadata table (CMT).
    
    %a compressed 8-byte capability metadata using a base address of a pointer (\cc{rs1}) and its size (\cc{rs2}) and stores the metadata in the location indexed by the tag of the pointer.
    %The \cc{bndstr} calculates bounds using a pointer (\cc{ptr}) and a size and stores the bounds in the location indexed by the PAC of the \cc{ptr} in an HBT.
    
    \item \textbf{\cc{cclr rs1}}: takes a tagged pointer address (\cc{rs1}) and clears its corresponding capability metadata stored in a CMT.
    %stores a zero value in the location indexed by the tag of a pointer (\cc{rs1}).
    %. The \cc{bndclr} clears bounds from the location indexed by the PAC of a pointer (\cc{ptr}) in an
    \ignore{
    \item \textbf{\cc{csrch rs1, rs2}}: takes a tagged pointer address (\cc{rs1}) and a size (\cc{rs2}). It calculates capability metadata using the given inputs and searches for the metadata in a CMT. If the same metadata are found, it returns one, otherwise zero.
    }
    %calculates a compressed 8-byte capability metadata using a base address of a pointer (\cc{rs1}) and its size (\cc{rs2}) and searches for the metadta in the location indxed by the tag of the pointer. If found, it returns 1, otherwise 0.
    %The \cc{bndclr} clears bounds from the location indexed by the PAC of a pointer (\cc{ptr}) in anHBT.
\end{compactitem}

\vspace{5pt}

In \mech{}, capability metadata may hold memory capabilities, such as upper and lower bounds and read, write, and execute permissions, as in typical capability architectures~\cite{CHERI,Cheri-concentrate,CHERIvoke,Cornucopia}. However, we note that the baseline BOOM core only supports 8-byte wide data-fetch width for cache accesses whereas modern architectures support up to 64-byte wide width. Given such a limitation, we decide to maintain 8-byte capability metadata for each object, which contain bounds information as an encrypted format~\cite{AOS}. Once wider data-fetch width is supported, the same mechanism proposed in \mech{} can be used to enforce more various memory capabilities. We leave this as our future work.

\begin{figure}[t]
\begin{lstlisting}[language=c++, style=mystyle3, escapechar=!]
  char stackObj[SIZE];        // Stack obj alloc
!\colorbox{gray!20}{\ \ \color{codered}{char} \color{black}{*shadowPtr = \&stackObj;}\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }!
!\colorbox{gray!20}{\ \ \color{codeblue}{tagd} \color{black}{shadowPtr;}\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }!
!\colorbox{gray!20}{\ \ \color{codeblue}{cstr} \color{black}{shadowPtr, SIZE;}\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }!
!\colorbox{gray!20}{\ \  shadowPtr[0] = 10;\ \ \ \ \ \ \ \ \ \ \ \ \ \ \color{codegreen}{// stackObj[0] = 10;}\ \ \ \ \ \ \ \ }!
!\colorbox{gray!20}{\ \ \color{codeblue}{cclr} \color{black}{(shadowPtr);} \ \ \ \ \ \ \ \ \ \ \ \ \ \ \color{codegreen}{// Release bounds} \ \ \ \ \ \ \ \ \ \ }!
\end{lstlisting}

\vspace{0.2cm}
\centering \small (a) Stack object protection.

\begin{lstlisting}[language=c++, style=mystyle3, escapechar=!]
  char *heapPtr=(char*)malloc(SIZE); // Heap obj alloc
!\colorbox{gray!20}{\ \ \color{codeblue}{tagd} \color{black}{heapPtr;}\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }!
!\colorbox{gray!20}{\ \ \color{codeblue}{cstr} \color{black}{heapPtr;}\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }!
  heap_ptr[0] = 10;
!\colorbox{gray!20}{\ \ \color{codeblue}{cclr} \color{black}{(heapPtr);} \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \color{codegreen}{// Release bounds} \ \ \ \ \ \ \ \ \ \ }!
!\colorbox{gray!20}{\ \ \color{codeblue}{xtag} \color{black}{heapPtr;}\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }!
  free(heapPtr);
\end{lstlisting}

\vspace{0.2cm}
\centering \small (b) Heap object protection.
\label{lst:heap}

\begin{lstlisting}[language=c++, style=mystyle3, escapechar=!]
char glbObj[SIZE];        // Global obj alloc
void foo() {
!\colorbox{gray!20}{\ \ \color{codered}{char} \color{black}{*shadowPtr = \&glbObj;}\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }!
!\colorbox{gray!20}{\ \ \color{codeblue}{tagd} \color{black}{shadowPtr;}\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }!
!\colorbox{gray!20}{\ \ shadowPtr[0] = 10;\ \ \ \ \ \ \ \ \ \color{codegreen}{// glbObj[0] = 10;}\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }!
}
int main(void) {
!\colorbox{gray!20}{\ \ \color{codered}{char} \color{black}{*shadowPtr = \&glbObj;}\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }!
!\colorbox{gray!20}{\ \ \color{codeblue}{tagd} \color{black}{shadowPtr;}\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }!
!\colorbox{gray!20}{\ \ \color{codeblue}{cstr} \color{black}{shadowPtr, SIZE;}\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }!
  ... }
\end{lstlisting}

\vspace{0.2cm}
\centering \small (c) Global object protection.
\label{lst:global}
\caption{Memory object protection using DPT.}
\label{fig:dps}
\end{figure}

\begin{figure*}[t]
\centering
\includegraphics[width=2.1\columnwidth]{Fig/pipeline.pdf}
\caption{Overview of hardware modifications in \mech{}.}
\label{fig:rv_cure}
\end{figure*}

\subsection{Data-Pointer Tagging (DPT)}
\label{sss:protection}
With the extended ISA, we develop DPT that assigns capability metadata, maintained in the CMT in memory, upon object allocation and releases the assigned metadata upon deallocation. During the object's lifetime, memory accesses by its tagged pointer are validated by capability checks. When the object is deallocated, its capability metadata are cleared from the CMT. Note that all dangling pointers to the deallocated object remain tagged, so subsequent accesses using those pointers will trigger capability-check failures.

To associate a pointer with its capability metadata, DPT tags the pointer using a \cc{tagd} instruction that embeds its pointer tag (CRC-16) in the pointer address. DPT then uses a \cc{cstr} instruction to calculate and store its capability metadata in the location indexed by its pointer tag in the CMT, i.e., \cc{CMT[tag]}. In addition, a \cc{cclr} instruction is used to clear a pointer's metadata from the CMT, and a \cc{xtag} instruction is used to remove a pointer tag in a pointer address.

Since the pointer tag size is limited, hash collisions can happen across pointers sharing the same tag. To handle such collisions, from the prior work~\cite{AOS}, we adopt the multi-way structure for the CMT that accommodates multiple capability metadata for each tag value. With the multi-way structure, we allow capability checks to iterate over multiple ways until valid metadata are found. We detail such operations with hardware extensions in \fref{cap_exec_pipe}. 

As explained, DPT deals with a pointer. However, we note that stack and global objects may not have a pointer pointing to themselves while heap objects always have explicit pointers. To protect these types, we create a shadow pointer, which is not present in program code but is inserted at compile time, and have any access to the object done via dereferencing the pointer, i.e., \cc{replaceAllUsesWith()} in LLVM. We detail our approach for each memory type below.

%we insert \textit{shadow pointers} for stack and global objects, which are not present in a program but are inserted at compile time. use a \textit{shadow pointer} mechanism for stack and global objects, where a shadow pointer is not present in program code but is inserted at compile time. For each stack and global object we want to protect, we create a shadow pointer, associate the object's bounds with the pointer, and have any access to the object done via dereferencing the pointer, i.e., \cc{replaceAllUsesWith()} in LLVM.

%Since array and struct types are most prone to memory bugs caused by incorrect indices~\cite{Califorms}, we only care about stack and global objects of such types. Note that all data pointers pointing to protected stack and global variables will get assigned tagged addresses since we tag and propagate addresses immediately after allocations. However, in the case of dynamic allocation, allocated types are often ambiguous, so we tag all heap pointers. When tagging, we use an encoded 64-bit type identifier as a modifier, i.e., \cc{cstr ptr, type}, as in the prior work~\cite{pacitup}, to ensure that we obtain the same tag using the same address with the same type.

%orthogonal (agnostic) to code pointer protection schemes.
%In addition, code pointers, such as a function pointer, can be protected by the existing PA solutions (see \fref{ss:pointer_integrity}). 



\noindent
\textbf{Stack object protection.}
We create a shadow pointer and associate an object's capability metadata with it (see lines 3-5 in \fref{fig:dps}a). Then, we have any memory access to the object done via the tagged pointer's dereferencing (see line 6 in \fref{fig:dps}a). The capability metadata are released right before the function returns (see line 7 in \fref{fig:dps}a). %We defer the detailed description on  to the point where we discuss intra-object protection in the next section.%Note that \cc{\_\_xtag\_ptr\_stack()} is inserted to clear its metadata. We defer the detailed description to the point where we discuss intra-object protection in the next section.

%Since we sign the pointer and replace all uses of the pointer at the root of its data flow,
%the pointer propagation **** automatically happens without any overhead.

\noindent
\textbf{Heap object protection.}
Dynamic memory allocation methods always return an integer pointer type (\cc{i8*}). Hence, we tag a returned pointer and store its capability metadata right after the allocation (see lines 2-3 in \fref{fig:dps}b). Its metadata are released right before the heap object is deallocated (see lines 5-6 in \fref{fig:dps}b). The \cc{xtag} is inserted to remove the pointer's tag to avoid capability checks during \cc{free()}.

%Like stack objects, the pointer propagation automatically happens...

\noindent
\textbf{Global object protection.}
In a program entry, e.g., \cc{main()}, we create a (local) shadow pointer and associate each global object's capability metadata with it (see lines 8-10 in \fref{fig:dps}c). Since global objects are accessible anywhere, we also create shadow pointers in each function where global objects are used (see lines 3-4 in \fref{fig:dps}c). However, we store the metadata only in the program entry to avoid storing the same metadata multiple times. We do not release metadata because global objects are alive throughout the entire program execution.


%linked_list = STT[getPAC(objPtr)];
%  !\color{codered}{foreach}! list in linked_list:
%    if list->ptr == subObjPtr:
%      !\textit{Set list as a head list}!;
\ignore{
\subsection{Dynamic Pointer Mutation}
\label{ss:dynamic_pointer_mutation}

While the proposed DPT method becomes a common approach to protecting all memory types, its guarantee is limited to inter-object protection. Pursuing extended coverage up to fine-grained, intra-object protection, one straightforward intuition can be that if we create a new pair of a pointer tag and narrowed capability for a sub-object and associate the pair with the sub-object, we could enforce fine-grained checks. At this point, two questions arise; 1) how to distinguish sub-objects and assign new pointer tags? and 2) how and when to assign and release narrowed bounds for sub-objects?
%Although more fine-grained protection is required to prevent intra-object overflows, achieving sub-object safety is not trivial, as evidenced by many prior studies suffering from performance or compatibility issues. %Below, we discuss challenges we encounter and present our approach to such challenges.

To answer the first question, we note that in LLVM IR, a \cc{GEP} instruction is used to index a sub-object from an object. This allows us to detect each sub-object indexing by looking for \cc{GEP} instructions. However, the \cc{GEP} instruction calculates the address of the indexed sub-object simply by adding an offset to its base address, and as a result, the sub-object inherits the same pointer tag from the parent object. To differentiate sub-objects and associate unique capability, we choose to re-tag (mutate) pointers returned by \cc{GEP}s to generate different tags.


\begin{figure}[t]
\begin{lstlisting}[language=c++, style=mystyle3, escapechar=!]
// Typedef of struct S is borrowed from Fig 1
void *mallocWrapper(size_t size) {
  void *ptr = malloc(size);
  // Craft custom data structures, etc.
  return ptr;
}
void foo() {
  int *intPtr = mallocWrapper(sizeof(int));
  struct S *strPtr = mallocWrapper(sizeof(struct S));
  strPtr->ovfArr[0] = 'a';
  bar(strPtr); ...
}
void bar(struct S* strPtr) {
  strPtr->ovfArr[1] = 'b'; ...
}
\end{lstlisting}
\caption{Ambiguous type information upon \cc{malloc()}.}
\label{fig:malloc_wrapper}
\end{figure}

\begin{figure}[t]
\begin{lstlisting}[language=c++, style=mystyle3, escapechar=!]
typedef struct stt_node {
  void *ptr;
  struct stt_node *next;
} stt_node;
stt_node *STT[SIZE];    // SIZE is 2^(TAG_SIZE)

void *!\textbf{\_\_dpt\_mutate}!(objPtr, subObjPtr, size, type):
  !\color{codeblue}{tagd}! subObjPtr, type;
  !\color{codeblue}{csrch}! subObjPtr, type;
  if !\color{codeblue}{csrch}! !\textit{returns}! 1:
    return subObjPtr;
  !\color{codeblue}{cstr}! subObjPtr, size; // Store metadata in CMT
  linked_list = STT[getTag(objPtr)];
  !\textit{Create a list with subObjPtr and set as a head list}!;
  return subObjPtr;

void !\textbf{\_\_dpt\_clear}!(ptr, lowBnd, uppBnd):
  !\color{codeblue}{cclr}! ptr;
  !\color{codeblue}{xtag}! ptr;
  linked_list = STT[geTag(ptr)];
  !\color{codered}{foreach}! list in linked_list:
    if lowBnd <= list->ptr <= uppBnd:
      !\textbf{\_\_dpt\_bndclr\_recur}!(list->ptr, lowBnd, uppBnd);
      !\textit{Remove list from linked\_list;}!
  return;
  
void !\textbf{\_\_dpt\_clear}!(objPtr, size):
  lowBnd = !\color{codeblue}{xpacm}!(objPtr);
  uppBnd = lowBnd+size;
  !\textbf{\_\_dpt\_clear\_recur}!(objPtr, lowBnd, uppBnd);
  return;
\end{lstlisting}
\caption{Sub-object tracing collector library functions.}
\label{fig:utility}
\end{figure}

Regarding the second question, one possible approach would be to store the capability metadata of all sub-objects at the time of object allocation and clear all the metadata at the time of deallocation. However, we observe that such a static de-/allocation method could be viable for stack and global objects but not for heap objects. This is because dynamic memory de-/allocation methods often have ambiguous types\footnote{Prior LLVM analysis supports runtime type checking for \cc{malloc()}, but the method incurs a runtime overhead and has limited coverage~\cite{llvmtypegithub}.}, and this makes it hard to determine sub-object's bounds at the time of object allocation. \fref{fig:malloc_wrapper} shows an example of \cc{malloc()} wrapper function usage, which can be found in several SPEC workloads, e.g., \cc{povray\_r/s}. In this example, the wrapper function allocates a memory region with a given size without knowing its type, and allocated objects' types are determined at call sites, i.e., outside the wrapper function.

With this observation, we choose to (dynamically) assign sub-object metadata when sub-objects are indexed using \cc{GEP}s. We call this method \textit{dynamic pointer mutation}. Note that \cc{GEP}s provide sub-objects' types based on the static data-type layout, and this allows calculating the size of indexed sub-objects using the known data type. However, one challenging point is that the same sub-object can be indexed multiple times in different locations (see lines 10 and 14 in \fref{fig:malloc_wrapper}). Hence, not to keep creating duplicates of the same metadata, we need to keep track of metadata allocations for sub-objects and allocate new ones only when needed. Such behaviors remind us of garbage collectors (GCs) that trace the allocation and release of memory using a defined data structure, e.g., a linked list, and reclaim unused memory at runtime. Motivated by the GCs, we design a sub-object tracing collector that enables precise and efficient sub-object metadata management.

%and provides the sub-object’s type based on the static data-type layout. This allows us to detect each sub-object indexing by looking for GEP instructions and then calculate the size of indexed sub-objects using the known data type. However, we note that the GEP instruction calculates the address of the indexed sub-object simply by adding an offset to its base address, and as a result, the sub-object inherits the same pointer tag, i.e., PAC, from the parent object. To differentiate sub-objects and associate unique bounds, we re-sign (mutate) the pointer returned by a GEP instruction to generate a different PAC

%To answer the first question,  One possible approach would be to store the bounds of all sub-objects at the time of object allocation and clear all the bounds at the time of deallocation. However, we observe that such a static de-/allocation method could be viable for stack and global objects but not for heap objects. This is because dynamic memory de-/allocation methods often have ambiguous type information\footnote{Prior LLVM analysis supports runtime type checking for \cc{malloc()}, but the method incurs a runtime overhead and has limited coverage~\cite{llvmtypegithub}.}, and this makes it hard to assign sub-object bounds at the site of an object allocation.

%However, achieving sub-object safety is non-trivial as evidenced by many prior studies suffering from performance or compatibility issues. Below, we discuss challenges we counter when we are to enable fine-grained protection via data-pointer signing 

%During our investigation, we note that dynamic memory allocation often has ambiguous type information\footnote{Prior LLVM analysis supports runtime type checking for \cc{malloc()}, but the method incurs a runtime overhead and has limited coverage~\cite{llvmtypegithub}.}, whereas static and global objects exhibit static type information. For example, a heap object can be allocated with a constant size and be cast to a different type later before use. This makes it hard to assign (statically) sub-object bounds upon an object allocation.

%\textit{When to assign/release bounds?} One possible approach would be to store the bounds of all sub-objects at the time of object allocation and clear all the bounds at the time of deallocation. However, we observe that such a static de-/allocation method could be viable for stack and global objects but not for heap objects. This is because dynamic memory de-/allocation methods often have ambiguous type information\footnote{Prior LLVM analysis supports runtime type checking for \cc{malloc()}, but the method incurs a runtime overhead and has limited coverage~\cite{llvmtypegithub}.}, and this makes it hard to assign sub-object bounds at the site of an object allocation.

 %This is because dynamic de-/allocation methods only take the size, e.g., in \cc{malloc()} or the address to free, e.g., in \cc{free()}, and the type of objects is not explicitly represented.
%While this could be viable for stack and global objects, 

%\textit{When to assign/release bounds?} One possible approach would be to store the bounds of all sub-objects at the time of object allocation and clear all the bounds at the time of deallocation. While this could be viable for stack and global objects, the problem is the dynamic de-/allocation methods only take the size, e.g., in \cc{malloc()} or the address to free, e.g., in \cc{free()}, and the type of objects is not explicitly represented.\footnote{Prior LLVM analysis supports runtime type checking for \cc{malloc()}, but the method incurs a runtime overhead and has limited coverage~\cite{llvmtypegithub}.} This makes this approach infeasible since we cannot handle sub-objects without knowing the data-type layout.


%With this observation, we choose to (dynamically) assign sub-object bounds when \textit{sub-objects are indexed} from objects, e.g., \cc{str.ovfArr} and \cc{str.vulArr} in \fref{lst:example_code}  In LLVM IR, a \cc{getelementptr} (\cc{GEP}) instruction is used to index a sub-object from an object and provides the sub-object's type based on the static data-type layout. This allows us to detect each sub-object indexing by looking for \cc{GEP} instructions and then calculate the size of indexed sub-objects using the known data type. However, we note that the \cc{GEP} instruction calculates the address of the indexed sub-object simply by adding an offset to its base address, and as a result, the sub-object inherits the same pointer tag, i.e., PAC, from the parent object. To differentiate sub-objects and associate unique bounds, we re-sign (mutate) the pointer returned by a \cc{GEP} instruction to generate a different PAC and assign narrowed bounds metadata with the pointer. We call this method \textit{dynamic pointer mutation}.

%Sub-object indexing can occur multiple times, e.g., one struct variable can be accessed in different locations. To avoid unnecessary memory overhead, we should maintain the information about previous sub-object bounds allocations and decide if we need to allocate new ones or not. Such behaviors remind us of garbage collectors (GCs) that trace the allocation and release of memory using a defined data structure, e.g., linked list, and reclaim unused memory at runtime. Motivated by the GCs, we design a sub-object tracing collector that enables precise and efficient sub-object bounds management. We present more details below.

\noindent
\textbf{Intra-object protection.} Typical GCs implement a linked list to maintain memory reference information. However, in our evaluation, such an approach is shown to impose an intolerable slowdown (up to $\sim$3x) as typical GCs do. Not to be overwhelmed by the overhead, we propose the use of a new \cc{csrch} instruction (see \fref{ss:isa_extensions}). Having a similar mechanism as the \cc{cstr} and \cc{cclr}, the \cc{csrch} takes the address and size of an indexed sub-object, accesses the location indexed by the mutated pointer's tag in the CMT, and efficiently checks the existence of the metadata. The use of \cc{csrch} enables us to accomplish practical sub-object safety at a ?\% average slowdown (see \fref{s:eval}).

%However, we still see the need to keep track of sub-object indexing using a linked list. This is because when an object is deallocated, we need to know which sub-objects' bounds (derived from that object) need to be removed from the HBT.


%To accomplish efficient protection with retained compatibility, we choose to assign the bounds \textit{when sub-objects are indexed from objects}, e.g., \cc{str.arr}. In LLVM IR, a \cc{getelementptr} (\cc{GEP}) instruction is used to index a sub-object from an object and provides the sub-object's explicit type based on the static data-type layout. This allows us to detect the sub-object indexing by looking for \cc{GEP} instructions and then calculate the size of indexed sub-objects using the known data type. However, we note that the \cc{GEP} instruction calculates the address of the indexed sub-object simply by adding an offset to its base address, and as a result, the sub-object inherits the same pointer tag, i.e., PAC, from the object. 

%To distinguish sub-objects and associate unique bounds, we re-sign (mutate) the pointer returned by a \cc{GEP} instruction to generate a different PAC and assign narrowed bounds metadata with the pointer. We call this method \textit{dynamic pointer mutation}. However, sub-objects can be indexed from the same object multiple times, e.g., a struct variable can be accessed in different functions. Hence, if we store bounds whenever sub-objects are indexed, we would end up storing duplicates of the same bounds, resulting in severe memory overhead. 

%One native approach to avoiding the issue would be to maintain a linked list of sub-object addresses indexed at runtime. For a given sub-object address, then, it should be possible to check whether or not we have stored its bounds before by iterating over the linked list. However, such an approach is shown to impose an intolerable slowdown (up to $\sim$3x) in our evaluation. To reduce the overhead, we propose the use of a new \cc{bndsrch} instruction (see \fref{ss:hardware_extension}). Having a similar mechanism as the \cc{bndstr} and \cc{bndclr}, the \cc{bndsrch} takes the address and size of an indexed sub-object, accesses the location indexed by the mutated pointer's PAC in the HBT, and efficiently checks the existence of bounds. The use of \cc{bndsrch} enables us to accomplish practical sub-object safety at a 7\% average slowdown, as presented in \fref{s:eval}. However, we still see the need to keep track of sub-object indexing using a linked list. This is because when an object is deallocated, we need to know which sub-objects' bounds (derived from that object) need to be removed from the HBT.

With the \cc{csrch} implementation, we develop library functions for our sub-object tracing collector, as shown in \fref{fig:utility}. We then insert \cc{\_\_dpt\_mutate()} when a sub-object is indexed (see line 8 in \fref{fig:dps}d) and \cc{\_\_xtag\_ptr()} when deallocating an object (see line 7 in \fref{fig:dps}a and line 5 in \fref{fig:dps}b). With a sub-object tracing table (STT), declared in the global scope, we maintain the mapping information between objects and their sub-objects at runtime. The STT is indexed by a pointer tag, and each entry holds the head of a linked list for the corresponding tag. When a sub-object we want to protect is accessed, we first search for the sub-object's metadata in the CMT using a \cc{csrch} instruction. If the \cc{csrch} returns 1, we just return the tagged sub-object pointer. If not, we create a new node, log the connection between them, and add it to the linked list in the corresponding STT entry. Then, we store its metadata in the CMT and return the tagged pointer. Note that an inner structure in a nested structure, i.e., a sub-object of the outer structure, can be an object of its own sub-objects. The mapping of such a nested structure can be implicitly maintained in the STT, as shown in \fref{fig:stt}. 

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{Fig/mutate.pdf}
\caption{Sub-object tracing table (STT).}
\label{fig:stt}
\end{figure}

When an object is deallocated, we erase its mapping information in the STT. By iterating over the linked list corresponding to the object's tag, we look for a list of which pointer address points to the object's memory region. If found, we remove the list from the linked list. At this point, we recall that an inner structure of a nested structure can have its own sub-objects. To clear the traces of all derivative sub-objects, we recursively iterate over the linked list corresponding to the erased pointer's tag. Compared to \cc{\_\_dpt\_mutate()}, \cc{\_\_dpt\_clear()} is called one time for each deallocation, and thus its linked-list iteration overhead is not significant.
}

==> Submitted/G.Architecture.tex <==


%-------------------------------------------------------------------------------
\section{RV-CURE Architecture}
\label{s:hardware}
%-------------------------------------------------------------------------------

For optimal performance, \mech{} implements architecture support for DPT. To explore realistic design space, we set the RISC-V out-of-order BOOM processor as our baseline architecture. On top of the BOOM core, we investigate practical hardware extensions, build a synthesizable custom processor, and conduct full-system level evaluations. 

\fref{fig:rv_cure} illustrates the overview of our hardware modifications made on four pipeline stages; \textit{decode}, \textit{execute}, \textit{memory}, \textit{commit} stages. \ballwhite{1} In the decode stage, we detect memory instructions and tag them with additional one bit, namely \cc{needCC}. We use this to indicate that this instruction may perform a potentially unsafe memory access and therefore need to be validated via a capability check. \ballwhite{2} To enable capability checks required, in the memory stage, we implement a capability-execution pipeline responsible for capability metadata management and checks. \ballwhite{3} Next, we extend the re-order buffer (ROB) with one-bit entries holding \cc{needCC} bits. Using the extended bit, we ensure that memory instructions can commit after they are validated by capability checks and turn out to be safe. \ballwhite{4} Lastly, in the execute stage, we add a pointer-tagging unit for new instructions, i.e., \cc{tagd} and \cc{xtag}. We detail our changes as follows.

\subsection{Capability Enforcement}
\mech{} guarantees memory safety via strict capability enforcement in hardware. To achieve this, in the decode stage, we first distinguish potentially unsafe memory instructions, i.e., load and store, and set their \cc{needCC} bits to \cc{true(1)}. By default, the \cc{needCC} bit is set to \cc{false(0)} for other instructions. The identified instructions are propagated following the CPU pipeline and are required to be validated by capability checks. To further strengthen the security level, we extend the ROB with one-bit entries holding \cc{needCC} bits and append one more condition to the existing commit condition such that instructions can commit only when their \cc{needCC} bits are \cc{false(0)}. To support this, we extend the existing interface from the LSU to the ROB with signals for clearing \cc{needCC} bits asserted to high upon successful capability checks.

This new constraint enables a precise exception for capability faults, preventing illegal reads and writes from leaking or corrupting memory contents before capability faults are detected and handled. However, in the case where capability checks take longer than normal executions, this can result in delayed instruction retirement at the ROB, thereby degrading performance. For instance, REST~\cite{REST} reports a 23\% higher slowdown with its precise exception support. Notably, even with this strict policy, our evaluations show that \mech{} achieves a marginal runtime overhead (see \fref{ss:performance}).

\subsection{Capability Execution Pipeline}\label{cap_exec_pipe}
To enable efficient checks, we design a capability-execution pipeline integrated in parallel with the existing memory execution pipeline. As shown in \fref{fig:overview}, the capability-execution pipeline consists of shadow load and store queues (SLQ and SSQ, respectively), arbitration logics for capability load and store request generation, and comparison logics for capability checks. Being paired with a load queue (LQ) and a store queue (SQ), respectively, the SLQ and SSQ take incoming memory addresses, passed from the memory address calculation unit at the execute stage, and process them based on a finite-state machine (FSM) described below.

\begin{compactitem}[$\bullet$]
  \item \cc{S\_INIT.} Each queue entry starts with this state. If its corresponding memory address arrives, it checks if the address contains a nonzero pointer tag. If a nonzero tag is found, it transitions to the \cc{S\_READY}, otherwise to the \cc{S\_DONE}.
  \item \cc{S\_READY.} An entry in this state generates a capability load request to access its corresponding capability metadata stored in the CMT. Once the request is sent to the data cache (D-cache), it goes to the \cc{S\_WAIT}.
  \item \cc{S\_WAIT.} In this state, an entry waits until a cache response for a capability load arrives. Upon the response arrival, a capability check is performed. If the check passes, it asserts signals for clearing its \cc{needCC} bit sent to the ROB and transitions to the \cc{S\_DONE}. If not, it goes back to the \cc{S\_READY} to access the next way in the CMT.
  \item \cc{S\_DONE.} In this state, an entry waits until it is deallocated.
\end{compactitem}

Note that an instruction can generate multiple capability loads until it passes a capability check. As explained in \fref{sss:protection}, \mech{} maintains a set-associative structure for the CMT. To support such a structure, we implement hardware-based iteration performed over multiple ways in the CMT. For capability requests, a capability address is computed using the below equation, where \textit{Base} is the base address of the CMT, \textit{T} is a pointer tag, \textit{N} is the number of ways of the CMT, and \textit{W} is the way to access. \begin{align}
CapAddr = Base + (T << (3 + log_{2}N )) + (W << 3)
\end{align}
Besides memory instructions, the SSQ takes and handles new instructions for metadata management, i.e., \cc{cstr} and \cc{cclr}. Those follow the FSM in the same way only except that a \cc{cstr} iterates until empty space is found, and a \cc{cclr} iterates until the expected metadata to clear are found. In addition, they perform stores on the location where previous capability loads stopped before being deallocated in the \cc{S\_DONE} state.

In the pipeline, an instruction can end up with a failure after iterating over the entire ways in the CMT. This can happen either when illegal memory accesses are given, and no valid metadata are found or when frequent object allocations happen, and no empty space is found in the CMT. In these cases, capability faults are generated and handled by a new exception handler we introduce in \fref{s:runtime}. 

Notably, the hardware complexity we impose on the existing memory pipeline is low. For the capability execution, we only require new capability requests to be scheduled through the LSU scheduler responsible for arbitrating various memory request types. This indicates that past the LSU scheduler, capability requests will go through the existing path all the way to the D-cache without extra changes. We confirm its negligible impact in our RTL synthesis task by being able to synthesize our modified design at the highest clock frequency achievable by the baseline BOOM core.

However, sharing the execution path can impact performance since it causes hardware resource contentions between regular memory requests and capability requests. Note that all hardware components have limited input and output bandwidth. In our design analysis, we find three major contention points. First, at the input port of the LSU scheduler, capability requests can conflict with regular memory requests, preventing them from being scheduled at the same clock cycle. Second, in the translation lookaside buffer (TLB) where virtual-to-physical address translation happens, capability requests can miss and occupy miss status holding register (MSHR) entries. Given that the TLB cannot accept new requests while its MSHR entries are full, extra TLB misses caused by capability requests can stall the TLB unit until previous misses are resolved. Last, in a similar manner, capability requests can miss and occupy MSHR entries in the D-cache, causing stalls on the D-cache until cache misses are resolved.

To minimize performance impact due to such contentions, we take two approaches. First, we assign the lowest priority with capability requests at the LSU scheduler so that regular memory requests are always prioritized with an assumption that delayed capability checks would not affect normal program execution unless instruction commits at the ROB are not delayed. Second, we introduce small on-chip buffers that help minimize the number of capability requests. We explain more details in the following sections.

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{Fig/buffers.pdf}
\caption{Capability cache and store/clear head buffers.}
\label{fig:buffers}
\end{figure}


\subsection{Capability Cache} \label{ss:cache}
%[TODO] move the properties to evaluation section. we first focus on two properties of DPT; 1) although the CMT is maintained in memory space, its contents, i.e., capability metadata, are associated with pointer tags and 2) regardless of allocation size, only one set of capability metadata are assigned and shared across the entire allocated region. 
DPT assigns only one set of capability metadata regardless of allocation size. This property provides a high locality of capability metadata, and hence even a small storage can be very useful. Based on this, we introduce a capability cache (C-cache) indexed by a lower 8-bit tag, i.e., \cc{tag(7,0)}. The cache consists of a meta array holding a higher 8-bit tag, i.e., \cc{tag(15,8)}, and a data array holding 8-byte metadata, totaling a 2.25KB size. The entries of the C-cache are allocated either when a \cc{cstr} commits its store or when a capability check for a certain load/store succeeds. When a \cc{cclr} commits, it clears its corresponding entry in the C-cache. As shown in \fref{fig:buffers}, the C-cache is placed in parallel with the LSU scheduler and takes incoming memory addresses. If an incoming address contains a nonzero tag, it looks up the C-cache and decides its next state. If valid metadata satisfying its capability check is found, i.e., a C-cache hit occurs, it transitions to the \cc{s\_done} and signals the ROB to clear its \cc{needCC} bit. If not, it transitions to the \cc{s\_ready} state and goes through the capability-check procedure. The C-cache turns out to be extremely effective with a high hit rate, 96.68\%, for SPEC CPU 2017 benchmarks, as shown in Column 1 in \fref{tab:hit_iter}, meaning that only 3.32\% of tagged instructions generate extra capability requests.


\begin{table}[t]
%\small
\scriptsize
\centering
\caption{C-cache hit rates and average iterations numbers.}
\label{tab:taint_results}
\begin{tabular}{@{}lcrrrrr@{}}
    \toprule
    \multirow{2}{*}{\textbf{Name}}
        & \multicolumn{1}{c}{\textbf{C-Cache}}
        & \multicolumn{5}{c}{\textbf{Iteration Mode}} \\
    \cmidrule(lr){2-2}
    \cmidrule(lr){3-7}
    %\cmidrule(lr){6-7}
        & \textbf{Hit Rate (\%)} 
        & \textbf{Base} & \textbf{BWB} & \textbf{LAFD}
        & \textbf{FAFD} & \textbf{Adtv} \\
    \midrule
    \textbf{perlbench\_r}   & 92.71     & 1.16      & 1.12      & 1.01      & 1.08      & 1.07  \\
    %\textbf{gcc\_r}        & ?         & ?         & ?         & ?         & ?         & ?     \\
    \textbf{mcf\_r}         & 98.32     & 5.45      & 5.32      & 1.00      & 3.98      & 1.00     \\
    \textbf{namd\_r}        & 97.37     & 2.23      & 1.89      & 1.03      & 1.04      & 1.00     \\
    %\textbf{parest\_r}     & ??        & ?         & ?         & ?         & ?         & ?     \\
    %\textbf{povray\_r}     & ?         & ?         & ?         & ?         & ?         & ?     \\
    \textbf{lbm\_r}         & 99.99     & 1.00      & 1.00      & 1.00      & 1.00      & 1.00     \\
    %\textbf{omnetpp\_r}    & ?         & ?         & ?         & ?         & ?         & ?     \\
    \textbf{xalancbmk\_r}   & 89.02     & 22.30     & 17.03     & 2.16      & 10.14     & 1.92  \\
    \textbf{x264\_r}        & 94.88     & 1.08      & 1.00      & 1.00      & 1.07      & 1.00     \\
    %\textbf{blender\_r}    & ?         & ?         & ?         & ?         & ?         & ?     \\
    \textbf{deepsjeng\_r}   & 96.63     & 1.05      & 1.03      & 1.00      & 1.03      & 1.00     \\
    \textbf{imagick\_r}     & 98.54     & 1.00      & 1.00      & 1.00      & 1.00      & 1.00     \\
    %\textbf{leela\_r}      & ??        & ?         & ?         & 1         & 1.02      & 1     \\
    \textbf{nab\_r}         & 99.66     & 7.43      & 7.10      & 5.14      & 2.83      & 2.83  \\
    \textbf{xz\_r}          & 99.70     & 1.00      & 1.00      & 1.00      & 1.00      & 1.00     \\
    \midrule
    \textbf{Average}        & 96.68     & 4.37      & 3.75      & 1.53      & 2.42      & 1.28    \\
    %\textbf{Avg. Ratio}
    %    & \multicolumn{2}{c}{69.54\%}
    %    & \multicolumn{2}{c}{60.36\%}
    %    & \multicolumn{2}{c}{24.25\%} \\
    \bottomrule
\end{tabular}
\label{tab:hit_iter}
\end{table}


\subsection{Store/Clear Head Buffers} \label{ss:buffer}
As mentioned in \fref{cap_exec_pipe}, the multi-way structure of the CMT may require iterative accesses. To optimize the access pattern, we make an intuition that if we can maintain pointers pointing to empty locations for \cc{cstr}s and locations where metadata to clear are stored for \cc{cclr}s, their accesses will succeed at their first attempts. With such an intuition, we introduce store and clear head buffers, SHB and CHB in short, shown in \fref{fig:buffers}. These buffers have a simple array structure indexed by a partial pointer tag, i.e., \cc{tag(7,0)}, totaling a 0.625KB size. Each entry of the SHB stores a (likely) empty location for each partial tag, and each entry of the CHB stores a location where the metadata for the next \cc{cclr} are (likely) located. According to the C/C++ programming models, we come up with three possible iteration modes. Since capability metadata for global objects is allocated once and not deallocated during program execution, we focus on stack and heap objects. Below, we assume a situation when a \cc{cstr} or a \cc{cclr} finishes its iterative search in the \cc{N}-th way in the \cc{M}-way CMT.

\noindent
\textbf{LAFD (last-allocated, first-deallocated) mode.} Stack objects have a deterministic lifetime; when a callee function is called or returns, its stack objects are allocated or deallocated in a stack frame. Based on this observation, we make a \cc{cstr} update its corresponding SHB entry with \cc{(N+1)\%M} when it commits from the SSQ. When a \cc{cclr} commits, we make it update its corresponding CHB entry with \cc{(N-1)\%M}.

\noindent
\textbf{FAFD (first-allocated, first-deallocated) mode.} In contrast, the lifetime of heap objects are not deterministic. Hence, we assume that older memory objects will be freed earlier than younger objects. Based on this assumption, we make a \cc{cstr} update its SHB entry with \cc{(N+1)\%M} and a \cc{cclr} update its CHB entry with \cc{(N+1)\%M} when they commit from the SSQ.

\noindent
\textbf{Adaptive mode.} As a hybrid approach, an adaptive mode takes advantages of both modes. We note that stack memory space grows downward, and heap memory space grows upward in memory space. Based on this, if a memory address of a \cc{cstr} or \cc{cclr} belongs to the upper half of the memory space, the LAFD mode suitable for stack objects is used. Otherwise, the FAFD mode suitable for heap objects is used.

To evaluate the effectiveness of such modes, we run SPEC 2017 C/C++ workloads using reference inputs and measure the average number of iterations for each mode in Column 4-6 in \fref{tab:hit_iter}. Interestingly, the results allow us to categorize the evaluated workloads into three types. First, workloads that do not incur frequent memory allocations, e.g., \cc{lbm}, exhibit near-one average iteration numbers for both modes since there are almost zero hash collisions. Second, workloads that invoke frequent dynamic memory allocations, e.g., \cc{perlbench\_r}, \cc{mcf\_r}, and \cc{xalancbmk\_r}, have lower iteration numbers with the LAFD mode. Third, workloads that invoke frequent function calls leading to frequent stack object de-/allocations, e.g., \cc{nab\_r}, show lower iteration numbers with the FAFD mode. Notably, the adaptive mode shows the lowest iteration numbers in all workloads. Thus, we choose the adaptive mode as our default mode. For comparisons, we also report the results for the baseline mode (\cc{Base}) where an iteration always starts from the first way and the AOS's iteration mode (\cc{BWB}) in Columns 2 and 3 in \fref{tab:hit_iter},. The baseline mode presents 4.37 iterative accesses on average, justifying the need for optimization. The BWB mode shows 3.75 iterative accesses on average, worse than the results of all the LAFD, FAFD, and adaptive modes.

\subsection{Handling Tag Dependencies}
As we execute capability checks out of order, correct ordering between capability checks and stores sharing the same tag needs to be ensured to prevent false positives or negatives, i.e., tag dependencies matter. To handle memory dependencies for regular loads and stores, the BOOM core implements costly hardware logic that compares the memory address of a fired load with all stores older than the load and kills the load if any older store with the same address is found. Fence instructions can also be used to prevent the execution of following instructions younger than the current instruction at the cost of non-trivial pipeline stalls. As a balanced way, we take the approach of stalling capability checks of instructions until all capability stores older than themselves, regardless of their tag values, are committed from the SSQ. Despite such a conservative approach, the number of capability stores is much less than the number of memory instructions, and both hardware and performance overheads are shown to be trivial.

==> Submitted/H.Runtime.tex <==

\begin{table}[t]
    \centering
    \caption{New control and status registers in \mech{}.}
    %\begin{scriptsize}
    \begin{small}
    \begin{tabular}{@{}ll@{}}
    
    \toprule
    \textbf{Name}                        & \textbf{Description}                           \\
    \midrule
    enableDPT                   & Switch to turn on capability enforcement             \\
    baseAddrCMT                 & Base address of the CMT               \\
    numWaysCMT                  & Number of ways of the CMT             \\
    \bottomrule
    \end{tabular}
\label{tab:csrs}
\end{small}
\end{table}

\section{Runtime Support}\label{s:runtime}
To operate \mech{} in a real system, we add runtime support to the Linux kernel compatible with RISC-V. Our modifications consist of a new exception handler for capability faults, new control and status registers (CSRs) for hardware configurations, and new process fields for process management.

\noindent
\textbf{Capability fault handler.} To handle capability faults, we define a new exception handler that has a similar mechanism as a page fault handler. Upon a capability fault exception, the exception handler reads the \cc{cause} CSR and determines which instruction type triggered the exception. If a \cc{cstr} instruction turns out to be faulted, the kernel resizes the CMT by doubling its number of ways and rearranges capability metadata in the CMT. If a \cc{cclr} instruction faulted, this may indicate a temporal safety error, such as double free. If a load or store faulted, this indicates a capability-check failure. In the last two cases, errors are printed to users, and the execution resumes.

\noindent
\textbf{New CSRs.} To configure the CPU pipeline for \mech{}, we define new CSRs in the standard RISC-V ISA~\cite{RISC-V-ISA} as shown in \fref{tab:csrs}. The \cc{enableDPT} CSR is used as a switch to turn on the \mech{} mode. The \cc{baseAddrCMT} and \cc{numWaysCMT} CSRs hold the base address and the number of ways of a CMT, respectively. To interface with such CSRs, we add a custom system call, \cc{\_\_dpt\_set()}, that is inserted into a program entry at instrumentation time. In addition to those, we add extra CSRs for debugging and gathering runtime statistics.

%In the user-mode (U-mode) of the standard RISC-V ISA~\cite{RISC-V-ISA}, we define the new control and status registers (CSRs) (see \fref{tab:csr}). Specifically, the \cc{enableAOS} CSR is used to enable the hardware-based memory checks by \mech{}. The base address of an HBT is stored in the \cc{baseAddrOfHBT} CSR, and the associativity of an HBT is configured via the \cc{numWaysOfHBT} CSR. To interface with such CSRs, we provide a custom system call, namely \cc{\_\_aos\_set()}, that is inserted into the entry of a user program at compilation and sets the CSRs with given argument values. Besides to those CSRs for configuration, we also add extra CSRs to count the number of failures of bounds operations; \cc{numBndstrFails}, \cc{numBndclrFails}, and \cc{numBndchkFails}. After a program is terminated, the kernel reads and prints those CSRs to let a user know whether any bounds operation has failed during program execution.

\noindent
\textbf{New process fields.} Since all configurations we define above are process-specific, the kernel is required to keep track of each user process' information. To do so, we add new fields to the process structure, i.e., \cc{task\_struct}, that are initialized upon process creation and are set by our custom system call. Upon a context switch, the kernel saves the current process' configuration information into the new process fields if the current process is enabled for \mech{} and configures the CPU pipeline with the next process' configurations if the next process needs to be enabled for \mech{}.

%and configure the CPU pipeline with the next process' configurations upon a context switch. To do so, we add new fields to the process structure, i.e., \cc{task\_struct}, and let
%Besides the hardware configurations through our system call, the kernel needs to keep track of the information of each user process. To do so, we add new fields to the process structure in the Linux kernel, i.e., \cc{task\_struct}. Those fields are initialized upon process creation and are properly set by our custom system call. During a context switch, if the current process is enabled with \mech{}, the kernel saves its configuration information in the process structure, including the base address and the number of ways of an HBT assigned to the process. Then, the kernel checks whether the next process to execute is also enabled with \mech{}. If so, the kernel overwrites the CSRs with the configuration information of the next process before it begins its execution. Otherwise, the kernel initializes the CSRs with zero to disable AOS features for the next process.


==> Submitted/I.Pruning.tex <==
%-------------------------------------------------------------------------------
\section{DPT with Static Taint Analysis}
\label{ss:taint}
%-------------------------------------------------------------------------------

\begin{table}[t]
%\small
\scriptsize
\centering
\caption{Static taint analysis results on SPEC CPU 2017.}
\label{tab:taint_results}
\begin{tabular}{@{}lrrrrrr@{}}
    \toprule
    \multirow{2}{*}{\textbf{Name}}
        & \multicolumn{2}{c}{\textbf{Stack Objects}}
        & \multicolumn{2}{c}{\textbf{Heap Objects}} 
        & \multicolumn{2}{c}{\textbf{Global Objects}} \\
        
    \cmidrule(lr){2-3}
    \cmidrule(lr){4-5}
    \cmidrule(lr){6-7}
        & \textbf{\# Taint} & \textbf{\# Total}
        & \textbf{\# Taint} & \textbf{\# Total}
        & \textbf{\# Taint} & \textbf{\# Total} \\
    \midrule
    \textbf{perlbench\_r}   & 184       & 220       & 53        & 67     & 52     & 214     \\
    \textbf{gcc\_r}         & 1195      & 1660      & 80        & 90     & 374     & 894     \\
    \textbf{mcf\_r}         & 1         & 4         & 0         & 18    & 1     & 1    \\
    \textbf{namd\_r}        & 17        & 27        & 88        & 92   & 0     & 0     \\
    \textbf{parest\_r}      & 7135      & 8762      & 680       & 974   & 37     & 2215     \\
    \textbf{povray\_r}      & 949       & 993       & 52        & 69    & 19    & 158   \\
    \textbf{lbm\_r}         & 3         & 9         & 0         & 1    & 0    & 2    \\
    \textbf{omnetpp\_r}     & 1166      & 1515      & 243       & 834    & 146    & 819   \\
    \textbf{xalancbmk\_r}   & 828       & 920       & 16        & 31    & 208     & 2620     \\
    \textbf{x264\_r}        & 110       & 205       & 17        & 21     & 55     & 234     \\
    \textbf{blender\_r}     & 8026      & 8767      & 63        & 96    & 129     & 13659     \\
    \textbf{deepsjeng\_r}   & 23        & 36        & 1         & 1     & 59     & 77     \\
    \textbf{imagick\_r}     & 365       & 430       & 1         & 4    & 11     & 131     \\
    \textbf{leela\_r}       & 124       & 188       & 18        & 28    & 6     & 10     \\
    \textbf{nab\_r}         & 105       & 145       & 27        & 27    & 5     & 25     \\
    \textbf{xz\_r}          & 39        & 54        & 9         & 9    & 11     & 36     \\
    \midrule
    \textbf{Avg. Ratio}
        & \multicolumn{2}{c}{70.34\%}
        & \multicolumn{2}{c}{63.43\%}
        & \multicolumn{2}{c}{26.60\%} \\
    \bottomrule
\end{tabular}
\end{table}

Extending security coverage causes inevitable side-effects: the memory overhead by object-granular metadata and the execution overhead by extra security checks. To mitigate such overheads, we support static taint analysis that helps identify security-critical objects and remove unnecessary checks. Our LLVM optimizer passes consist of points-to analysis, taint analysis, and selective DPT passes.

%While our custom passes share basic mechanisms with other tools~\cite{llvmaa,drchecker}, we aim to design conservative analysis focused on high precision. Hence, we examine all possible data flows with the inter-procedural analysis and find the exhaustive alias sets. We then perform intentional over-tainting and identify objects that can be safely pruned for performance. Our analysis is flow-insensitive, context-insensitive, and field-sensitive.

%Many existing analysis tools~\cite{llvmaa,drchecker,points-andersen,points-steens} aim to provide a practically concise bug report and thereby make a trade-off between precision (high coverage with many false positives) and soundness (moderate coverage with all true positives). This is because a tool with a high false-positive rate may be disregarded by users even when its report contains true bugs~\cite{bessey-report}.

%For this reason, we decide to design new LLVM optimizer passes consisting of points-to analysis, taint analysis, and selective data-pointer signing passes. While our methods share basic mechanisms with other tools~\cite{llvmaa,drchecker}, we aim to design conservative analysis focused on high precision. Hence, we examine all possible data flows with the inter-procedural analysis and find the exhaustive alias sets. We then perform intentional over-tainting and identify objects that can be safely pruned for performance. Our analysis is flow-insensitive, context-insensitive, and field-sensitive.

%Below, we present three new LLVM optimizer passes, i.e., \mname{} points-to analysis, taint analysis, and selective data-pointer signing passes, and describe how they cooperate with the data-pointer signing scheme.

%In contrast to such tools for bug reporting purposes, our analysis methods aim to 
%Typical analysis tools~\cite{llvmaa,drchecker,points-andersen,points-steens} make a trade-off between precision, i.e., high coverage with many false positives, and soundness, i.e., moderate coverage with all true positives. This is because a tool with a high false-positive rate may be disregarded by users even when its report contains true bugs~\cite{bessey-report}. In contrast to such tools for bug reporting purposes, we aim to 
%designed to provide a practically concise bug report, our analysis method aims to only decide selective protection. This allows us to design conservative static analysis focused on high precision. Hence, we examine all possible data flows with the inter-procedural analysis and find the exhaustive alias sets. In this way, our analysis is flow-insensitive, context-insensitive, and field-sensitive.

\ignore{
\subsection{Terminology}
We define the terms we use to describe our method.

\begin{compactitem}[$\bullet$]
  \item A \textit{call graph (CG)} records the function call relationship in a program. A \textit{control-flow graph} (CFG) represents the control flow between \textit{basic blocks} (BBs), and each BB contains a sequence of instructions without any branch except for the exit. For program analysis, we obtain a CG using the existing \cc{CallGraphWrapper} pass and topologically sort each function's CFG using the Tarjan's algorithm~\cite{Tarjan72}. During our analysis, we iterate over instructions by traversing all BBs in functions.
  
  \item In LLVM, the \textit{value} class is the base class of all values, including instruction and function. LLVM constructs the \textit{def-use} and \textit{use-def} chains, where each value maintains a list of values using the particular value. For example, if \cc{value B} uses \cc{value A} as an operand, it becomes a \textit{user} of \cc{value A}. By iterating over the def-use chain, e.g., \cc{A->users()}, we keep track of the possible data flows of values.
\end{compactitem}
}

\ignore{
\begin{figure}[t]
\begin{lstlisting}[language=c++, style=mystyle3, escapechar=!]
visitSet = {}; // Init
void getPtrAlias(V): // V is a pointer value
  if V is found in visitSet: return;
  else: visitSet.insert(V);
    
  !\color{codered}{foreach}! U in V->users(): // U is a user of V
    if U is !\color{codeblue}{GEPInst}!:
      if a succ. node with same indices found:
        !\textit{Add U to alias set of succ. node}!;
      else:
        !\textit{Create new succ. node and add U to the node}!;
      getPtrAlias(U);
    !\color{codered}{elif}! U is !\color{codeblue}{BitCastInst}!:
      if a succ. node with same type found:
        !\textit{Add U to alias set of succ. node}!;
      else:
        !\textit{Create new succ. node and add U to the node}!;
      getPtrAlias(U);
    !\color{codered}{elif}! U is !\color{codeblue}{StoreInst}! or !\color{codeblue}{LoadInst}!:
      !\textit{Add valOp to alias set of ptrOp}!!\color{black}{'}!!\textit{s mem. node}!;
    !\color{codered}{elif}! U is !\color{codeblue}{CallInst}!:
      !\textit{Add argval to alias set}!;
      getPtrAlias(argval);
    !\color{codered}{elif}! U is !\color{codeblue}{ReturnInst}!:
      !\textit{Add U to alias set}!;
      !\color{codered}{foreach}! retval in call sites:
        !\textit{Add retval to alias set}!;
        getPtrAlias(retval);
  return

void pointsToAnalysis(M): // M is a module
  valueSet = {}; // Init
  !\color{codered}{foreach}! Inst in BBs,Funcs,CG:
    if Inst is !\color{codeblue}{AllocaInst}!:
      valueSet.insert(Inst);
    !\color{codered}{elif}! Inst is !\color{codeblue}{CallInst}!:
      if calledFunc is Dynamic alloc. func:
        valueSet.insert(Inst);
  !\color{codered}{foreach}! GV in M.getGlobalList(): // Global variable
    valueSet.insert(GV);
  !\color{codered}{foreach}! V in valueSet:
    !\textit{Create root node with value}!;
    getPtrAlias(V):
  return;
\end{lstlisting}
\caption{Algorithm of \mname{} points-to analysis.}
\label{fig:points_to}
\end{figure}
}

\noindent
\textbf{Points-to analysis.}
%\subsection{Points-To Analysis}
%\label{sss:points-to}
This analysis determines the set of pointers (aliases) that can ever point to the same object in memory. By traversing all basic blocks in a program, we first find the pointer values created by memory allocation methods, e.g., \cc{\%stackObj}, \cc{\%heapPtr}, and \cc{\%call} in \fref{fig:dps}c. Using \cc{getGlobalList()} in a given module, we also obtain a list of global variables, e.g., \cc{@glbObj} in \fref{fig:dps}c. We then create a root node for each value and continue to construct a \textit{points-to graph}, where each node contains a set of aliasing values with the same type. Starting from each root node, we recursively iterate over the users of each value. During the iteration, we create a successor node when a pointer creates a new value or is cast to a different type, e.g., \cc{GetElementPtr}, \cc{BitCast}, \cc{Load}, \cc{Call}, \cc{Return} instructions.

\ignore{
Specifically, we focus on the instruction types below. 

\begin{compactitem}[$\bullet$]
    \item \textit{GetElementPtr} (\cc{\%result = GEP(type,\%ptrOp,indices)}) calculates the address of a sub-object within an object. To be field-sensitive, we maintain the indices for each node that includes sub-objects. When a new sub-object value is indexed, we look for a successor node with the same indices. If found, we put the value in that node's alias set. Otherwise, we create a new successor.
    
    \item \textit{BitCast} (\cc{\%result = bitcast type \%op to type2}) converts the operand's type to a different type (\cc{type2}) and creates a new value. We search for a successor node with the same type. If found, we add the new pointer to the node's alias set. If not, we create a new successor.
    
    \item \textit{Store} (\cc{store \%valOp, \%ptrOp}) writes a value to the memory address pointed to by a pointer operand. Note that pointers can be propagated through memory. Conservatively, we consider all values, stored in or loaded from any alias of a pointer operand, as aliased. To do so, we form a \textit{memory edge} between two nodes containing either a value operand or a pointer operand, i.e., \cc{node A} \cc{->} \cc{node B} when an alias in \cc{node A} is stored in or loaded from the address pointed to by any alias in \cc{node B}. Here, we call \cc{node A} a \textit{memory node} of \cc{node B}. Hence, when a value is used as a value operand of a store instruction, we add the value to the alias set of the pointer operand's memory node.
    
    \item \textit{Load} (\cc{\%valOp = load type, \%ptrOp}) reads a value from the memory address pointed to by a pointer operand. As we do for \textit{Store}, we add the value operand to the alias set of the pointer operand's memory node.
    
    \item \textit{Call} (\cc{\%call = call @name(args)}) indicates a function call that makes a control-flow change. If a pointer value is used as a function call's operand, we obtain its corresponding argument by looking into the function definition and add it to the alias set of the pointer value's node.
    
    \item \textit{Return} (\cc{ret \{\%retval}\}) returns to a caller function with an optional return value. If a pointer value is returned, we search for all call sites and add the return values of the callee functions to the alias set of the pointer value's node.
\end{compactitem}
}

\ignore{
\begin{figure}[t]
\begin{lstlisting}[language=c++, style=mystyle3, escapechar=!]
PG = getPointsToGraph(); // From points-to analysis
visitSet = {}; // Init

void handleNode(node):
  if node is found in visitSet: return;
  else: visitSet.insert(node);
  
  node->setTainted(true); // Mark as tainted
  !\color{codered}{foreach}! alias in node->aliasSet:
    !\color{codered}{foreach}! U in alias->users():
      if U is LoadInst:
        doTaintPropagation(U);
  return;

void doTaintPropagation(V):
  !\color{codered}{foreach}! U in V->users(): // U is a user of V
    if U is !\color{codeblue}{StoreInst}!: // store %valOp, %ptrOp
      if valOp == V:
        handleNode(PG->findNode(ptrOp));
    !\color{codered}{elif}! U is !\color{codeblue}{LoadInst}!:
      continue;
    !\color{codered}{elif}! U is !\color{codeblue}{GEPInst}!:
      handleNode(PG->findNode(U));
    !\color{codered}{elif}! U is !\color{codeblue}{CallInst}!:
      !\textit{Get argval from function definition}!;
      doTaintPropagation(argval);
    !\color{codered}{elif}! U is !\color{codeblue}{ReturnInst}!:
      !\color{codered}{foreach}! retval in call sites:
        doTaintPropagation(retval);
    else:
      doTaintPropagation(U);
  return;
  
void taintAnalysis(M):
  !\color{codered}{foreach}! Inst in BBs,Funcs,CG:
    if Inst is !\color{codeblue}{CallInst}!:
      if calledFunc is Extern. I/O func:
        handleNode(PG->findNode(Inst));
  return;
\end{lstlisting}
\caption{Algorithm of \mname{} taint analysis.}
\label{fig:taint}
\end{figure}
}




\noindent
\textbf{Taint analysis.}
In this analysis, we detect taint sources and propagate taint information throughout a program's data flow. We define taint sources as the destination operands of library functions, e.g., \cc{arr} in \cc{scanf("\%s",arr)}, that receive potentially malicious data, such as file I/O, user inputs, and network. To mark values as tainted, we set a propagation policy such that 1) \textit{any pointers that may hold data coming from tainted pointers} are tainted and 2) \textit{all aliases of a tainted pointer} are also tainted. With such a policy, as shown in \fref{tab:taint_results}, we identify 70.34\%, 63.43\%, and 26.6\% of stack, heap, and global objects in the SPEC 2017 C/C++ workloads. We discuss performance and security implications of the results in \fref{ss:performance} and \fref{ss:use_of_taint}.

\ignore{
%\fref{fig:taint} presents our algorithm.
We iterate over instructions to search for library function calls that receive external inputs, such as \cc{scanf()}. If found, we find a node to which the function's taint source value belongs. We then determine the node as tainted, iterate over the users of each alias in the node's alias set, and look for load instructions. Note that the loads found should use the taint source value or its tainted alias as a pointer operand. Hence, we proceed with a recursive taint propagation call that looks for values taking data loaded from a tainted pointer and marks them as tainted.

To extend the coverage, we further take into account several cases where static analysis could have limitations.
}

\begin{figure}[t]
\centering
\includegraphics[width=0.8\columnwidth]{Fig/graph.pdf}

\centering \small (a) Points-to graph representation during a reachability test.
%\label{fig:ex_graph}

\begin{lstlisting}[language=c++, style=mystyle3, escapechar=!]
char constArr[] = "Hello World";
char vulArr[10];
!\colorbox{gray!20}{\color{codered}{char} \color{black}{*ptr = vulArr;}\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }!
!\colorbox{gray!20}{\color{codeblue}{tagd} \color{black}{ptr, TYPE, 20;}\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }!
!\colorbox{gray!20}{\color{codeblue}{cstr} \color{black}{ptr, 20;}\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }!
scanf("%s", ptr);
printf("constArr: %s\n", constArr);
printf("vulArr: %s\n", ptr); ... }
\end{lstlisting}

\vspace{0.5cm}
\centering \small (b) Instrumented code after applying the selective DPT pass.
%\label{fig:ex_code}
\caption{Example of selective DPT on unsafe code (\fref{lst:example_code}).}
\label{fig:selective_sign}
\end{figure}

\ignore{
\noindent
\textbf{Intrinsic functions.} For better optimization, some library functions can be represented as intrinsic functions. Since their function bodies are not presented in LLVM IR, this hinders our inter-procedural analysis. To increase the coverage, we detect string functions known to be prone to memory bugs, such as \cc{strcpy()} and \cc{memcpy()}, and manually propagate taint from source to destination.

\noindent
\textbf{Function pointers.} The static analysis has difficulties in tracking the control flow change by function pointers since the functions being called are determined at runtime. To mitigate the limitation, we collect functions not included in the CG, which might be called only via function pointers, and perform separate taint analysis, tainting all function arguments.

\noindent
\textbf{Command line arguments.} Since the command line arguments, e.g., \cc{argc}, \cc{argv[]} in C/C++, are supplied by a user, we taint all the arguments of \cc{main()}.
}

\noindent
\textbf{Selective DPT.}
Finally, we determine which values are vulnerable, in terms of memory safety, and thus need to be protected via DPT. To make a decision, we perform a simple taint reachability test. In the points-to graph obtained from the previous analysis, we traverse all successor nodes of each root node and check if any tainted node is found. Note that each root node contains a memory object value returned by an initial memory allocation method. If a tainted node is found, we consider the root node's object value to be vulnerable and therefore apply DPT to the value (see \fref{sss:protection}). Notably, the only decision we make through all the analysis is whether we apply DPT at each object's allocation site or not. Hence, we do not make any intrusive changes to the program code.

\fref{fig:selective_sign} shows an example of code instrumentation using selective DPT. During the taint analysis, we detect the value used as a destination operand of \cc{scanf()} and mark as tainted the node to which the value belongs, as shown in \fref{fig:selective_sign}a. We then figure out the nodes reaching the tainted node. As a result, we recognize \cc{\%vulArr} as a security-critical object and protect it via DPT, as shown in \fref{fig:selective_sign}b.



==> Submitted/V.Methodology.tex <==
%-------------------------------------------------------------------------------
\section{Methodology}
%-------------------------------------------------------------------------------

\begin{table}[t]
    %\scriptsize
    \scriptsize
    \centering
    \caption{System configurations of the BOOM core.}
    \begin{tabular}{llll}
      \toprule
      \textbf{Clock}
        & 65 MHz
        & \textbf{L1-I cache}
        & 32KB, 8-way \\
      \textbf{LLC}
        & 4MB
        & \textbf{L1-D cache}
        & 64KB, 16-way \\
      \textbf{DRAM}
        & 16 GB DDR3
        & \textbf{L2 cache}
        & 512KB, 8-way \\
      \midrule
      \multicolumn{2}{l}{\textbf{Front-end}}
        & \multicolumn{2}{l}{8-wide fetch} \\
        & & \multicolumn{2}{l}{16 RAS {\&} 512 BTB entries} \\
        & & \multicolumn{2}{l}{gshare branch predictor} \\
      \cmidrule(lr){3-4}
      \multicolumn{2}{l}{\textbf{Execution}}
        & \multicolumn{2}{l}{3-wide decode/dispatch} \\
        & & \multicolumn{2}{l}{96 ROB entries} \\
        & & \multicolumn{2}{l}{100 int {\&} 96 floating point regs} \\
        \cmidrule(lr){3-4}
        \multicolumn{2}{l}{\textbf{Load-store unit}}
        & \multicolumn{2}{l}{24 LQ and 24 SQ entries} \\
        & & \multicolumn{2}{l}{24 SLQ and 24 SSQ entries} \\
        \cmidrule(lr){3-4}
        \multicolumn{2}{l}{\textbf{Ptr-tagging unit}}
        & \multicolumn{2}{l}{tagd and xtag: 1-cycle latency} \\
        \bottomrule
    \end{tabular}
    \label{tab:params}
\end{table}

We prototype \mech{} on top of the RISC-V BOOM core~\cite{BOOM} and operate using FireSim~\cite{firesim}, an open-source FPGA-accelerated hardware platform for full-system simulation. We synthesize our custom core at 65MHz, the default target frequency of the BOOM core, and launch Amazon EC2 F1 instances running the Linux OS compatible with RISC-V. To create instrumented binaries, we design custom optimizer and backend passes in LLVM-9.0.1~\cite{LLVM}. To add runtime support required by \mech{}, we modify the Linux kernel (\cc{version:5.7-rc3)}. To evaluate performance, we compile and run SPEC 2017 C/C++ workloads~\cite{SPEC2017}. While our environment setup enables cycle-accurate simulations at a full-system level, we observe that the inherently long execution time of some SPEC 2017 C/C++ workloads makes FPGA simulations infeasible. Note that the achievable clock frequency is at most 65MHz due to the limitation of the FPGA environment, and this can lead to simulation time longer than a few weeks for several workloads. Considering this constraint, we estimate the expected execution time by running unintrumented programs on our host machine and choose an appropriate input size for each workload that allows us to finish the whole program execution in a reasonable time frame (< 1 week). As a result, we run \cc{perlbench\_r}, \cc{mcf\_r}, and \cc{xz\_r} using reference inputs, run \cc{lbm\_r}, \cc{xalancbmk\_r}, \cc{x264\_r}, and \cc{deepsjeng\_r}, and \cc{nab\_r} using train inputs, and run the others using test inputs. With the system configurations presented in \fref{tab:params}, we evaluate three configurations as follows.

\begin{compactitem}[$\bullet$]
  \item \cc{DPT-Heap}: \mname{} enabled only with heap memory protection. This configuration has security coverage comparable to that of the prior work~\cite{AOS,CHEx86,C3}.
  \item \cc{DPT-Full}: \mname{} with full memory safety, including stack, heap, and global memory protection.
  \item \cc{DPT-Taint}: \cc{DPT-Full} combined with static taint analysis.
\end{compactitem}

%We evaluate performance and security by running programs instrumented by \mname{} using the gem5 simulator~\cite{gem5}, where the underlying hardware platform is implemented. The proposed compiler methods are designed as optimization passes in LLVM-8.0~\cite{LLVM}. To compile programs, we extract bitcode files by using the \cc{wllvm} tool~\cite{wllvm} with the \cc{-O0} option. Then, we apply our passes and generate instrumented programs using the Arm AArch64 ISA with the \cc{-O3} option. 

%To measure the performance, we run the SPEC CPU 2006 workloads~\cite{SPEC2006} with reference input sets. Among the C/C++ applications compilable in our environment, we exclude six applications (\cc{gcc}, \cc{soplex}, \cc{h264ref}, \cc{omnetpp}, \cc{perlbench}, and \cc{xalacbmk}) from our evaluation because they have inherent memory safety violations due to memory model violation or real bugs~\cite{IntelMPX}. The numerous bugs detected by \mname{} imposed a non-trivial slowdown, so we could not make a fair comparison for those. We evaluate the remaining applications with four system configurations using the parameters shown in \fref{tab:params}. We guarantee that the instrumented programs of all configurations execute the same call path as the baseline.


%Furthermore, we evaluate the NIST Juliet test suite 1.3 for C/C++~\cite{Juliet-suite}. In the test suite, we select seven common weakness enumeration (CWE) categories on memory safety violations and show that \mname{} is capable of detecting all memory bugs in our scope.


==> Submitted/W.Evaluation.tex <==
%-------------------------------------------------------------------------------
\section{Evaluation}
\label{s:eval}
%-------------------------------------------------------------------------------

\subsection{Performance Analysis}\label{ss:performance}
\fref{fig:execution_time} presents the slowdowns of three configurations across the SPEC 2017 C/C++ workloads, normalized to the baseline. First, \cc{DPT-Heap} exhibits a 4.6\% average slowdown. Among the various types of memory protection (see \fref{ss:ensuring}), \cc{DPT-Heap} only enables heap memory protection, having security coverage comparable to that of previous pointer-tagging methods, such as AOS and C\textsuperscript{3}. With our generalized approach, \cc{DPT-Full} extends security coverage up to stack and global objects and shows a 10.9\% slowdown on average.

The increased runtime overhead is attributed to the cache pollution effect and increased hardware resource contentions. As we extend protection coverage, the number of memory objects we need to protect increases, and therefore more capability metadata need to be maintained in the memory space. Given that capability metadata are redundant in terms of normal program execution, such metadata can thrash useful cache lines when they are brought into the D-cache, causing cache pollution. Moreover, the increased number of capability checks for more memory objects can result in increased hardware resource contentions in the memory execution pipeline as explained in \fref{cap_exec_pipe}. The C-cache (see \fref{ss:cache}) contributes to minimizing such contentions by enabling on-the-fly capability checks without additional memory accesses.



While \cc{DPT-Full} shows negligible performance overheads for most applications, demonstrating its feasibility as a runtime solution, non-trivial performance overheads are measured for some workloads, such as \cc{perlbench\_r}, \cc{xalacbmk\_r}. To interpret such overheads, we collect runtime statistics representing the number of new instructions inserted by DPT instrumentation (\fref{fig:new_inst}) and the ratio of tagged memory instructions over the total memory instructions (\fref{fig:load_store}). Our analysis based on the statistics reveals that in \cc{perlbench\_r}, a high ratio of tagged memory instructions ($\sim$30\%) results in a number of capability checks. Moreover, with non-trivial memory object allocations, the C-cache hit rate is measured low (92.71\%), indicating that not a few capability checks cause non-trivial extra memory accesses, causing resource contentions in the memory pipeline. In the case of \cc{xalancbmk\_r}, we observe numerous dynamic memory allocations that cause not only considerable cache pollution but also a non-trivial overhead from iterative accesses to the CMT. As shown in \fref{tab:hit_iter}, \cc{xalancbmk\_r} has a near-two average iteration number.

%First, \cc{DPT-Heap} exhibits a 4.6\% average slowdown for its heap memory protection. We analyze that the performance overhead mainly comes from the memory overhead by additional capability metadata.  As we pursue broader protection, we may need to maintain more metadata from various memory types, and those can \textit{thrash} useful cache lines in caches, lowering the cache hit rate. In addition, the additional security checks at runtime can cause cache port contentions, thereby delaying regular memory accesses. Moreover, we observe that applications invoking numerous function calls tend to have non-trivial overhead due to frequent function calls repeating bounds de-/allocations for stack objects upon each entry and exit. For example, \cc{milc} invokes about 10 function calls per 1K instructions, significantly higher than that of other applications, and exhibits the worst slowdown (15\%).

\begin{figure}[t]
\centering
%\includegraphics[width=\columnwidth]{Fig/performance.pdf}
\includegraphics[width=\columnwidth]{Fig/performance.png}
\caption{Normalized slowdown across the SPEC workloads.}
\label{fig:execution_time}
\end{figure}

\begin{figure}[t]
\centering
%\includegraphics[width=\columnwidth]{Fig/new_inst.pdf}
\includegraphics[width=\columnwidth]{Fig/new_inst.png}
\caption{Number of new instructions inserted by DPT.}
\label{fig:new_inst}
\end{figure}

Using static taint analysis, \cc{DPT-Taint} avoids redundant overheads for untainted (safe) memory objects and thereby reduces the average slowdown to 7.5\%. \fref{tab:taint_results} shows that the analysis identifies $\sim$30\% of memory objects as untainted and effectively prunes capability execution overheads for untainted objects. The runtime statistics support the effectiveness of the static taint analysis. \fref{fig:new_inst} shows that, compared to \cc{DPT-Full}, \cc{DPT-Taint} reduces the number of new instructions inserted by 40.1\% on average. The reduced number of pointer-tagging and capability instructions leads to a less number of capability requests generated for capability checks and sent to the D-cache. \fref{fig:network_traffic} shows that \cc{DPT-Taint} reduces the number of cache accesses by capability requests by 41.63\% on average. %Note that the reduction in the number of memory requests helps not only mitigate runtime overhead but also 
%From these results, we confirm that \mech{} mitigates the inevitable execution and memory overhead resulting from a memory protection scheme and enables practical yet robust protection.
 
%Notably, \cc{gobmk} prunes 99.9\% of global objects and reduces its overhead from 3.51x to 24\%. \cc{milc} also benefits from the taint analysis by pruning 78.0\% of the objects, and its overhead is reduced by 9\%. 

%As mentioned above, the main sources of the runtime overhead are . We note that the static taint analysis can be effective in . To do so, \cc{DPT-Taint} employs static taint analysis and . Notably, the average slowdown is reduced down to 8.5\%. Furthermore, our analysis reveals that can be effective in reducing power consumption by reducing the number of cache accesses. To confirm this, we count the number of cache accesses by capability requests. As shown in *, the number of extra memory requests are reduced by * on average.
%From these results, we confirm that \mech{} mitigates the inevitable execution and memory overhead resulting from a memory protection scheme and enables practical yet robust protection.


\begin{figure}[t]
\centering
%\includegraphics[width=\columnwidth]{Fig/tag_ratio.pdf}
\includegraphics[width=\columnwidth]{Fig/tag_ratio.png}
\caption{Ratio of tagged memory instructions.}
\label{fig:load_store}
\end{figure}

\begin{figure}[t]
\centering
%\includegraphics[width=\columnwidth]{Fig/network_traffic.pdf}
\includegraphics[width=\columnwidth]{Fig/network_traffic.png}
\caption{Number of cache accesses by capability requests.}
\label{fig:network_traffic}
\end{figure}


\subsection{Hardware Overhead Estimation}
To estimate the hardware overhead imposed by \mech{}, we synthesize our design using Synopsys Design Compiler using 45nm FreePDK libraries~\cite{FreePDK45} at 1GHz clock frequency. To obtain realistic estimates of the SRAM modules, such as L1 D-cache, L1 I-cache, and branch predictor (BPD) tables, we black-box all the SRAM blocks and use analytical models from OpenRAM~\cite{OpenRAM}. \fref{tab:hw_overhead} shows that \mech{} only incurs 8.6\% area and 11.6\% power overhead.


\begin{table}[t]
    \centering
    \caption{Hardware overhead estimates.}
    \begin{scriptsize}
    \begin{tabular}{@{}lcc@{}}
    \toprule
                                & \textbf{Area (mm\textsuperscript{2})}  & \textbf{Power (mW)}        \\
    \midrule
    \textbf{BOOM Core}~\cite{BOOM}       & 6.2812                        & 15.3612           \\
    \textbf{\mech{} Core}                & 6.8266                        & 17.1550           \\
    \bottomrule
    \end{tabular}
\label{tab:hw_overhead}
\end{scriptsize}
\end{table}

==> Submitted/X.Security.tex <==
%-------------------------------------------------------------------------------
\section{Security Analysis}
\label{sec:security}
%-------------------------------------------------------------------------------
\ignore{
\subsection{\mname{} Capabilities}
The capabilities of \mname{} are enforced by a security policy that all memory objects protected have corresponding object pointers carrying over encrypted pointer tags, and all memory accesses by the tagged (signed) pointers are validated.

\noindent
\textbf{Spatial safety.} Once an object is allocated, it occupies a valid, restricted memory region in memory. \mname{} ensures that the alive object's bounds are maintained in memory, and any memory access deviating from its allowed range is detected by comparing the memory address with the object's bounds.

\noindent
\textbf{Temporal safety.} After an object is deallocated, any dangling pointers to the region become invalid. \mname{} prevents the use of such dangling pointers, i.e., use-after-free, by removing the object's bounds from the HBT but leaving dangling pointers signed. Afterward, any subsequent use of such pointers will fail in bounds checking because of the lack of the corresponding bounds.

\noindent
\textbf{Double-free.} In glibc 2.26, the new thread local-caching mechanism (\cc{tcache}) exposed a new heap exploit, namely double-free. \mname{} can also prevent double-free attacks. As can be seen in \fref{lst:heap}, we insert the \cc{wyfy\_bndclr()} before \cc{free()} and enforce the pointer's bounds to be cleared using the \cc{bndclr} . When double-free occurs, the execution of the \cc{bndclr} will fail since the corresponding bounds would have been cleared before and will not be found in the CMT.
}

\ignore{
\subsection{Juliet Test Suite}
To evaluate the \mname{} capabilities, we run the NIST Juliet test suite 1.3 for C/C++~\cite{Juliet-suite}. Out of a total of 118 test categories, we select the categories of the types of errors we expect \mname{} to cover, as enumerated in \fref{tab:juliet}. We confirm that the selected test cases include spatial, temporal, and sub-object safety violations. From the selected categories, we exclude several subcategories that require a network connection or depend on randomly generated values since the gem5 simulator does not support them. We confirm that \mname{} detects all bugs that lie in the categories of our interest.
}

%Most of the test cases are intentionally devised such that inherent memory bugs statically happen without external inputs. Hence, we test them without our static analysis (\textit{WYFY-F}). For the specific subcategories, such as \cc{fgets} and \cc{fscanf}, where memory bugs are invoked by external inputs, we run the test cases enabling our static analysis (\textit{WYFY-FT}). 

\subsection{Forgeability}
While the attack surface exposed to attackers is significantly reduced by \mname{}'s protection, attackers might try to exploit forging attacks. For example, attackers may try to forge the upper bits of a pointer, where a pointer tag is stored, e.g., via pointer arithmetic. Some prior work~\cite{AOS,C3} seeks enhanced security by adopting cryptographic hash functions as a pointer-tag generation algorithm, such as QARMA~\cite{QARMA} and Gimli~\cite{Gimli}. In \mech{}, we use CRC-16, which is simple and provides low hash collisions, since we aim for our design to be freely used in other commercial or open-source projects. Despite the static algorithm of CRC-16, address space layout randomization (ASLR) techniques in modern operating systems help make CRC-16 hashes unpredictable with weak security. Such unpredictability makes the forging attacks less feasible. Assume that an attacker adds an integer large enough to zero out a tagged pointer's tag to bypass the \mname{}'s mechanism. Without knowing the pointer's tag value, the attacker will not know which integer value needs to be used. Instead, the attacker might attempt to change the tag to an (nonzero) arbitrary value and access memory regions associated with that. However, the attacker still has no knowledge of which memory regions are associated with which tags.



%\noindent
%\textbf{CMT forgeability.} Attackers may attempt to corrupt bounds in the CMT and go through bounds checking with corrupted ones. Since a bounds address can be computed using the base address of the CMT and a PAC, i.e., \cc{CMT[PAC]}, we ensure that a user process does not create any virtual-to-physical address translation to memory regions of the CMT. Hence, the CMT is only accessible via bounds instructions, e.g., \cc{bndstr}, not regular memory instructions. With such a constraint, corrupting the CMT using bounds instructions is challenging because attackers do not know which location in the HBT needs to be manipulated without knowing the PAC corresponding to a target memory region.

\ignore{
\begin{table}[tb]
%\small
\scriptsize
\centering
\caption{Tested CWE categories in Juliet test suite.}
\label{tab:juliet}
%\begin{tabular}{@{}p{4cm}p{1.7cm}p{1.7cm}@{}}
%\begin{tabular}{@{}l>{\centering\arraybackslash}m{1.4cm}@{}}
\begin{tabular}{@{}lccc@{}}
%{@{}l>{\centering\arraybackslash}m{1cm}@{}}

    \toprule
    \textbf{Category}           & \textbf{\# Tests} & \textbf{\# Detected} & \textbf{\# Detected} \\
                                & & \textbf{by AOS~\cite{AOS}}  & \textbf{by \mname{}} \\
    \midrule
    CWE121\_Stack\_Based\_Buffer\_Ovf.      & 4749 & \xmark     & \cmark     \\ %\hline
    CWE124\_Buffer\_Underwrite                  & 1876 & \xmark      & \cmark    \\  %\hline
    CWE127\_Buffer\_Underread                   & 1876 & \xmark      & \cmark    \\  %\hline
    CWE416\_Use\_After\_Free                    & 415  & \cmark     & \cmark    \\  %\hline
    CWE122\_Heap\_Based\_Buffer\_Ovf.       & 5332 & \cmark   & \cmark    \\ % \hline
    CWE126\_Buffer\_Overread                    & 1170 & \xmark     & \cmark  \\  %\hline
    CWE415\_Double\_free                        & 962  & \cmark    & \cmark   \\
    \midrule
    \textbf{Detection rate}  &       & \textbf{41\%}     & \textbf{100\%}      \\
    \bottomrule
\end{tabular}
\end{table}
}

%\noindent
%\textbf{SMT.} [TODO]

\subsection{False Positives}
Given the limited tag size, hash collisions cause false positives across data pointers carrying the same tag. However, the available tag size, varying from 11 to 32 bits depending on the virtual address schemes, provides robustness against false positives. For example, to exploit false positives with a 16-bit tag size, adversaries would need to attempt 45425 runs to achieve a 50\% likelihood for a correct guess~\cite{pacitup}. %A brute-force attack would also be impractical since different PA keys will be assigned whenever a new process is spawned.

\ignore{
\subsection{Pointer Integrity}
\label{ss:pointer_integrity}
Chen et al.~\cite{dop_attack} demonstrate that non-control-data attacks can be realistic attack vectors. Without altering control flow, such data-oriented programming (DOP) attacks exploit data pointers to corrupt application data, including user identity and security-critical configurations. \mname{} effectively protects against such attacks by enforcing an invariant that memory accesses always operate within the allowed range. Besides the DOP attacks, control-flow attacks, such as return-oriented programming~\cite{ROP} and jump-oriented programming~\cite{JOP}, become a promising attack vector. We note that the proposed data-pointer signing scheme is orthogonal to the existing PA-based code-pointer integrity methods~\cite{armpa, pacitup}. Since our design is based on the AArch64 architecture, the Arm PA primitives can be easily enabled for code-pointer signing to protect against control-flow attacks.
}
\subsection{Double-Free} 

In glibc 2.26, the new thread local-caching mechanism (tcache) exposed a new heap exploit, namely double-free. This attack can be prevented in \mech{}. As shown in \fref{fig:dps}b, we insert a \cc{cclr} before \cc{free()} and clear the pointer's capability metadata. When double-free occurs, the \cc{cclr} will fail since the corresponding metadata would have been already cleared and will not be found in the CMT.

\subsection{Use of Static Taint Analysis}\label{ss:use_of_taint}
The security guarantee of typical static analysis techniques is determined by the precision (high coverage with many false positives) and soundness (moderate coverage with all true positives) of the analysis~\cite{drchecker}.
%Too precise static analysis may require infeasible computational complexity whereas sound analysis may suffer from high false positives. Nevertheless, 
Meanwhile, extensive research in the area has presented many practical solutions. For instance, control-flow integrity (CFI) and data-flow integrity (DFI) solutions have shown their practicality by detecting numerous bugs in real-world programs~\cite{DFI,CFI,PITTYPAT}. By sharing the basic mechanism, our analysis guarantees security comparable to that of prior work. When users want to use \mech{} for testing and debugging, e.g., to catch and fix benign bugs, or prefer better security,
%being concerned about any potential security holes,
the static taint analysis can be skipped. %during the compiler's optimization phase.


%However, developers may want to use the \mname{} framework for testing and debugging purposes, e.g., to catch and fix benign bugs from human errors. Or, one may prefer better security to high performance, being concerned about any potential security holes. In those cases, the taint analysis pass can be skipped during the compiler's optimization phase.






==> Submitted/Y.Discussion.tex <==
%-------------------------------------------------------------------------------
\section{Discussion}
%-------------------------------------------------------------------------------
\subsection{Compatibility}
From our full-system evaluations, we learn valuable lessons in terms of compatibility issues all pointer-tagging methods may have. First, we observe that pointer arithmetic using two pointers, e.g., \cc{offset=ptrA-ptrB;} can result in incorrect values when both pointers are tagged and have different tags. As an example, we find this type of operations in programs where custom data structures are defined, and the relative offset between two objects is obtained by subtracting one's address from another's. To avoid this issue, given that LLVM IR converts such pointer arithmetic into two \cc{ptrtoint} instructions and a \cc{sub} instruction, we insert \cc{xtag}s before \cc{ptrtoint}s and remove pointer tags before pointer arithmetic. We presume that this finding may contradict some prior work that claims the advantage of not requiring source code recompilation~\cite{C3}.

Next, some functions in standard or third-party libraries, such as file I/O functions, may cause compatibility issues when they take tagged pointers as function arguments. We presume that those functions contain pointer arithmetic incompatible with tagged pointers, such as the above-mentioned case. To work around this issue, we whitelist compatible and safe functions and insert \cc{xtag}s to remove tags of pointers passed to library functions not included in our list. In fact, Google observed a similar challenge with Arm memory tagging extensions (MTE) and modified various routines in the Android C library~\cite{GoogleLLC}. We expect such efforts to be made to help mitigate this issue.

\ignore{
\subsection{Static vs. Dynamic Taint Analysis}
Typical static taint analysis~\cite{PhASAR,DepTaint,SWAN,ConDySTA} causes an over-tainting problem since it analyzes all possible executions at compile time. In contrast, dynamic taint analysis~\cite{GPU-taint,TaintCheck,TaintBochs,Dytan,TaintDroid,LIFT} can track the exact execution path at the cost of runtime overhead. In this work, while we focus on static taint analysis to avoid extra runtime overheads, we leave the exploration of dynamic analysis techniques as future work.
}

\subsection{Applicability}
Even though we prototype \mech{} in the RISC-V ecosystem, we believe that our hardware modifications are generally applicable to other architectures, such as x86, AArch64, and SPARC. This is because the BOOM core has primary architecture components common to modern architectures, such as an out-of-order memory execution pipeline including TLBs, a page-table walker (PTW), and a memory management unit (MMU), and our changes are made on top of those.


==> Submitted/Y.RelatedWork.tex <==
\ignore{
\begin{table*}[t]
    \centering
    \caption{Comparison between \mname{} and previously proposed memory safety mechanisms.}
    \label{tab:comparison}
    \begin{threeparttable}
    \begin{scriptsize}
    \begin{tabular}{@{}lccccc@{}}
    %\begin{tabular}{@{}lC{0.94cm}C{0.8cm}C{1.2cm}C{1.2cm}@{}}
    
    \toprule
    Mechanism & HW/SW-based & Spatial Safety & Temporal Safety & Sub-Object Safety & Compatibility Loss~\tnote{1} \\
    \midrule
    ASan~\cite{asan}& SW     & \cmark    & \cmark    & \xmark    & $-$    \\
    SoftBound~\cite{Softbound}  & SW    & \cmark    & \xmark    & \xmark    & $-$    \\
    Baggy Bounds~\cite{BaggyBounds,BaggyBoundsChecking}    
                                & SW    & \cmark    & \xmark    & \xmark    & $-$    \\
    TaintCheck~\cite{TaintCheck}& SW    & \cmark~\tnote{2} & \cmark~\tnote{2} & \xmark & $-$ \\
    \midrule
    
    %Arm PA~\cite{armpa}         & HW    & \xmark    & \xmark    & \xmark    & $-$    \\
    %PARTS~\cite{pacitup}    & HW    & \xmark    & \xmark    & \xmark    & $-$    \\
    %ZeRØ~\cite{zero21}            & HW    & \xmark    & \xmark    & \xmark    & $-$    \\
    %\midrule
    REST~\cite{REST}            & HW    & \cmark~\tnote{3}    & \xmark    & \xmark    & $-$    \\ 
    Califorms~\cite{Califorms}  & HW    & \cmark~\tnote{3}    & \cmark~\tnote{3}    & \xmark    & Src, Bin  \\ 
    \midrule
    Intel MPX~\cite{IntelMPX}   & HW    & \cmark    & \xmark    & \cmark    & $-$    \\ 
    HardBound~\cite{Hardbound}  & HW    & \cmark    & \xmark    & \xmark    & $-$    \\ 
    Watchdog~\cite{Watchdog}    & HW    & \cmark    & \cmark    & \xmark    & $-$    \\
    CHERI~\cite{CHERI,Cheri-concentrate,CHERIvoke,Cornucopia}
                                & HW    & \cmark    & \cmark    & \cmark    & Src, Bin    \\ 
    \midrule
    Arm MTE~\cite{armpa}        & HW    & \cmark    & \cmark    & \cmark    & $-$    \\ 
    SPARC ADI~\cite{SPARC_ADI}  & HW    & \cmark~\tnote{4}    & \cmark~\tnote{4}    & \xmark    & $-$    \\
    \midrule
    AOS~\cite{AOS}              & HW    & \cmark~\tnote{4}  & \cmark~\tnote{4}  & \xmark    & $-$ \\
    C\textsuperscript{3}~\cite{C3}  & HW    & \cmark~\tnote{4}  & \cmark~\tnote{4}  & \xmark    & $-$ \\
    No-FAT~\cite{No-FAT}          & HW    & \cmark~\tnote  & \cmark~\tnote  & \cmark~\tnote    & Src, Bin \\
    In-Fat Pointer~\cite{in-fat-pointer} & HW   & \cmark   & \xmark    & \cmark    & $-$    \\
    \midrule
    \mname{}    & HW       & \cmark            & \cmark        & \cmark
                & $-$    \\
    \bottomrule
    \end{tabular}
    \end{scriptsize}

    \begin{tablenotes}
    \begin{footnotesize}
    \item[1] Some prior work requires source modifications or recompiling the libraries, losing source compatibility (Src) or binary compatibility (Bin).
    \item[2] Taint analysis-based security checking is applied only to selected attack targets, such as a jump address and format string.
    \item[3] Canary-based protection is applied.
    \item[4] Protection only applies to heap memory regions.
    
    \end{footnotesize}
    \end{tablenotes}    
    
\end{threeparttable}
\label{tab:related_work}
\end{table*}
}


\ignore{
\begin{table}[t]
    \centering
    \caption{Comparison between \mname{} and previous defense mechanisms for memory safety.}
    \label{tab:comparison}
    \begin{threeparttable}
    \begin{footnotesize}
    %\begin{tabular}{@{}lccccc@{}}
    \begin{tabular}{lcccc}
    %\begin{tabular}{@{}lC{0.94cm}C{0.8cm}C{1.2cm}C{1.2cm}@{}}
    
    \toprule
    Mechanism   & Spatial & Temporal & Sub-Obj. & Comp. \\
                & Safety & Safety & Safety & Loss~\tnote{1} \\
              
    %\midrule
    %ASan~\cite{asan}& SW    & \xmark    & \cmark    & \cmark    & \xmark    & $-$    \\
    %SoftBound~\cite{Softbound}  & SW    & \xmark    & \cmark    & \xmark    & \xmark    & $-$    \\
    %Baggy Bounds~\cite{BaggyBounds,BaggyBoundsChecking}    
    %                            & SW    & \xmark    & \cmark    & \xmark    & \xmark    & $-$    \\
    %TaintCheck~\cite{TaintCheck}& SW    & \xmark    & \cmark~\tnote{2} & \cmark~\tnote{2} & \xmark & $-$ \\
    %\midrule
    %Arm PA~\cite{armpa}         & \cmark    & \xmark    & \xmark    & \xmark    & $-$    \\
    %PARTS~\cite{pacitup}    & \cmark    & \xmark    & \xmark    & \xmark    & $-$    \\
    %ZeRØ~\cite{zero21}            & \cmark    & \xmark    & \xmark    & \xmark    & $-$    \\
    \midrule
    REST~\cite{REST}            & \cmark    & \xmark    & \xmark    & $-$    \\ 
    Califorms~\cite{Califorms}  & \cmark    & \cmark    & \xmark    & Src, Bin  \\ 
    \midrule
    Intel MPX~\cite{IntelMPX}   & \cmark    & \xmark    & \cmark    & $-$    \\ 
    HardBound~\cite{Hardbound}  & \cmark    & \xmark    & \xmark    & $-$    \\ 
    Watchdog~\cite{Watchdog}    & \cmark    & \cmark    & \xmark    & $-$    \\
    CHERI~\cite{Cornucopia,Cheri-concentrate,CHERI,CHERIvoke}
                                & \cmark    & \cmark    & \cmark    & Src, Bin    \\ 
    \midrule
    Arm MTE~\cite{armpa}        & \cmark    & \cmark    & \cmark    & $-$    \\ 
    SPARC ADI~\cite{SPARC_ADI}  & \cmark~\tnote{2}    & \cmark~\tnote{2}    & \xmark    & $-$    \\
    \midrule
    AOS~\cite{AOS}              & \cmark~\tnote{2}  & \cmark~\tnote{2}  & \xmark    & $-$ \\
    C\textsuperscript{3}~\cite{C3}  & \cmark~\tnote{2}  & \cmark~\tnote{2}  & \xmark    & $-$ \\
    No-FAT~\cite{No-FAT}          & \cmark~\tnote  & \cmark~\tnote  & \cmark~\tnote    & Src, Bin \\
    In-Fat Pointer~\cite{in-fat-pointer} & \cmark   & \xmark    & \cmark    & $-$    \\
    \midrule
    \mname{}    & \cmark            & \cmark        & \cmark
                & $-$    \\
    \bottomrule
    \end{tabular}
    \end{footnotesize}

    \begin{tablenotes}
    \begin{footnotesize}
    \item[1] Some prior work requires source modifications or recompiling the libraries, losing source compatibility (Src) or binary compatibility (Bin).
    %\item[2] Taint analysis-based security checking is applied only to selected attack targets, such as a jump address and format string.
    \item[2] Protection only applies to heap memory regions.
    
    \end{footnotesize}
    \end{tablenotes}    
    
\end{threeparttable}
\label{tab:related_work}
\end{table}
}

\section{Related Work}
\label{s:related_work}
%Since we aim to design a hardware mechanism in this work, we focus on previous hardware-based approaches.
We compare and discuss prior proposals against memory safety as follows.


\noindent
\textbf{Software solutions.}
While software approaches~\cite{asan,Softbound,BaggyBounds,BaggyBoundsChecking,TaintCheck,EffectiveSan} typically guarantee a variety of security policies, their versatility comes with significant overhead. For example, AddressSanitizer (ASan)~\cite{asan} stores valid bits for live objects in reserved space (shadow memory) for every 8 bytes and validates memory accesses by checking the valid bits. Combined with a quarantine zone design for preventing temporal reuse of freed regions, ASan presents a 73\% slowdown. %TaintCheck~\cite{TaintCheck} uses dynamic taint analysis by performing binary rewriting at runtime and enables automatic detection on a subset of overwrite attacks. However, its way of binary rewriting and dynamic taint propagation at runtime suffers from up to 37x slowdown~\cite{LIFT}.


\ignore{
\noindent
\textbf{Pointer authentication.} 
As a commercial technology, Arm PA~\cite{armpa} aims to prevent illegal pointer modification. Using QARMA~\cite{QARMA}, Arm PA places a PAC in a pointer and authenticates the PAC before use to verify its integrity. Using the same primitives, PARTS~\cite{pacitup} further extends the security capabilities by proposing PA-based data-pointer integrity.
%To detect illicit manipulation, PARTS signs a data pointer right before storing it in memory and authenticates right after loading it from memory.
ZeRØ~\cite{zero21} implements new memory instructions and a metadata encoding scheme to protect code and data pointers. Despite the low cost of PA-based methods, their security coverage is limited since neither spatial nor temporal safety is fully ensured. 
%[TODO] should the limitation of data pointer integrity be mentioned here or later?
%We defer more details of security analysis to \fref{sec:security}.
}

\noindent
\textbf{Trip-wire.}
Trip-wire methods place secret bytes around objects to protect. The secret bytes are not supposed to be accessed by unprivileged normal operations, and any access to the secret bytes is prohibited. REST~\cite{REST} embeds a randomized token near benign buffers and has a comparator in the cache hierarchy to detect the token being accessed. Califorms~\cite{Califorms} leverages unused padding bytes and places security bytes at byte granularity, minimizing memory overhead. Trip-wire solutions have limited security coverage despite low-cost protection because they cannot detect out-of-bounds accesses jumping over secret bytes.

%However, it may have compatibility issues due to its source-to-source translation and type layout changes.


\noindent
\textbf{Fat pointer.}
\label{ssc:fat-pointer}
Fat-pointer schemes extend the pointer size to hold security metadata. The CHERI capability model~\cite{CHERI, Cheri-concentrate, CHERIvoke, Cornucopia} implements a capability co-processor with a set of capability registers (256 bits each at worst case) holding bounds and permission bits. Object accesses are forced to check their bounds and control access using the capability metadata. However, the design requires changes to most system stacks, including the compiler, the language runtime, and the OS, and ends up losing both source and binary compatibility. Similarly, Hardbound~\cite{Hardbound} and Watchdog~\cite{Watchdog} implement register extensions to maintain per-pointer metadata. However, their overhead of explicit memory checking and metadata propagation results in a significant slowdown. Intel Memory Protection Extensions (MPX)~\cite{IntelMPX} implements two-level address translation to access bounds. However, its complicated addressing based on a multi-level bounds table incurs non-trivial overhead.

%Moreover, its hardware complexity is reported to be significant.\footnote{The initial architecture~\cite{CHERI} reports 32\% increased logic elements and 8\% reduction of achievable clock frequency.}

\noindent
\textbf{Memory tagging.}
SPARC Application Data Integrity (ADI)~\cite{SPARC_ADI} and Arm Memory Tagging Extension (MTE)~\cite{armpa} are the representative commercial products that implement memory tagging. In such designs, memory allocation creates a tag and colors the corresponding memory region with the tag. When loads and stores access the colored region, the tag present in a pointer is compared with the tag stored in memory. However, the limited tag size, e.g., 4 bits in Arm MTE, causes a high false-positive rate and allows an attacker to brute-force the tag bits via a sufficient number of attempts. 

\noindent
\textbf{Pointer tagging.}
\label{ss:pointer-tagging}
%Similarly, pointer-tagging schemes place a pointer tag in a pointer but use the tag to look up an object metadata in memory or check an object-based tag match.
C\textsuperscript{3}~\cite{C3} proposes a state-less (requiring no extra metadata) mechanism that entangles data encryption with encoded memory addresses.
Using a binning allocator, No-FAT~\cite{No-FAT} exposes memory allocation size to hardware and performs hardware-based bounds checking. To enforce temporal safety, No-FAT stores a random tag in a pointer and verifies the tag upon a memory access. In-Fat Pointer~\cite{in-fat-pointer} diversifies object metadata schemes and supports sub-object safety by narrowing object bounds. 
%However, prior studies exhibit limitations in terms of security coverage and compatibility. AOS and C\textsuperscript{3} only provide heap memory safety, while In-Fat Pointer does not guarantee temporal safety. No-FAT may lose compatibility due to source-to-source translation for intra-object protection.

\ignore{
\subsection{LLVM Aliasing Analysis}
A memory object used in LLVM Aliasing Analysis\cite{llvmaa}  is a region of a memory space reserved by a memory allocation like alloca for stack, allocation calls for heap, and global variable definition. It is expressed as a pair of its starting address and a static size. Based on this information, LLVM Aliasing Analysis provides the method to determine whether or not pointers in the code reference or modify the same memory object. LLVM Alaising Analysis is working well with accessing certain address with the same pointer, However, when the pointer name is changed from assigning the pointer to another pointer, it usually fails to recognize that those pointers are pointing the same memory object. Our taint analysis can track the pointer after assigning the pointer to another pointer.
}


==> Submitted/Z.Conclusion.tex <==
%-------------------------------------------------------------------------------
\section{Conclusions}
%-------------------------------------------------------------------------------

We proposed \mname{}, a RISC-V capability architecture that implements full-system support for practical memory safety. For capability enforcement, we proposed a generalized data-pointer tagging method, DPT. To achieve optimal performance, we investigated efficient, lightweight hardware extensions for DPT based on the RISC-V BOOM core. Furthermore, we leveraged static taint analysis to prune possibly redundant capability checks. Putting it all together, \mname{} achieved robust protection at a 7.5\% average slowdown across the SPEC 2017 C/C++ workloads. Our hardware synthesis task measured 8.6\% area and 11.6\% power overheads.% We also evaluated \mname{}'s security capabilities using the NIST Juliet test suite.

%We proposed \mname{}, a framework to implement hardware-assisted full memory safety. We revamped the previously proposed pointer signing scheme to support memory safety for stack, heap, and global variables. While we sign the original heap pointers, we allocate a shadow pointer for stack and global variables. All signed pointers are validated upon dereferencing. Also, sub-object safety is guaranteed via dynamic pointer mutation. Attackers typically utilize external inputs to exploit memory safety vulnerabilities. Our static taint analysis identifies potentially harmful pointers by tracking the dataflow of untrusted external inputs. We avoid unnecessary safety checks for safe pointers to reduce the performance overhead. Our evaluations showed that \mname{} incurs an 18.4\% slowdown on average for SPEC 2006 benchmarks. We believe that our proposal can significantly improve memory safety while it is lightweight enough to be deployable in commodity systems.

==> Submitted/ZZ.PriorReviews.tex <==
Before this submission, we have submitted to ASPLOS'23 Spring and received valuable reviews from reviewers. In this current version, we addressed the previous reviews as follows.

\section{Reviewer A}
\noindent
\textbf{R1 Contribution summary}

\noindent
The extended abstract presented WYFY, a hardware-software approach that combines data pointer tagging and static analysis to address the memory (un)safety problem in C/C++ applications. The problem is well motivated and the proposed solution aims at addressing the performance/security/compatibility limitations of prior techniques.

\noindent
\textbf{Paper summary}

\noindent
The paper presented WYFY, a hardware-software approach that combines data pointer tagging and static analysis to address the memory (un)safety problem in C/C++ applications. The problem is well motivated and the proposed solution aims at addressing the performance/security/compatibility limitations of prior techniques.

\noindent
\textbf{R2 Strengths}

\noindent [+] Memory safety is an important problem

\noindent [+] The paper is well written

\noindent
\textbf{R2 Weaknesses}

\noindent [-] Minor improvements over prior work

\noindent [-] The evaluation methodology is unclear

\noindent [-] Limited performance evaluation

\noindent [-] Missing important related work

\noindent
\textbf{R2 Overall merit}

\noindent 1. Reject

\noindent
\textbf{Questions for authors’ response}

\noindent Please refer to my comments on the full paper below.

\noindent
\textbf{R1 Comments for author}

\noindent Thank you for submitting your work to ASPLOS. The lack of memory safety in C/C++ is an important problem and developing better hardware-assisted solutions is always needed. I have a few comments after reading the extended abstract:

\noindent 1 - Key contributions: The abstract stated that "none of the prior work achieves full memory safety with legacy code compatibility at reasonable overhead" and " WYFY is the first hardware-based mechanism that ensures complete memory safety with legacy code compatibility". While the abstract cited multiple papers to support this claim (e.g., C3/In-Fat/Califorms/No-FAT), the abstract did not acknowledge a recent work (CHEx86 from ISCA 2020), which also provides complete memory safety at low overheads while having full compatibility with legacy binaries.

\noindent 2 - Advantage over prior work: It is not clear how WYFY is significantly different than AOS (other than the sub-object granularity and stack/global protection). I will defer the decision till reviewing the full paper.

\noindent 3 - Pruning unnecessary security checks: I am a bit concerned about depending on static analysis to selectively protect a subset of program objects. This approach is effective in reducing the performance overheads, yet it typically leaves security holes that could be exploited by an attacker, depending on the soundness of the static analysis.

\noindent 4 - Main Artifacts: Are there any specific reasons to use SPEC CPU 2006 workloads instead of SPEC CPU 2017? The latter have higher memory footprint that may affect the quality of the reported overheads.

\noindent
\textbf{R2 Comments for author}

\noindent Thank you for submitting your work to ASPLOS. The lack of memory safety in C/C++ is an important problem and developing stronger hardware-assisted solutions is always needed. Please find my comments and questions on the full paper below:

\noindent 1 - Key contributions: The paper states that "none of the prior work achieves full memory safety with legacy code compatibility at reasonable overhead" and "WYFY is the first hardware-based mechanism that ensures complete memory safety with legacy code compatibility". While multiple papers are cited to support this claim (e.g., C3/In-Fat/Califorms/No-FAT), the authors did not acknowledge or compare against a recent work (CHEx86 from ISCA 2020), which also provides complete memory safety at low overheads while having full compatibility with legacy binaries. Are there any reason for excluding CHEx86 from the related work section and Table 4?

\noindent 2 - Limited improvements over prior work: It is not clear to me how WYFY is significantly different than AOS. The sub-object granularity and stack/global protection are straightforward extensions that have been discussed in prior memory safety solutions before, such as Intel MPX and CHERI.

\noindent 3 - Binary compatibility: The paper states that WYFY maintains both source and binary compatibility. While I agree that source-code compatibility is guaranteed due to maintaining the same pointer size, I would say pointer tagging techniques (including WYFY) do not maintain binary compatibility with uninstrumented code (e.g., third party libraries) for the following two reasons:

(a) The uninstrumented code might use the upper pointer bits for storing other software-related information, which will corrupt WYFY's metadata or affect the correctness of the uninstrumented code.

(b) Conventional address space formats assume that the pointer upper bits are set to zeros for user-land pointers and ones for kernel pointers. Prior memory safety techniques, such as REST/MPX/CHEx86 are compatible with the aforementioned convention. WYFY on the other hand breaks this convention by introducing PAC in the upper pointer bits.

\noindent While point (b) could be addressed by modifying the hardware to explicitly clear the upper pointer bits before memory accesses, point (a) needs further consideration to guarantee smooth interaction with uninstrumented third-party code.

\noindent 4 - Temporal memory safety: If I understood correctly, WYFY detects temporal safety violations as dangling pointers to any free'd objects will remain signed whereas the corresponding HBT entry will be removed, causing a bounds-checking error upon any later dangling pointer access. What would happen after reusing the HBT entry for a new allocation? Won't it be possible to have the PAC of the new allocation collide with the PAC of the dangling pointer, causing the temporal error to go undetected? I think simply maintaining all bounds information of previously free'd objects per each PAC will significantly increase the proposal complexity as the metadata will now become a factor of the overall program objects (millions) and not just the number of live objects.

\noindent 5 - Pruning unnecessary security checks: I am a bit concerned about depending on static analysis to selectively protect a subset of program objects. This approach is effective in reducing the performance overheads, yet it typically leaves security holes that could be exploited by an attacker, depending on the soundness of the static analysis.

\noindent 6 - Using LLVM IR GEP instructions for sub-object memory safety: There is a major caveat in this design choice. The GEP instruction calculates the address of the indexed sub-object by adding an offset to the object base address as seen within the same function scope. In other words, if a function foo(void *ptr) receives a sub-object pointer that has already been adjusted in a different function scope, the GEP instruction within foo will not use the correct base address as a parameter. Instead, it will just add the new offset to the previously-adjusted pointer. How would WYFY handle those cases?

\noindent 7 - Evaluation Methodology: The used evaluation methodology is unclear. Have you run all programs end-to-end on Gem5? If not, have you used sim-points or run the first few billion instructions as AoS?

\noindent 8 - Main artifacts: Are there any specific reasons to use SPEC CPU 2006 workloads instead of SPEC CPU 2017? The latter have higher memory footprint that may affect the quality of the reported overheads.

\noindent 9 - Missing benchmarks: Additionally, all the heavyweight benchmarks (e.g., perlbench, gcc) are not evaluated. Even if certain applications have memory safety bugs (I see that reference [41] only reports four bugs in SPEC 2006), you could either patch those bugs prior to running the performance evaluation or silence the corresponding bounds-checking alarms at runtime to allow for end-to-end evaluation.

\noindent 10 - Reported statistics: It is unclear how the results of Table 2 (\#Total) columns are collected. Do they correspond to end-to-end program execution? If yes, the \#Total heap objects are significantly lower than the ones reported in prior work (e.g., AoS). If no, could you please clarify the reason?

\noindent 11 - Multi-threading support: It would be useful to include a discussion on how WYFY handles multi-threaded applications especially the metadata management aspect and whether it causes any false positives on not.

\noindent 12 - Threat model: While the paper states that side-channel attacks are out-of-scope, I believe a discussion on how side-channel leakage could affect the security guarantees of WYFY (and any future memory safety solution) is important. For example, recent reports (e.g., https://github.com/microsoft/MSRC-Security-Research/blob/master/papers/2020/Security analysis of memory tagging.pdf) discussed how a simple leakage can undermine the security guarantees of memory tagging schemes, such as ARM MTE.

\section{Reviewer B}

\noindent
\textbf{R1 Contribution summary}

\noindent This paper presents WYFY, a workflow for achieving memory safety. The key idea is to use a combination of static program analysis and hardware-based memory protection (ARM pointer authentication). The paper claims to provide complete memory safety (more on this below).

\noindent
\textbf{Paper summary}

\noindent WYFY is a combined hardware/software approach to ensuring memory safety. The main idea is to perform program analysis offline in order to determine how external data inputs affect code that may be exploitable and then protect such code using hardware support. There are additional techniques used under a broad scheme called "data-pointer signing" to treat stack and global objects similarly to how the heap is treated (i.e., by using a shadow pointer). WYFY is low overhead and its security is evaluated using various benchmarks by the authors.

\noindent
\textbf{R2 Strengths}

\noindent Memory safety is a critical issue that requires an effective and efficient solution.
The paper is clearly written and easily understandable

\noindent
\textbf{R2 Weaknesses}

\noindent The most glaring weakness is that the paper is quite incremental compared to AOS. It seems like the main improvement over AOS is that the authors added protection for stack and global variables.
The other major weakness is that the security assumptions are not clearly discussed. I think intuitively, it makes sense that most vulnerable code can be manipulated with external inputs. However, I'd have hoped for a discussion of the implications of this design decision.

\noindent
\textbf{R2 Overall merit}

\noindent 2. Major revision - weak paper, but it has value and can be fixed with revisions

\noindent
\textbf{Questions for authors’ response}

\noindent 1- Can you clearly articulate the major improvements over AOS and how your approach differs? 2- Are there any downsides of the assumption that most vulnerable code can be manipulated using external inputs? Are you missing anything due to this assumption? 3- Is it safe to rely of getelementpointer to ensure security of sub-objects in the presence of pointer aliasing? I guess you mention your analysis is conservative, but wouldn't his result in over-tainting in most legacy code?

\noindent
\textbf{R1 Comments for author}

\noindent (1) The motivation for the paper is quite clear. Memory bugs are still a big problem that causes many security vulnerabilities and innovative and low overhead solutions are welcome.

\noindent (2) It is unclear how the approach is able to provide complete memory safety given that it is only targeted at a subset of memory objects based on a heuristic. You say that vulnerabilities are "typically" exploited through untrusted external inputs. How do you identify untrusted inputs? Is the solution complete as you propose? How can you provide that it is complete? All these questions need to be answered for the claims to be credible and the EA has no evidence to answer these claims. However, the EA is intriguing, and I think the paper should advance to the next round.

\noindent (3) I don't think the idea to try to identify code that must be kept secure is a new one. There is a lot of work on program partitioning in the same vein. I expect this kind of defense to be evaluated with memory intensive applications, and this paper doesn't appear to have done so, which makes it a bit hard to interpret the results. I think the paper needs to better articulate the architectural support and its contributions (presumably the EA is lacking in this but the actual paper does a better job).

\noindent (4) The paper is a good fit for ASPLOS

\noindent
\textbf{R2 Comments for author}

\noindent (1) I think the main insights of the paper are sound and if the revision requests that I outline below are addressed, the paper can be published. This is of course assuming there is a clear differentiator between the proposed approach in this paper and AOS (this wasn't clear to me at all, beyond the simple things like extending protections to stack and globals).

\noindent (2) As mentioned above, the clear advantage over prior work is unclear and the most significant weakness of this paper.

\noindent (3) The paper is otherwise a really good for ASPLOS.

\noindent (4) The approach seems to be sound, given the assumption that vulnerable code can only be accessed via externally manipulatable inputs. Is this always true? It seems like it is intuitively true, but I'd like the authors to comment on this and argue for why this is a foolproof heuristic. If it is not (and that it OK), I'd like a more thorough discussion of the limitations. Note that such limitations wouldn't preclude an acceptance from my perspective. I am actually on board with the idea that the most relevant security-critical code is one that can be manipulated by external inputs.

\noindent
\textbf{Revision requests}

\noindent A clear description of the difference between AOS and WYFY must be present in the revision.

\noindent A justification for the security assumptions (dependence on external inputs) must be present in the revision.

\section{Reviewer C}

\noindent
\textbf{R1 Contribution summary}

\noindent This work proposes a memory safety framework that allows unmodified code to run with minimal performance overhead.

\noindent
\textbf{Paper summary}

\noindent This work proposes to enhance prior work on pointer safety to protect all of the memory address space, including stack and global variables. The work also includes a static taint analysis that aims to reduce the number of checks that need to be done at runtime.

\noindent
\textbf{R2 Strengths}

\noindent Provides pointer safety for all object types (stack, heap, global variable) Keep compatibility for legacy code Pruning mechanism to reduce the security check overhead.

\noindent
\textbf{R2 Weaknesses}

\noindent it is unclear what the novelty over AOS is. It seems that this work is simply extending AOS to allow for stack and global variable protection, but it is not clear why these are challenging to merit a publication on its own. The evaluation is a bit concerning as it seems the authors are cherry picking the benchmarks that perform best. The authors decided to exclude 6 benchmarks because their approach found too many errors.

\noindent
\textbf{R2 Overall merit}

\noindent 2. Major revision - weak paper, but it has value and can be fixed with revisions

\noindent
\textbf{Questions for authors’ response}

\noindent Can you succinctly state what are the challenges (or key insights) that allow you to protect the stack and global variable sin a more efficient way compared to AOS?

\noindent Did you evaluate how much bigger your binary is after your compiler modifications? I see you have how many more instructions are executed on figure 11 but this is limited by your evaluation methodology.

\noindent How does it work with the global variables bounds that are never released? Is the HBT per process and hence flushed after the program exits?

\noindent How do you handle context switches?

\noindent If you assume the inputs to main to be tainted, doesn't this guarantee that the whole program is tainted? Presumably the inputs to main are used for something useful in most programs. What am i missing here?

\noindent What does it mean for your analysis to be field sensitive?

\noindent Can you please explain further what happened with the additional 6 benchmarks that you excluded? This seems like cherry picking to me. I can definitely be wrong but please explain why i would be wrong.

\noindent How do you guarantee that the experiments you ran go through the same call path as the baseline? Are you taking checkpoints? ?Are you warming up the system? Are you running a specific number of instructions?

\noindent What happens when the bndclr instruction fails? How is this protecting against double free attacks?

\noindent
\textbf{R1 Comments for author}

\noindent Memory safety is definitely an important security feature that should be included in all computing devices without incurring significant cost. The key insights are interesting and could merit a second look to determine their worth. The contribution, while still with some performance overhead, enables the implementation of memory safety without having to modify legacy code. The paper is a good fit for ASPLOS.

\noindent
\textbf{R2 Comments for author}

\noindent The key insights of the work are unclear, particularly when you compare the contributions to AOS. The paper does not really related the reasons why you chose the particular details of your design, making it difficult to understand the novelty of your work. Your evaluation methodology is a bit odd. Excluding benchmarks because they have bad performance is not really good practice. I could be wrong here, hence my questions above. Furthermore, it is unclear how you guaranteed the gem5 runs to always go through the same call path, as you give no details about how you ran your programs. Also, this is no a show stopper but you are using SPEC 2006 which is now very outdated. I highly recommend upgrading to SPEC2017.

\noindent
\textbf{Revision requests}

\noindent I would like to see the distinctions and key insights compared to AOS clearly outlined. I would also like to see an analysis on how this approach inflates binaries (by how much). I would like to see an explanation of how experiments were ran to guarantee the call path is the same as the baseline. The writing needs to be polished so that the main ideas are clearly explained.

\section{Reviewer D}

\noindent
\textbf{R1 Contribution summary}

\noindent This paper uses the ARM pointer authentication (PA) primitives to implement a pointer-tagging scheme to provide memory safety. The pointer authentication code is generated for pointers to selective data objects and the tag is stored in the unused bits of the pointer. Further, the paper prunes unnecessary checks with static taint analysis. The paper reports 7\% average slowdown on SPEC 2006 workloads.

\noindent
\textbf{Paper summary}

\noindent The paper proposes to use pointer authentication like tagging scheme, which builds on prior work Always-On-Safety (AOS), to detect memory safety violations for objects on the heap, stack, and the global space . The idea is to create a tag when the object is allocated based on the pointer value, type, and size. This tag is stored this tag in the upper bits of the pointer. Then there is a hardware bounds table that is used to map the tag to the bounds of the object.

\noindent To enable support for sub-objects, the paper proposes to dynamically creates tags when sub-objects are accessed. It proposes a linked data structure (which it calls sub-object tracing table) and a new instruction bndsrch to identify if sub-objects have already been allocated.

\noindent
\textbf{R2 Strengths}

\noindent Fast and compatible memory safety is a a great direction. If pointer authentication becomes mainstream, repurposing it for providing some memory safety is a useful direction.

\noindent
\textbf{R2 Weaknesses}

\noindent The paper is unclear in many of its mechanisms. Some of which have been previously explored. Static taint analysis, shadow pointer and dynamic mutation for sub-objects have been explored in prior work.

\noindent Limitations of 16-bit tags will prevent it from enforcing full memory safety. The design space is not carefully explored.

\noindent Lacks a critical analysis of performance benefits.

\noindent
\textbf{R2 Overall merit}

\noindent 1. Reject

\noindent
\textbf{Questions for authors’ response}

\noindent See the detailed R2 comments for the context for the questions.

\noindent Can you tell where the performance benefits of WYFY is coming from in contrast to prior pointer-based techniques?

\noindent Can you provide details on the metadata actually maintained with each PAC entry and how it avoids collisons?

\noindent Highlight the novelty of dynamic pointer mutation and shadow pointers compared to the sub-object identification in SoftBound?

\noindent Can you compare the guarantees of WYFY in detecting dangling pointers in comparison to pool-allocation techniques?

\noindent
\textbf{R1 Comments for author}

\noindent The abstract is well motivated. It solves an important problem of enforcing memory safety.

\noindent I had a hard time figuring out the key insight of the paper. The use of pointer authentication codes and propagation of tags in the unused bits of the pointer is now used by numerous techniques. The abstract would have been stronger if it highlighted what was novel/unique about data-pointer signing in comparison to a lot of recent work in this space.

\noindent The abstract claims it provides compatibility. It is unclear what trade-offs are being made between comprehensive protection versus compatibility.

\noindent Similarly, 56-bits of the virtual address space will soon be used on x86-64 bit systems. It is unclear how future proof the proposed approach is.

\noindent
\textbf{R2 Comments for author}

\noindent Thanks for the submitting the paper to ASPLOS. I like the direction of repurposing pointer authentication to provide memory safety.

\noindent I think the paper is still not ready for ASPLOS for the following reasons. Addressing the comments below will make the paper stronger.

\noindent Compared to pointer-based checking schemes like HardBound/Watchdog/Intel MPX, the key benefit of pointer tagging is primarily in reducing the cost of metadata propagation. As far as I understood the paper, you still need to maintain base and bound for every PAC, so that you can detect whether the pointer is in bounds. The paper does not provide details on how base/bounds are maintained in the hardware bounds table, which maintains a location that has the base and bounds. The above pointer checking schemes maintain bounds in registers, so the checks on a deference are pretty cheap. In contrast, every deference in WYFY needs to consult a hardware bounds table, then likely access memory locations pointed by the entry in the hardware bounds table. Further, you need additional information to detect collisions. So the metadata overhead is similar to pointer-based checking schemes especially with sub-objects. Can you clarify?

\noindent The paper will benefit from a rationale for performance compared to pointer-based checking tools. My hypothesis for better performance of WyFY compared to Watchog/WatchdogLite is from selectively instrumenting objects rather than the metadata.

\noindent The number of pointer tags that can be used are small. There are only 2\textsuperscript{16} pointer tags. You cannot reuse pointer tags, which will decrease the ability to detect errors. Moreover, x86\_64 is going to use 56-bit address spaces soon. Hence, the technique may not be future proof and may have limited value going forward in such scenarios.

\noindent Some of the introduced contributions are not deep in my opinion. For example, "shadow pointer" is pretty trivial. Why can't you use the array name as the pointer for the stack object?

\noindent Similarly, the idea similar to dynamic pointer mutation for sub-objects was proposed in SoftBound [PLDI 2009] (see the section on Optional narrowing of bounds). The paper strangely states that SoftBound as not detecting sub-object overflows. AFAIK, CCured and SoftBound papers highlighted the need for detecting sub-object overflows.

\noindent In WYFY, PACs of two different objects of the same type reallocated to the same memory location will be identical. In such cases, the proposed scheme will not be able to detect accesses to dangling pointers. This guarantee is similar to "Automatic Pool Allocation" [Lattner et al, PLDI 2005] used in the SAFECode project. The paper does not provide details on how PAC is actually computed: for example, what is used for the modifier? How do you encode the type with the PAC?

\noindent Writing and exposition can be significantly improved. Section 5.1 is weird. It says it is a study but there is very little information on the study. A lot of other corner cases that are important in the context of memory safety is not addressed. How do you handle zero-length arrays? Similarly Section 4 has 4.1 but no other sub sections.

\noindent How do you handle third party libraries? What happens when a tagged pointer is used in a third-party library? Unless your hardware explicitly ignores the upper 16-bits, you will likely need to perform deep copies of data structures to zero out the upper bits of the pointer. On x86\_64, if you store information in the upper 16-bits and then try to deference, it is not the same as accessing the location without the information in the upper bits.

\noindent What does encryption in PAC buy you? IMO, it just adds more cost to metadata management without providing any additional benefit for the purpose of memory safety.

\section{Reviewer E}

\noindent
\textbf{R1 Contribution summary}

\noindent The paper proposes WYFY, a hardware-assisted bounds checking mechanism that leverages ARM's PAC to tag only those security-critical pointers that are deemed potentially vulnerable by a static taint analysis pass.

\noindent
\textbf{Paper summary}

\noindent The paper extends WYFY, a memory safety solution that extends prior work on Always-on-Safety (AoS) published at MICRO'20. The key additions include -- (a) protections extended to stack and global data objects, (b) a mechanism to selectively insert security checks only for security-critical objects identified through static taint analysis, and (c) a re-signing/mutation scheme for intra-object granularity protection. The evaluation shows that WYFY is able to provide both temporal and spatial memory safety guarantees at an average of 7% in performance overhead.

\noindent
\textbf{R2 Strengths}

\noindent Important research direction

\noindent Modest performance degradation

\noindent Good security evaluation (although could be improved as mentioned in the comments below)

\noindent
\textbf{R2 Weaknesses}

\noindent Low novelty

\noindent Compatibility argument is weak

\noindent Unclear if the decision to selectively apply security checks need to be made at compile-time

\noindent Weak methodology and performance evaluation


\noindent
\textbf{R2 Overall merit}

\noindent 1. Reject

\noindent
\textbf{Questions for authors’ response}

\noindent Please clearly establish your novelty claims in comparison to AoS and other recent related work.

\noindent Please justify your decision to use static taint analysis for selectively inserting/pruning security checks.

\noindent Can you comment on the soundness of the taint analysis procedure and elaborate if and how you deal with the problem of tracking pointer/integer provenance?

\noindent Please tone down your claims regarding compatibility. See further comments below.

\noindent Improve security evaluation to discuss the feasibility/infeasibility of blind attacks.

\noindent Improve performance evaluation methodology and analysis as described in comments below.

\noindent
\textbf{R1 Comments for author}

\noindent Although the motivation for hardware-assisted memory safety is solid, I'm concerned about the highly incremental nature of this proposal. Most of the techniques have been borrowed by prior work, and it is not true that WYFY is the first hardware-based mechanism that ensures complete memory safety with legacy code compatibility. There have been multiple solutions proposed in the past that are legacy code compatible including CHEx86 from ISCA 2020.

\noindent
\textbf{R2 Comments for author}

\noindent The paper tackles an important and a highly relevant problem of providing a high performance and source/binary-compatible memory safety solution for traditional C/C++ applications. The proposed solution is quite attractive due to its low performance overhead and relative simplicity. However, I'm also quite concerned about the low novelty in this work, given the sheer wealth of related work in this area. In particular, it is directly built upon prior work on AoS, leveraging all of its existing protection mechanisms, while only making incremental and straightforward extensions. It would really help if the authors clearly establish their novelty claims head on in the introduction section.

\noindent Of all the extensions proposed by this work, the most prominent one seems to be the selective application of security checks for only security-critical data. This is notably a major deviation from AoS (which by definition is always-on), but also clearly one that provides the most benefit from a performance standpoint (at least as observed from the key performance result shown in Figure 10). However, I'm not completely convinced that this decision needs to happen at compile-time through static taint analysis due to the following reasons. First, the definition of what is considered security-critical can change based on the application, program context, and the execution environment. Second, it is unclear if the analysis described in the paper is sound. I understand that it is a conservative interprocedural pointer analysis, but pointers regularly get passed to and get manipulated at external functions from completely different modules. Extending such an analysis across modules and to library functions seems non-trivial. Third, it is unclear if and how WYFY addresses the problem of tracking pointer and integer provenance.

\noindent My other major concern is about the compatibility argument made in the paper. While I agree with the authors that no source code changes are required and the solution does not violate any ABI requirements, it is important to note that it also does not offer memory safety protections for legacy code. It also requires ISA modifications on top of those already required by AoS, which makes the compatibility argument much weaker. Multiple solutions presented in Table 4 offer protections for legacy code without requiring any source-level, binary-level, or ISA modifications. On that note (and as mentioned in my R1 review), the paper also leaves out an important prior work, CHEx86 (published at ISCA'20), from its related work section and comparison in Table 4. Not only does CHEx86 offer source/binary/ISA compatibility, but also extends protections to legacy code. In addition, the paper also discusses a context-sensitive variant similar to WYFY, where protections are enabled only for security-critical regions, which makes it a very closely related work that needs to be compared against.

\noindent As for the evaluation, I appreciate that the authors include a security evaluation that demonstrates WYFY's ability to protect against several exploits from the Juliet suite targeting temporal and spatial safety vulnerabilities. I would, however, recommend fleshing out Section 9.2 further with an evaluation that demonstrates the feasibility/infeasibility of blind attacks and entropy exhaustion exploits tailored to break WYFY.

\noindent The performance evaluation in its current form seems quite lacking to me. First, the baseline processor configuration is quite odd with an 8-issue processor with only 192 ROB entries and 32 LQ entries. The latencies of the L2 cache also seems to be omitted. Second, the choice of SPEC CPU 2006 is not appropriate for this evaluation as it doesn't include several pointer-intensive applications that are part of SPEC CPU 2017. It is also not clear if simpoints are used in the evaluation. They should be if they aren't used as pointer access patterns are known to change as execution switches from phase to phase. Third, the experiments seem to be limited to execution time and instruction mix comparison. I'd recommend including some sensitivity studies to understand the impact of different hardware modifications and workload characteristics. Fourth, the evaluation is limited to single-threaded workloads, but it is unclear if there are any additional performance penalties incurred by multithreaded workloads. Finally, Table 4 should also probably include some notion of overhead (performance, power, area, memory, etc.) to allow for a more comprehensive comparison.


\section{How We Address Prior Reviews}
\noindent

\noindent
\textbf{Security implications of static taint analysis}
In Section 11.4, we discuss the security implications of static taint analysis. \hfill \break

\noindent
\textbf{Evaluation methodology}
In our previous submission, we relied on evaluations using the gem5 simulator. In this submission, we completely changed our methodology by prototyping a full system RISC-V architecture and conducted full-system evaluations. \hfill \break

\noindent
\textbf{Applicability to other architectures.}
In section 12.2, we discuss the applicability of our hardware modifications to other architectures. \hfill \break


==> Tex/ZZ.PriorReviews.tex <==
Before this submission, we have submitted to ASPLOS'23 Spring and received valuable reviews from reviewers. In this current version, we addressed the previous reviews as follows.

\section{Reviewer A}
\noindent
\textbf{R1 Contribution summary}

\noindent
The extended abstract presented WYFY, a hardware-software approach that combines data pointer tagging and static analysis to address the memory (un)safety problem in C/C++ applications. The problem is well motivated and the proposed solution aims at addressing the performance/security/compatibility limitations of prior techniques.

\noindent
\textbf{Paper summary}

\noindent
The paper presented WYFY, a hardware-software approach that combines data pointer tagging and static analysis to address the memory (un)safety problem in C/C++ applications. The problem is well motivated and the proposed solution aims at addressing the performance/security/compatibility limitations of prior techniques.

\noindent
\textbf{R2 Strengths}

\noindent [+] Memory safety is an important problem

\noindent [+] The paper is well written

\noindent
\textbf{R2 Weaknesses}

\noindent [-] Minor improvements over prior work

\noindent [-] The evaluation methodology is unclear

\noindent [-] Limited performance evaluation

\noindent [-] Missing important related work

\noindent
\textbf{R2 Overall merit}

\noindent 1. Reject

\noindent
\textbf{Questions for authors’ response}

\noindent Please refer to my comments on the full paper below.

\noindent
\textbf{R1 Comments for author}

\noindent Thank you for submitting your work to ASPLOS. The lack of memory safety in C/C++ is an important problem and developing better hardware-assisted solutions is always needed. I have a few comments after reading the extended abstract:

\noindent 1 - Key contributions: The abstract stated that "none of the prior work achieves full memory safety with legacy code compatibility at reasonable overhead" and " WYFY is the first hardware-based mechanism that ensures complete memory safety with legacy code compatibility". While the abstract cited multiple papers to support this claim (e.g., C3/In-Fat/Califorms/No-FAT), the abstract did not acknowledge a recent work (CHEx86 from ISCA 2020), which also provides complete memory safety at low overheads while having full compatibility with legacy binaries.

\noindent 2 - Advantage over prior work: It is not clear how WYFY is significantly different than AOS (other than the sub-object granularity and stack/global protection). I will defer the decision till reviewing the full paper.

\noindent 3 - Pruning unnecessary security checks: I am a bit concerned about depending on static analysis to selectively protect a subset of program objects. This approach is effective in reducing the performance overheads, yet it typically leaves security holes that could be exploited by an attacker, depending on the soundness of the static analysis.

\noindent 4 - Main Artifacts: Are there any specific reasons to use SPEC CPU 2006 workloads instead of SPEC CPU 2017? The latter have higher memory footprint that may affect the quality of the reported overheads.

\noindent
\textbf{R2 Comments for author}

\noindent Thank you for submitting your work to ASPLOS. The lack of memory safety in C/C++ is an important problem and developing stronger hardware-assisted solutions is always needed. Please find my comments and questions on the full paper below:

\noindent 1 - Key contributions: The paper states that "none of the prior work achieves full memory safety with legacy code compatibility at reasonable overhead" and "WYFY is the first hardware-based mechanism that ensures complete memory safety with legacy code compatibility". While multiple papers are cited to support this claim (e.g., C3/In-Fat/Califorms/No-FAT), the authors did not acknowledge or compare against a recent work (CHEx86 from ISCA 2020), which also provides complete memory safety at low overheads while having full compatibility with legacy binaries. Are there any reason for excluding CHEx86 from the related work section and Table 4?

\noindent 2 - Limited improvements over prior work: It is not clear to me how WYFY is significantly different than AOS. The sub-object granularity and stack/global protection are straightforward extensions that have been discussed in prior memory safety solutions before, such as Intel MPX and CHERI.

\noindent 3 - Binary compatibility: The paper states that WYFY maintains both source and binary compatibility. While I agree that source-code compatibility is guaranteed due to maintaining the same pointer size, I would say pointer tagging techniques (including WYFY) do not maintain binary compatibility with uninstrumented code (e.g., third party libraries) for the following two reasons:

(a) The uninstrumented code might use the upper pointer bits for storing other software-related information, which will corrupt WYFY's metadata or affect the correctness of the uninstrumented code.

(b) Conventional address space formats assume that the pointer upper bits are set to zeros for user-land pointers and ones for kernel pointers. Prior memory safety techniques, such as REST/MPX/CHEx86 are compatible with the aforementioned convention. WYFY on the other hand breaks this convention by introducing PAC in the upper pointer bits.

\noindent While point (b) could be addressed by modifying the hardware to explicitly clear the upper pointer bits before memory accesses, point (a) needs further consideration to guarantee smooth interaction with uninstrumented third-party code.

\noindent 4 - Temporal memory safety: If I understood correctly, WYFY detects temporal safety violations as dangling pointers to any free'd objects will remain signed whereas the corresponding HBT entry will be removed, causing a bounds-checking error upon any later dangling pointer access. What would happen after reusing the HBT entry for a new allocation? Won't it be possible to have the PAC of the new allocation collide with the PAC of the dangling pointer, causing the temporal error to go undetected? I think simply maintaining all bounds information of previously free'd objects per each PAC will significantly increase the proposal complexity as the metadata will now become a factor of the overall program objects (millions) and not just the number of live objects.

\noindent 5 - Pruning unnecessary security checks: I am a bit concerned about depending on static analysis to selectively protect a subset of program objects. This approach is effective in reducing the performance overheads, yet it typically leaves security holes that could be exploited by an attacker, depending on the soundness of the static analysis.

\noindent 6 - Using LLVM IR GEP instructions for sub-object memory safety: There is a major caveat in this design choice. The GEP instruction calculates the address of the indexed sub-object by adding an offset to the object base address as seen within the same function scope. In other words, if a function foo(void *ptr) receives a sub-object pointer that has already been adjusted in a different function scope, the GEP instruction within foo will not use the correct base address as a parameter. Instead, it will just add the new offset to the previously-adjusted pointer. How would WYFY handle those cases?

\noindent 7 - Evaluation Methodology: The used evaluation methodology is unclear. Have you run all programs end-to-end on Gem5? If not, have you used sim-points or run the first few billion instructions as AoS?

\noindent 8 - Main artifacts: Are there any specific reasons to use SPEC CPU 2006 workloads instead of SPEC CPU 2017? The latter have higher memory footprint that may affect the quality of the reported overheads.

\noindent 9 - Missing benchmarks: Additionally, all the heavyweight benchmarks (e.g., perlbench, gcc) are not evaluated. Even if certain applications have memory safety bugs (I see that reference [41] only reports four bugs in SPEC 2006), you could either patch those bugs prior to running the performance evaluation or silence the corresponding bounds-checking alarms at runtime to allow for end-to-end evaluation.

\noindent 10 - Reported statistics: It is unclear how the results of Table 2 (\#Total) columns are collected. Do they correspond to end-to-end program execution? If yes, the \#Total heap objects are significantly lower than the ones reported in prior work (e.g., AoS). If no, could you please clarify the reason?

\noindent 11 - Multi-threading support: It would be useful to include a discussion on how WYFY handles multi-threaded applications especially the metadata management aspect and whether it causes any false positives on not.

\noindent 12 - Threat model: While the paper states that side-channel attacks are out-of-scope, I believe a discussion on how side-channel leakage could affect the security guarantees of WYFY (and any future memory safety solution) is important. For example, recent reports (e.g., https://github.com/microsoft/MSRC-Security-Research/blob/master/papers/2020/Security analysis of memory tagging.pdf) discussed how a simple leakage can undermine the security guarantees of memory tagging schemes, such as ARM MTE.

\section{Reviewer B}

\noindent
\textbf{R1 Contribution summary}

\noindent This paper presents WYFY, a workflow for achieving memory safety. The key idea is to use a combination of static program analysis and hardware-based memory protection (ARM pointer authentication). The paper claims to provide complete memory safety (more on this below).

\noindent
\textbf{Paper summary}

\noindent WYFY is a combined hardware/software approach to ensuring memory safety. The main idea is to perform program analysis offline in order to determine how external data inputs affect code that may be exploitable and then protect such code using hardware support. There are additional techniques used under a broad scheme called "data-pointer signing" to treat stack and global objects similarly to how the heap is treated (i.e., by using a shadow pointer). WYFY is low overhead and its security is evaluated using various benchmarks by the authors.

\noindent
\textbf{R2 Strengths}

\noindent Memory safety is a critical issue that requires an effective and efficient solution.
The paper is clearly written and easily understandable

\noindent
\textbf{R2 Weaknesses}

\noindent The most glaring weakness is that the paper is quite incremental compared to AOS. It seems like the main improvement over AOS is that the authors added protection for stack and global variables.
The other major weakness is that the security assumptions are not clearly discussed. I think intuitively, it makes sense that most vulnerable code can be manipulated with external inputs. However, I'd have hoped for a discussion of the implications of this design decision.

\noindent
\textbf{R2 Overall merit}

\noindent 2. Major revision - weak paper, but it has value and can be fixed with revisions

\noindent
\textbf{Questions for authors’ response}

\noindent 1- Can you clearly articulate the major improvements over AOS and how your approach differs? 2- Are there any downsides of the assumption that most vulnerable code can be manipulated using external inputs? Are you missing anything due to this assumption? 3- Is it safe to rely of getelementpointer to ensure security of sub-objects in the presence of pointer aliasing? I guess you mention your analysis is conservative, but wouldn't his result in over-tainting in most legacy code?

\noindent
\textbf{R1 Comments for author}

\noindent (1) The motivation for the paper is quite clear. Memory bugs are still a big problem that causes many security vulnerabilities and innovative and low overhead solutions are welcome.

\noindent (2) It is unclear how the approach is able to provide complete memory safety given that it is only targeted at a subset of memory objects based on a heuristic. You say that vulnerabilities are "typically" exploited through untrusted external inputs. How do you identify untrusted inputs? Is the solution complete as you propose? How can you provide that it is complete? All these questions need to be answered for the claims to be credible and the EA has no evidence to answer these claims. However, the EA is intriguing, and I think the paper should advance to the next round.

\noindent (3) I don't think the idea to try to identify code that must be kept secure is a new one. There is a lot of work on program partitioning in the same vein. I expect this kind of defense to be evaluated with memory intensive applications, and this paper doesn't appear to have done so, which makes it a bit hard to interpret the results. I think the paper needs to better articulate the architectural support and its contributions (presumably the EA is lacking in this but the actual paper does a better job).

\noindent (4) The paper is a good fit for ASPLOS

\noindent
\textbf{R2 Comments for author}

\noindent (1) I think the main insights of the paper are sound and if the revision requests that I outline below are addressed, the paper can be published. This is of course assuming there is a clear differentiator between the proposed approach in this paper and AOS (this wasn't clear to me at all, beyond the simple things like extending protections to stack and globals).

\noindent (2) As mentioned above, the clear advantage over prior work is unclear and the most significant weakness of this paper.

\noindent (3) The paper is otherwise a really good for ASPLOS.

\noindent (4) The approach seems to be sound, given the assumption that vulnerable code can only be accessed via externally manipulatable inputs. Is this always true? It seems like it is intuitively true, but I'd like the authors to comment on this and argue for why this is a foolproof heuristic. If it is not (and that it OK), I'd like a more thorough discussion of the limitations. Note that such limitations wouldn't preclude an acceptance from my perspective. I am actually on board with the idea that the most relevant security-critical code is one that can be manipulated by external inputs.

\noindent
\textbf{Revision requests}

\noindent A clear description of the difference between AOS and WYFY must be present in the revision.

\noindent A justification for the security assumptions (dependence on external inputs) must be present in the revision.

\section{Reviewer C}

\noindent
\textbf{R1 Contribution summary}

\noindent This work proposes a memory safety framework that allows unmodified code to run with minimal performance overhead.

\noindent
\textbf{Paper summary}

\noindent This work proposes to enhance prior work on pointer safety to protect all of the memory address space, including stack and global variables. The work also includes a static taint analysis that aims to reduce the number of checks that need to be done at runtime.

\noindent
\textbf{R2 Strengths}

\noindent Provides pointer safety for all object types (stack, heap, global variable) Keep compatibility for legacy code Pruning mechanism to reduce the security check overhead.

\noindent
\textbf{R2 Weaknesses}

\noindent it is unclear what the novelty over AOS is. It seems that this work is simply extending AOS to allow for stack and global variable protection, but it is not clear why these are challenging to merit a publication on its own. The evaluation is a bit concerning as it seems the authors are cherry picking the benchmarks that perform best. The authors decided to exclude 6 benchmarks because their approach found too many errors.

\noindent
\textbf{R2 Overall merit}

\noindent 2. Major revision - weak paper, but it has value and can be fixed with revisions

\noindent
\textbf{Questions for authors’ response}

\noindent Can you succinctly state what are the challenges (or key insights) that allow you to protect the stack and global variable sin a more efficient way compared to AOS?

\noindent Did you evaluate how much bigger your binary is after your compiler modifications? I see you have how many more instructions are executed on figure 11 but this is limited by your evaluation methodology.

\noindent How does it work with the global variables bounds that are never released? Is the HBT per process and hence flushed after the program exits?

\noindent How do you handle context switches?

\noindent If you assume the inputs to main to be tainted, doesn't this guarantee that the whole program is tainted? Presumably the inputs to main are used for something useful in most programs. What am i missing here?

\noindent What does it mean for your analysis to be field sensitive?

\noindent Can you please explain further what happened with the additional 6 benchmarks that you excluded? This seems like cherry picking to me. I can definitely be wrong but please explain why i would be wrong.

\noindent How do you guarantee that the experiments you ran go through the same call path as the baseline? Are you taking checkpoints? ?Are you warming up the system? Are you running a specific number of instructions?

\noindent What happens when the bndclr instruction fails? How is this protecting against double free attacks?

\noindent
\textbf{R1 Comments for author}

\noindent Memory safety is definitely an important security feature that should be included in all computing devices without incurring significant cost. The key insights are interesting and could merit a second look to determine their worth. The contribution, while still with some performance overhead, enables the implementation of memory safety without having to modify legacy code. The paper is a good fit for ASPLOS.

\noindent
\textbf{R2 Comments for author}

\noindent The key insights of the work are unclear, particularly when you compare the contributions to AOS. The paper does not really related the reasons why you chose the particular details of your design, making it difficult to understand the novelty of your work. Your evaluation methodology is a bit odd. Excluding benchmarks because they have bad performance is not really good practice. I could be wrong here, hence my questions above. Furthermore, it is unclear how you guaranteed the gem5 runs to always go through the same call path, as you give no details about how you ran your programs. Also, this is no a show stopper but you are using SPEC 2006 which is now very outdated. I highly recommend upgrading to SPEC2017.

\noindent
\textbf{Revision requests}

\noindent I would like to see the distinctions and key insights compared to AOS clearly outlined. I would also like to see an analysis on how this approach inflates binaries (by how much). I would like to see an explanation of how experiments were ran to guarantee the call path is the same as the baseline. The writing needs to be polished so that the main ideas are clearly explained.

\section{Reviewer D}

\noindent
\textbf{R1 Contribution summary}

\noindent This paper uses the ARM pointer authentication (PA) primitives to implement a pointer-tagging scheme to provide memory safety. The pointer authentication code is generated for pointers to selective data objects and the tag is stored in the unused bits of the pointer. Further, the paper prunes unnecessary checks with static taint analysis. The paper reports 7\% average slowdown on SPEC 2006 workloads.

\noindent
\textbf{Paper summary}

\noindent The paper proposes to use pointer authentication like tagging scheme, which builds on prior work Always-On-Safety (AOS), to detect memory safety violations for objects on the heap, stack, and the global space . The idea is to create a tag when the object is allocated based on the pointer value, type, and size. This tag is stored this tag in the upper bits of the pointer. Then there is a hardware bounds table that is used to map the tag to the bounds of the object.

\noindent To enable support for sub-objects, the paper proposes to dynamically creates tags when sub-objects are accessed. It proposes a linked data structure (which it calls sub-object tracing table) and a new instruction bndsrch to identify if sub-objects have already been allocated.

\noindent
\textbf{R2 Strengths}

\noindent Fast and compatible memory safety is a a great direction. If pointer authentication becomes mainstream, repurposing it for providing some memory safety is a useful direction.

\noindent
\textbf{R2 Weaknesses}

\noindent The paper is unclear in many of its mechanisms. Some of which have been previously explored. Static taint analysis, shadow pointer and dynamic mutation for sub-objects have been explored in prior work.

\noindent Limitations of 16-bit tags will prevent it from enforcing full memory safety. The design space is not carefully explored.

\noindent Lacks a critical analysis of performance benefits.

\noindent
\textbf{R2 Overall merit}

\noindent 1. Reject

\noindent
\textbf{Questions for authors’ response}

\noindent See the detailed R2 comments for the context for the questions.

\noindent Can you tell where the performance benefits of WYFY is coming from in contrast to prior pointer-based techniques?

\noindent Can you provide details on the metadata actually maintained with each PAC entry and how it avoids collisons?

\noindent Highlight the novelty of dynamic pointer mutation and shadow pointers compared to the sub-object identification in SoftBound?

\noindent Can you compare the guarantees of WYFY in detecting dangling pointers in comparison to pool-allocation techniques?

\noindent
\textbf{R1 Comments for author}

\noindent The abstract is well motivated. It solves an important problem of enforcing memory safety.

\noindent I had a hard time figuring out the key insight of the paper. The use of pointer authentication codes and propagation of tags in the unused bits of the pointer is now used by numerous techniques. The abstract would have been stronger if it highlighted what was novel/unique about data-pointer signing in comparison to a lot of recent work in this space.

\noindent The abstract claims it provides compatibility. It is unclear what trade-offs are being made between comprehensive protection versus compatibility.

\noindent Similarly, 56-bits of the virtual address space will soon be used on x86-64 bit systems. It is unclear how future proof the proposed approach is.

\noindent
\textbf{R2 Comments for author}

\noindent Thanks for the submitting the paper to ASPLOS. I like the direction of repurposing pointer authentication to provide memory safety.

\noindent I think the paper is still not ready for ASPLOS for the following reasons. Addressing the comments below will make the paper stronger.

\noindent Compared to pointer-based checking schemes like HardBound/Watchdog/Intel MPX, the key benefit of pointer tagging is primarily in reducing the cost of metadata propagation. As far as I understood the paper, you still need to maintain base and bound for every PAC, so that you can detect whether the pointer is in bounds. The paper does not provide details on how base/bounds are maintained in the hardware bounds table, which maintains a location that has the base and bounds. The above pointer checking schemes maintain bounds in registers, so the checks on a deference are pretty cheap. In contrast, every deference in WYFY needs to consult a hardware bounds table, then likely access memory locations pointed by the entry in the hardware bounds table. Further, you need additional information to detect collisions. So the metadata overhead is similar to pointer-based checking schemes especially with sub-objects. Can you clarify?

\noindent The paper will benefit from a rationale for performance compared to pointer-based checking tools. My hypothesis for better performance of WyFY compared to Watchog/WatchdogLite is from selectively instrumenting objects rather than the metadata.

\noindent The number of pointer tags that can be used are small. There are only 2\textsuperscript{16} pointer tags. You cannot reuse pointer tags, which will decrease the ability to detect errors. Moreover, x86\_64 is going to use 56-bit address spaces soon. Hence, the technique may not be future proof and may have limited value going forward in such scenarios.

\noindent Some of the introduced contributions are not deep in my opinion. For example, "shadow pointer" is pretty trivial. Why can't you use the array name as the pointer for the stack object?

\noindent Similarly, the idea similar to dynamic pointer mutation for sub-objects was proposed in SoftBound [PLDI 2009] (see the section on Optional narrowing of bounds). The paper strangely states that SoftBound as not detecting sub-object overflows. AFAIK, CCured and SoftBound papers highlighted the need for detecting sub-object overflows.

\noindent In WYFY, PACs of two different objects of the same type reallocated to the same memory location will be identical. In such cases, the proposed scheme will not be able to detect accesses to dangling pointers. This guarantee is similar to "Automatic Pool Allocation" [Lattner et al, PLDI 2005] used in the SAFECode project. The paper does not provide details on how PAC is actually computed: for example, what is used for the modifier? How do you encode the type with the PAC?

\noindent Writing and exposition can be significantly improved. Section 5.1 is weird. It says it is a study but there is very little information on the study. A lot of other corner cases that are important in the context of memory safety is not addressed. How do you handle zero-length arrays? Similarly Section 4 has 4.1 but no other sub sections.

\noindent How do you handle third party libraries? What happens when a tagged pointer is used in a third-party library? Unless your hardware explicitly ignores the upper 16-bits, you will likely need to perform deep copies of data structures to zero out the upper bits of the pointer. On x86\_64, if you store information in the upper 16-bits and then try to deference, it is not the same as accessing the location without the information in the upper bits.

\noindent What does encryption in PAC buy you? IMO, it just adds more cost to metadata management without providing any additional benefit for the purpose of memory safety.

\section{Reviewer E}

\noindent
\textbf{R1 Contribution summary}

\noindent The paper proposes WYFY, a hardware-assisted bounds checking mechanism that leverages ARM's PAC to tag only those security-critical pointers that are deemed potentially vulnerable by a static taint analysis pass.

\noindent
\textbf{Paper summary}

\noindent The paper extends WYFY, a memory safety solution that extends prior work on Always-on-Safety (AoS) published at MICRO'20. The key additions include -- (a) protections extended to stack and global data objects, (b) a mechanism to selectively insert security checks only for security-critical objects identified through static taint analysis, and (c) a re-signing/mutation scheme for intra-object granularity protection. The evaluation shows that WYFY is able to provide both temporal and spatial memory safety guarantees at an average of 7% in performance overhead.

\noindent
\textbf{R2 Strengths}

\noindent Important research direction

\noindent Modest performance degradation

\noindent Good security evaluation (although could be improved as mentioned in the comments below)

\noindent
\textbf{R2 Weaknesses}

\noindent Low novelty

\noindent Compatibility argument is weak

\noindent Unclear if the decision to selectively apply security checks need to be made at compile-time

\noindent Weak methodology and performance evaluation


\noindent
\textbf{R2 Overall merit}

\noindent 1. Reject

\noindent
\textbf{Questions for authors’ response}

\noindent Please clearly establish your novelty claims in comparison to AoS and other recent related work.

\noindent Please justify your decision to use static taint analysis for selectively inserting/pruning security checks.

\noindent Can you comment on the soundness of the taint analysis procedure and elaborate if and how you deal with the problem of tracking pointer/integer provenance?

\noindent Please tone down your claims regarding compatibility. See further comments below.

\noindent Improve security evaluation to discuss the feasibility/infeasibility of blind attacks.

\noindent Improve performance evaluation methodology and analysis as described in comments below.

\noindent
\textbf{R1 Comments for author}

\noindent Although the motivation for hardware-assisted memory safety is solid, I'm concerned about the highly incremental nature of this proposal. Most of the techniques have been borrowed by prior work, and it is not true that WYFY is the first hardware-based mechanism that ensures complete memory safety with legacy code compatibility. There have been multiple solutions proposed in the past that are legacy code compatible including CHEx86 from ISCA 2020.

\noindent
\textbf{R2 Comments for author}

\noindent The paper tackles an important and a highly relevant problem of providing a high performance and source/binary-compatible memory safety solution for traditional C/C++ applications. The proposed solution is quite attractive due to its low performance overhead and relative simplicity. However, I'm also quite concerned about the low novelty in this work, given the sheer wealth of related work in this area. In particular, it is directly built upon prior work on AoS, leveraging all of its existing protection mechanisms, while only making incremental and straightforward extensions. It would really help if the authors clearly establish their novelty claims head on in the introduction section.

\noindent Of all the extensions proposed by this work, the most prominent one seems to be the selective application of security checks for only security-critical data. This is notably a major deviation from AoS (which by definition is always-on), but also clearly one that provides the most benefit from a performance standpoint (at least as observed from the key performance result shown in Figure 10). However, I'm not completely convinced that this decision needs to happen at compile-time through static taint analysis due to the following reasons. First, the definition of what is considered security-critical can change based on the application, program context, and the execution environment. Second, it is unclear if the analysis described in the paper is sound. I understand that it is a conservative interprocedural pointer analysis, but pointers regularly get passed to and get manipulated at external functions from completely different modules. Extending such an analysis across modules and to library functions seems non-trivial. Third, it is unclear if and how WYFY addresses the problem of tracking pointer and integer provenance.

\noindent My other major concern is about the compatibility argument made in the paper. While I agree with the authors that no source code changes are required and the solution does not violate any ABI requirements, it is important to note that it also does not offer memory safety protections for legacy code. It also requires ISA modifications on top of those already required by AoS, which makes the compatibility argument much weaker. Multiple solutions presented in Table 4 offer protections for legacy code without requiring any source-level, binary-level, or ISA modifications. On that note (and as mentioned in my R1 review), the paper also leaves out an important prior work, CHEx86 (published at ISCA'20), from its related work section and comparison in Table 4. Not only does CHEx86 offer source/binary/ISA compatibility, but also extends protections to legacy code. In addition, the paper also discusses a context-sensitive variant similar to WYFY, where protections are enabled only for security-critical regions, which makes it a very closely related work that needs to be compared against.

\noindent As for the evaluation, I appreciate that the authors include a security evaluation that demonstrates WYFY's ability to protect against several exploits from the Juliet suite targeting temporal and spatial safety vulnerabilities. I would, however, recommend fleshing out Section 9.2 further with an evaluation that demonstrates the feasibility/infeasibility of blind attacks and entropy exhaustion exploits tailored to break WYFY.

\noindent The performance evaluation in its current form seems quite lacking to me. First, the baseline processor configuration is quite odd with an 8-issue processor with only 192 ROB entries and 32 LQ entries. The latencies of the L2 cache also seems to be omitted. Second, the choice of SPEC CPU 2006 is not appropriate for this evaluation as it doesn't include several pointer-intensive applications that are part of SPEC CPU 2017. It is also not clear if simpoints are used in the evaluation. They should be if they aren't used as pointer access patterns are known to change as execution switches from phase to phase. Third, the experiments seem to be limited to execution time and instruction mix comparison. I'd recommend including some sensitivity studies to understand the impact of different hardware modifications and workload characteristics. Fourth, the evaluation is limited to single-threaded workloads, but it is unclear if there are any additional performance penalties incurred by multithreaded workloads. Finally, Table 4 should also probably include some notion of overhead (performance, power, area, memory, etc.) to allow for a more comprehensive comparison.


\section{How We Address Prior Reviews}
\noindent

\noindent
\textbf{Security implications of static taint analysis}
In Section 11.4, we discuss the security implications of static taint analysis. \hfill \break

\noindent
\textbf{Evaluation methodology}
In our previous submission, we relied on evaluations using the gem5 simulator. In this submission, we completely changed our methodology by prototyping a full system RISC-V architecture and conducted full-system evaluations. \hfill \break

\noindent
\textbf{Applicability to other architectures.}
In section 12.2, we discuss the applicability of our hardware modifications to other architectures. \hfill \break


==> Tex/ZZZ.Rebuttal.tex <==
# Reviewer A
- Is RV-CURE capable handling memory safety of multi-threaded programs where threads execute on concurrent cores.

- Does RV-CURE prevent Pacman like disclosure of capability information.

- Are the perl benchmark overheads with RV-CURE fundamental or is there a way to address this in the future?

- What are the memory overheads of RV-CURE?

- Does RV-CURE slows down the execution of code that does not use any memory safety support from the hardware?

- For taint analysis, what is the strategy for pointers passed to external libraries? What are the list of sources you are currently accounting for? Do you mark direct syscalls?

# Reviewer C
- How does RV-CURE outperform the state of the art, e.g. No-FAT in terms of performance and/or security?

- How does the CMT structure look like and it is a SRAM-based structure accessed by hardware or software-based data structure that can be resized if required?

- What are the limitations of this approach for identifying the memory bounds of objects?


# Reviewer E
- Could you elaborate on the use of permissions (as mentioned in chapter 5.2)? It is unclear to me how the "cstr" instruction knows which permissions to use, and also, Figure 5 does not mention them.

- How does the compiler know when a function call is an allocation? E.g., when using third-party, dynamically linked, allocation libraries with potentially obscure functions like realpath.

% Response
We really appreciate your valuable comments and feedback. We answer the questions from reviewers as follows.

\textbf{[A,E] Multithreading}

RV-CURE can handle multithreaded programs. One essential property of DPT is atomic capability checks performed for each memory instruction without explicit instructions. Therefore, RV-CURE is free from data race issues that can happen between capability load and check instructions. The consistency of the capability cache can be ensured by the conventional cache coherence protocol. While capability metadata can be shared across concurrent threads (or cores), once an owner core modifies certain metadata, the coherence protocol will send invalidate requests to other sharer cores. By taking those requests, it's possible to invalidate the corresponding entry of the capability cache.

\textbf{[A] Resilience against PACMAN-like Disclousre}

In our current setting, we cannot prevent tag disclosure by speculative execution attacks. However, we believe such disclosure can lead to actual exploits when memory violations, e.g., tag overwrite via buffer overflow, are exploitable. Hence, RV-CURE can still make the system more resilient against such attacks.

\textbf{[A] Memory overhead}

The memory overhead is mainly caused by the CMT (4MB with 8 ways) and thus is not significant. Note that DPT does not require explicit metadata propagation which can create multiple metadata copies, causing increased memory overhead.

\textbf{[A] Normal execution overhead}

When the enableDPT CSR (Table 3) is false, the CPU pipeline operates in normal mode without any execution overhead.

\textbf{[A] Taint analysis regarding external libraries}

For known I/O functions in C/C++, we taint function arguments specifying destination addresses as well as return values of the functions. For external libraries or intrinsic functions (including syscalls) of which function body is not represented in LLVM IR, we taint all pointer-type function arguments and return values.

\textbf{[C] Comparison to No-FAT}

No-FAT presented an elegant approach for full memory safety. However, the No-FAT's mechanism is highly tied to the heap memory layout supported by the binning memory allocation. Also, No-FAT requires formidable compiler instrumentation for: 1) transforming all stack and global object allocations to heap allocations and 2) modifying data layout of structs via source-to-source translation, which can cause compatibility issues with external libraries. Compared to No-FAT, RV-CURE changes neither object-allocation semantics nor data structures of objects.

\textbf{[C] CMT structure}

The CMT is a software-based data structure maintained in memory space. For each tagged memory instruction, the hardware calculates a virtual memory address using the base address of the CMT and the instruction's tag and generates a capability-check request to memory. With the support of hardware-based iteration, RV-CURE enables transparent capability checks without additional instruction overhead.

\textbf{[C] Memory bounds identification}

From our experience, variable-sized arrays, e.g., arr[], are represented differently as typical allocations in LLVM IR. We handle such cases by taking the size variable itself as a source operand of a cstr instruction.

\textbf{[E] Use of permissions}

While we leave the use of various permissions as our future work, we expect that more permissions, e.g., read-only property for constant values, execute property for memory chunks used by JIT, by introducing variants of capability store instructions.

\textbf{[E] Memory allocation identification}

Although programmer's intervention would be needed in the end, we think the compiler pass can be extended to accept the list of third-party allocation functions and apply the pointer tagging and capability assignment for returned pointers.

